First-Order Methods for Linearly Constrained Bilevel Optimization

Algorithms for bilevel optimization often encounter Hessian computations, which are prohibitive in high dimensions. While recent works offer first-order methods for unconstrained bilevel problems, the constrained setting remains relatively underexplored. We present first-order linearly constrained optimization methods with finite-time hypergradient stationarity guarantees. For linear equality constraints, we attain $\epsilon$-stationarity in $\widetilde{O}(\epsilon^{-2})$ gradient oracle calls, which is nearly-optimal. For linear inequality constraints, we attain $(\delta,\epsilon)$-Goldstein stationarity in $\widetilde{O}(d{\delta^{-1} \epsilon^{-3}})$ gradient oracle calls, where $d$ is the upper-level dimension. Finally, we obtain for the linear inequality setting dimension-free rates of $\widetilde{O}({\delta^{-1} \epsilon^{-4}})$ oracle complexity under the additional assumption of oracle access to the optimal dual variable. Along the way, we develop new nonsmooth nonconvex optimization methods with inexact oracles. We verify these guarantees with preliminary numerical experiments.

==> backup_src/abstract.tex <==
Algorithms for bilevel optimization often encounter Hessian computations, which are prohibitive in high dimensions. While recent works offer first-order methods for {unconstrained} bilevel problems, the \textit{constrained} setting remains relatively underexplored. We present  first-order linearly constrained optimization methods with finite-time hypergradient stationarity guarantees. For linear \textit{equality} constraints, we attain $\epsilon$-stationarity in $\widetilde{O}(\epsilon^{-2})$ gradient oracle calls, which is nearly-optimal. 
For linear \textit{inequality} constraints, we attain $(\delta,\epsilon)$-Goldstein stationarity in $\widetilde{O}(d{\delta^{-1} \epsilon^{-3}})$ gradient oracle calls, where $d$ is the upper-level dimension. 
Finally, we obtain for the linear inequality setting dimension-free rates of $\widetilde{O}({\delta^{-1} \epsilon^{-4}})$ oracle complexity under the additional assumption of oracle access to the optimal dual variable. Along the way, we develop new nonsmooth nonconvex optimization methods with inexact oracles. Our numerical experiments verify these guarantees.


==> backup_src/conclusion.tex <==
\section{Limitations and future directions}\label{sec:limitation}
One limitation to our approach is that the inexact gradient oracle we constructed in \cref{sec:inequality-bilevel} requires access to the exact dual multiplier $\lambda^*$.
For a first-order algorithm, the closest proxy one could get to this would be a highly accurate approximation (which could be computed up to $\epsilon$ error in $O(\log(1/\epsilon))$ gradient oracle evaluations). Removing this ``exact dual access'' assumption (\cref{{item:assumption_safe_constraints}}) would be an important result. 

Another important direction for future work would be to extend the hypergradient stationarity guarantee of \cref{thm:linIneqInformal} to bilevel programs with \emph{general convex} constraints. 
To this end, we conjecture that the use of a 
primal-only gradient approximation oracle could be potentially effective. 

Finally, our current rate of $\widetilde{O}(\delta^{-1} \epsilon^{-4})$ oracle calls for reaching $(\delta,\epsilon)$-Goldstein stationarity is not necessarily inherent to the problem; indeed, it might be the case that an alternate approach could improve it to the best known rate of ${O}(\delta^{-1} \epsilon^{-3})$ for nonsmooth nonconvex optimization.

\section*{Acknowledgments} 
GK is supported by an Azrieli Foundation graduate fellowship. 
KW is supported by Schmidt Sciences AI2050 Fellowship and NSF IIS-2403240. SS acknowledges generous support from the Alexander von Humboldt Foundation. SP is supported by  NSF CCF-2112665 (TILOS AI Research Institute) and gratefully acknowledges Ali Jadbabaie for many useful discussions. 
ZZ is supported by NSF FODSI Fellowship. 

==> backup_src/condensed-relatedwork.tex <==
\subsection{Related work}\label{sec:related_work} 
The vast body of work on asymptotic results for bilevel programming, starting with classical works such as \citet{anandalingam1990solution, ishizuka1992double, white1993penalty, vicente1994descent, ye1995optimality, ye1997exact}, typically fall into two categories: those based on approximate implicit differentiation: ~\citet{domke2012generic, pedregosa2016hyperparameter, gould2016differentiating, amos2017optnet, liao2018reviving, agrawal2019differentiable, grazzi2020iteration, lorraine2020optimizing} and those via iterative differentiation:~\citet{domke2012generic, maclaurin2015gradient, franceschi2017forward,   franceschi2018bilevel,  shaban2019truncated, grazzi2020iteration}. Another recent line of work  in this category includes \citet{liu2021value, ye2023difference, khanduri2023linearly, gao2024moreau}, which use various smoothing techniques. 

The first non-asymptotic result for bilevel programming was provided by \citet{ghadimi2018approximation}, which was followed by a flurry of work: for example, algorithms that are single-loop stochastic: ~\citet{chen2021closing, chen2022single, hong2023two}, projection-free: ~\citet{akhtar2022projection, jiang2023conditional, abolfazli2023inexact, cao2024projection}, use variance-reduction and momentum: ~\citet{khanduri2021near, guo2021randomized, yang2021provably, dagreou2022framework}, those for single-variable bilevel programs: ~\citet{sabach2017first, amini2019iterative, amini2019iterativereg, jiang2023conditional, merchav2023convex}, and  for bilevel programs with special  constraints: ~\citet{tsaknakis2022implicit, khanduri2023linearly, xu2023efficient, abolfazli2023inexact}. 

The most direct predecessors of our work are those by \citet{liu2021value, kwon2023fully, yao2024constrained, lu2024firstorder, khanduri2023linearly}. As alluded to earlier, \citet{liu2022bome} recently made a significant contribution by providing  for bilevel programming a fully first-order algorithm with finite-time stationarity guarantees. 
This was extended to the stochastic setting by \citet{kwon2023fully} (which we build upon), simplified and improved by \citet{chen2023near}, and extended to the constrained setting by \citet{yao2024constrained, lu2024firstorder, khanduri2023linearly}.

The works of \citet{yao2024constrained, lu2024firstorder} study the more general problem of bilevel programming with {general convex} constraints. However, they use KKT stationarity as a proxy to the hypergradient stationarity. Our \cref{thm:linIneqInformal} is restricted to linear inequality constraints,  we provide stationarity guarantees 
directly in terms of the objective of interest.
Moreover, \citet{yao2024constrained} assumes joint convexity of the lower-level constraints in upper and lower variables to allow for efficient projections, 
while we require convexity only in the lower-level variable. 
% Indeed, \cref{thm:linIneqInformal} also applies when the lower-level constraint is \emph{bilinear} in $x$ and $y$, a setting \cite{yao2024constrained} does not extend to. 

% Furthermore, as alluded to earlier, compared with \cite{khanduri2023linearly} (which also solves linearly constrained bilevel programming), \pswt{repeat-ish}
The current best result for the linearly constrained setting is that of \citet{khanduri2023linearly}. However, this work 
requires Hessian computations (and is therefore not fully first-order). Moreover, \citet{khanduri2023linearly} imposes {strong regularity assumptions}  on the hyperobjective $F$, which are, in general, impossible to verify.
In contrast,  \Cref{thm:lineq-cost-inf} imposes \textit{assumptions solely on the constituent functions $f$ and $g$}, none directly on $F$,
thus making substantial progress on these two fronts.

% Furthermore, under slightly stronger assumptions, \cref{thm:linIneqInformal} is,  to the best of our knowledge, the first to achieve fully first-order finite-time $(\delta,\epsilon)$-stationarity of the hypergradient for linearly constrained bilevel optimization (cf. \cref{sec:related_work} for a discussion of \cite{yao2024constrained, lu2024firstorder}, which solve the general constrained bilevel program). 

==> backup_src/experiment.tex <==
\section{Experiments}\label{sec:exp}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{src/figures/ydim200_loss.pdf}
        \caption{Convergence and gradient error of Fully First-order Constrained Bilevel Algorithm (F2CBA) compared to cvxpylayer~\cite{agrawal2019differentiable}.}
        \label{fig:convergence-comparison}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{src/figures/ydim200_gradient_error.pdf}
        \caption{Convergence analysis with varying gradient inexactness $\alpha$ to measure the tradeoff of accuracy and convergence.}
        \label{fig:convergence-comparison-2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{src/figures/time_results.pdf}
        \caption{Computation cost per gradient step of varying problem size $d_y$. We vary $d_y$ from 100 to 1000 to measure the computation cost.}
        \label{fig:computation-comparison}
    \end{subfigure}
    \caption{We run \cref{alg: OIGRM} using \cref{alg:inexact-gradient-oracle} on the bilevel optimization in the toy example in \cref{eqn:experiment-bilevel-optimization} with $d_x = 100$, $d_y = 200$, $n_{\text{const}} = d_y / 5$, and accuracy $\alpha = 0.1$. \cref{fig:convergence-comparison}, \cref{fig:convergence-comparison-2}, \cref{fig:computation-comparison} vary \# of iterations, gradient exactness $\alpha$, and $d_y$, respectively, to compare the performance under different settings.}
    % Figure~\ref{fig:convergence-comparison} shows that \cref{alg: OIGRM} converges in the same rate as CvxpyLayer, while the gradient errors at each iteration are plotted in the colorful bars and are mostly below $\alpha = 0.1$ as guaranteed. Figure~\ref{fig:convergence-comparison-2} shows the convergence under different gradient inexactness $\alpha$. Figure~\ref{fig:computation-comparison} shows the computation cost of both methods under different lower level problem size $d_y$.}
    \label{fig:three graphs}
\end{figure}

We  generate instances of the following constrained bilevel optimization problem: 
\begin{align*}\numberthis\label[prob]{eqn:experiment-bilevel-optimization}
     & \mbox{min}_{x} ~  c^\top y^* + 0.01 \norm{x}^2 + 0.01 \norm{y^*}^2 ~\text{ s.t. } ~ y^* = \argmin\nolimits_{y: h(x,y) \leq 0} \frac{1}{2} y^\top Q y + x^\top P y, 
\end{align*}
% \begin{align}\label{}
%     \min\nolimits_{x} \quad & \\
%     \text{s.t.} \quad & \nonumber
% \end{align}
where $h(x,y) = A y - b$ is a $d_h$-dim linear constraint. The PSD matrix $Q \in \reals^{d_y \times d_y}$, $c \in \reals^{d_y}$, $P \in \reals^{d_x \times d_y}$, and constraints $A \in \reals^{d_h \times d_y}$, $b \in \reals^{d_h}$ are randomly generated from normal distributions (cf. \cref{appendix:experiment-setup}).
We compare \cref{alg: OIGRM} with a non-fully first-order method using \texttt{cvxpyLayer}~\cite{agrawal2019differentiable}. Both algorithms use Adam~\cite{kingma2014adam} to control the learning rate, and are averaged over 10 random seeds.

% \paragraph{Convergence and computation comparisons:} 
\looseness=-1\cref{fig:convergence-comparison} shows that  
% compares the convergence of both methods. We can see that 
both the algorithms converge to the same optimal solution at the same rate. Simultaneously, the colorful bars represent the gradient differences between two methods, showing the inexactness of our gradients.
\cref{fig:convergence-comparison-2} additionally varies this inexactness to demonstrate its impact on convergence with standard deviation plotted. 
\cref{fig:computation-comparison} compares the computation costs for different lower-level problem sizes. Our fully first-order method significantly outperforms, in computation cost, the non-fully first-order method implemented using differentiable optimization method. 
The implementation can be found in \url{https://github.com/guaguakai/constrained-bilevel-optimization}.
% in computation cost.



==> backup_src/inequalitySetting-gradient-approximation.tex <==
\section{Inequality constraints: constructing the inexact gradient oracle}\label{sec:inequality-bilevel}

Computing a stationary point of $F$ of \cref{prob:ineq} via any first-order method would require: %
\begin{align}\label{eqn:second-order-method}
    \nabla F(x) = \nabla_x f(x,y^*) + \left(\tfrac{ dy^*(x)}{d x}\right)^\top \nabla_y f(x,y^*),
\end{align}
for which the key challenge lies in computing  ${d y^*(x)}/{d x}$. This requires differentiating through an argmin operator, 
which typically requires second-order derivatives.  
Instead, here we 
differentiate (using the implicit function theorem) through the KKT conditions describing $y^*(x)$
and get: 
\begin{align}\label{eqn:kkt-system}
\begin{bmatrix}
\nabla^2_{yy} g + (\lambda^*)^\top \nabla_{yy}^2 h & \nabla_y h_\mathcal{I}^\top \\
\text{diag}(\lambda^*_\mathcal{I}) \nabla_y h_\mathcal{I} & 0
\end{bmatrix}
\begin{bmatrix}
    \frac{d y^*(x)}{d x} \\
    \frac{d \lambda^*_\mathcal{I}(x)}{d x}
\end{bmatrix}
= 
-
\begin{bmatrix}
    \nabla^2_{yx} g + (\lambda^*)^\top \nabla_{yx}^2 h \\
    \text{diag}(\lambda^*_\mathcal{I}) \nabla_x h_\mathcal{I}
\end{bmatrix}
\end{align}
where given $x$, we assume efficient access to the optimal dual solution $\lambda^*(x)$ of the LL problem in \cref{prob:ineq}. In \cref{eqn:kkt-system}, we use $\mathcal{I} \coloneqq \{i \in [d_h]: h_i(x,y) = 0, \lambda^*_i > 0 \}$ to denote the set of active constraints with non-zero dual solution, with
$h_\mathcal{I} \coloneqq [h_i]_{i \in \mathcal{I}}$ and $\lambda^*_{\mathcal{I}} \coloneqq [\lambda^*_i]_{i \in \mathcal{I}}$ being the constraints and dual variables, respectively,  corresponding to $\mathcal{I}$.  
% (cf. \cref{sec:inactive-constraints-in-differentiable-optimization} for details). 
% For simplicity of exposition, here we assume the active constraint set $\mathcal{I}$ to be exactly specified, which may not hold in practice (cf. \cref{appendix:misspecified-active-constraint-set}).

Observe that as currently stated, \cref{eqn:kkt-system} leads to a second-order computation of ${dy^*(x)}/{dx}$.
In the rest of the section, we provide a fully first-order {approximate} hypergradient oracle by constructing an equivalent reformulation of \cref{prob:ineq} using a penalty function.
% (with two different penalties). 

\subsection{Reformulation via the penalty method}
We begin by reformulating \cref{prob:ineq} into a single level constrained optimization problem:
\begin{align}\label{eqn:inequality_reformulation}
    \text{minimize}_{x,y} ~ f(x,y)  \text{ subject to}
    ~\begin{cases}
        g(x,y) + (\lambda^*(x))^\top h(x,y) \leq g^*(x) \\ 
        h(x,y) \leq 0
    \end{cases},
\end{align}
where $g^*(x)  \coloneqq \min_{y: h(x,y) \leq 0} g(x,y) = g(x,y^*(x))$ and $\lambda^*(x)$ is the optimal dual solution. The equivalence of this reformulation to  \cref{prob:ineq} is spelled out in \cref{appendix:reformulation-equivalence}. 
% For a given $x$, evaluating \cref{eqn:inequality_reformulation} requires computing the primal solution $y^*(x)$ and the corresponding dual solution $\lambda^*(x)$ to the lower level problem.\pswt{commenting out because the sentence was not implying anything that was being used later}
% Given the reformulated problem in \cref{eqn:inequality_reformulation}, 
From \cref{eqn:inequality_reformulation}, we  define the following penalty function, crucial to our analysis:
\begin{align}
    \mathcal{L}_{\lambda^*, \boldsymbol{\alpha}}(x,y) = f(x,y) + \alpha_1 \left( g(x,y) + (\lambda^*)^\top h(x,y) - g^*(x)  \right) + \frac{\alpha_2}{2} \norm{h_\mathcal{I}(x,y)}^2, \numberthis\label{eqn:penalty-lagrangian}
\end{align}
where $\boldsymbol{\alpha} = [\alpha_1, \alpha_2] \geq 0$ are the penalty parameters.
Notably, we can compute its derivative with respect to $x$ of \cref{eqn:penalty-lagrangian} in a fully first-order fashion by the following expression: 
\begin{align*}
    \nabla_x \mathcal{L}_{\lambda^*, \boldsymbol{\alpha}}(x, y) = \nabla_x f(x,y) \! + \! \alpha_1 (\nabla_x g(x,y) \! + \! \nabla_x h(x,y)^\top \lambda^* \! - \! \nabla_x g^*(x) ) \! + \! \alpha_2 \nabla_x h_\mathcal{I}(x,y)^\top h_\mathcal{I}(x,y).
    % \label{eqn:lagrangian-derivative}
\end{align*}
To give some intuition for our choice of penalties in \cref{{eqn:penalty-lagrangian}}, we note that  the two constraints in \cref{eqn:inequality_reformulation} behave quite differently.
The first constraint $g(x,y) + \lambda^*(x)^\top h(x,y)  \leq g^*(x)$ is one-sided, i.e., can only be violated or met, and hence just needs a penalty parameter $\alpha_1$ to weight the ``violation''.
As to the second constraint $h(x,y) \leq 0$, it can be arbitrary. To allow for such a ``two-sided'' constraint, we penalize only the active constraints $\mathcal{I}$, i.e., we use $\norm{h_{\mathcal{I}}(x,y)}^2$ to penalize deviation.


Next, we define the optimal solutions to the penalty function optimization by:
\begin{align*}
    y_{\lambda^*, \boldsymbol{\alpha}}^*(x) := \arg\min\nolimits_{y} \mathcal{L}_{\lambda^*, \boldsymbol{\alpha}}(x,y).\numberthis\label{eq:def_y_lambda_star} 
\end{align*}
% where $S$ is the set of active constraints in the lower level optimization problem. This additional constraint ensures that inactive constraints in the lower level problem stay satisfied, while only the active constraints can be violated. This design choice plays an important role in the later analysis.
% , and $S$ is the set of active constraints with non-zero dual solution in the lower-level problem. \pswt{already defined in the previous paragraph; removed y* and lambda because they are also already defined}
% , and the penalty function $p(x,y) = h(x,y) - h(x,y^*) - \nabla_y h(x,y^*)^\top (y - y^*) \geq 0 ~\forall y$.
We now show that this minimizer is close to the optimal solution of the LL problem, while suffering only a small constraint violation. 
\begin{restatable}[]{lemma}{solutionApproximation}\label{thm:solution-bound}
Given any $x$, the corresponding dual solution $\lambda^*(x)$,  primal solution $y^*(x)$ of the lower optimization problem in \cref{prob:ineq}, and $y_{\lambda^*, \boldsymbol{\alpha}}^*(x)$ as in \cref{{eq:def_y_lambda_star}}, satisfy:
\begin{align}\label{eqn:solution-bound}
    \norm{y_{\lambda^*, \boldsymbol{\alpha}}^*(x) - y^*(x)} \leq O(\alpha_1^{-1}) \text{~~and~~} \norm{h_\mathcal{I}(x,y_{\lambda^*, \boldsymbol{\alpha}}^*(x))} \leq O(\alpha_1^{-1/2} \alpha_2^{-1/2}).
\end{align}
\end{restatable}
The proof of \cref{thm:solution-bound} is based on the Lipschitzness of $f$ and strong convexity of $g$ for sufficiently large $\alpha_1$.
The aforementioned constraint violation bound on $h_\mathcal{I}(x,y)$ is later used in \cref{thm:diff_in_hypergrad_and_gradLagr} to bound the inexactness of our proposed gradient oracle.
% that involves constraint violation. 

\subsection{Main result: approximating the hypergradient}
The main export of this section is the following bound on the approximation of  the hypergradient. This, together with the bounds in 
% Based on the penalty function $\mathcal{L}_{\lambda^*,\alpha}(x,y)$ and bounds on $y^*_{\lambda^*,\alpha}$ in 
\cref{thm:solution-bound}, validate our use of the penalty function in \cref{eqn:penalty-lagrangian}. 
\begin{restatable}[]{lemma}{gradientApproximation}\label{thm:diff_in_hypergrad_and_gradLagr}
Consider $F$ as in \cref{{prob:ineq}},   $\mathcal{L}$ as in  \cref{{eqn:penalty-lagrangian}},  a fixed $x$, and $y_{\lambda^*, \boldsymbol{\alpha}}^*$ as in \cref{{eq:def_y_lambda_star}}. Then under \cref{assumption:linEq_smoothness,item:assumption_safe_constraints}, we have: 
\begin{align*}%\label{eqn:gradient-approximation}
   & \norm{\nabla F(x) - \nabla_x \mathcal{L}_{\lambda^*, \boldsymbol{\alpha}}(x, y_{\lambda^*, \boldsymbol{\alpha}}^*)} \leq O({\alpha_1^{-1}}) + O({\alpha_1^{-1/2}\alpha_2^{-1/2}}) + O({\alpha_1^{1/2}}{\alpha_2^{-1/2}}) + O({\alpha_1^{-3/2}}{\alpha_2^{1/2}}).
\end{align*}
\end{restatable}
The proof can be found in \cref{appendix:proof-of-inexact-gradient}. 
With this hypergradient approximation guarantee, we design \cref{alg:inexact-gradient-oracle} to compute an inexact gradient oracle for the hyperobjective $F$.
\begin{algorithm}[h]\caption{Inexact Gradient Oracle for General Inequality Constraints}\label{alg:inexact-gradient-oracle}
\begin{algorithmic}[1]
\State \textbf{Input:}
Upper level variable $x$, accuracy $\alpha$, penalty parameters $\alpha_1 = {\alpha^{-2}}, \alpha_2 = {\alpha^{-4}}$.
\State Compute $y^*$, $\lambda^*$, and active constraints $\mathcal{I}$ of the constrained LL problem $\min_{y: h(x,y) \leq 0} g(x,y)$. \label{line:inner-optimization-problem} 
\State Define penalty function $\mathcal{L}_{\lambda^*, \boldsymbol{\alpha}}(x,y)$ by ~\cref{eqn:penalty-lagrangian}
\State Compute the minimizer $y^*_{\lambda^*, \boldsymbol{\alpha}} = \arg\min\nolimits_{y} \mathcal{L}_{\lambda^*, \boldsymbol{\alpha}}(x,y)$ (as in ~\cref{eq:def_y_lambda_star}).\label{line:lagrangian-optimization}
\State \textbf{Output:} $\widetilde{\nabla} F \coloneqq \nabla_x \mathcal{L}_{\lambda^*, \boldsymbol{\alpha}}(x,y^*_{\lambda^*, \boldsymbol{\alpha}})$.
\end{algorithmic}
\end{algorithm}

==> backup_src/inequalitySetting-inexact-grad-oracle-cost.tex <==
\begin{restatable}[]{theorem}{computationCostInequality}\label{thm:cost_of_computing_ystar_gammastar_inequality}
    Given any accuracy parameter $\alpha > 0$, \cref{alg:inexact-gradient-oracle} outputs $\widetilde{\nabla}_x F(x)$ such that $\|\widetilde{\nabla} F(x) - \nabla F(x)\| \leq \alpha$ within $\widetilde{O}({\alpha^{-1}})$ gradient oracle evaluations. 
\end{restatable}
The full proof of this result may be found in \cref{appendix:cost_of_computing_ystar_gammastar_inequality}.   


% \begin{proof}[Proof sketch (full proof in \cref{appendix:cost_of_computing_ystar_gammastar_inequality})]
%     By choosing 
%     the penalty parameters $\alpha_1 = \alpha^{-2}$ and $\alpha_2 = \alpha^{-4}$, ~\cref{thm:diff_in_hypergrad_and_gradLagr} guarantees the inexactness of the gradient oracle is upper bounded by $O(\alpha)$.
    
% % \jz{Please remove the discussion on the LL problem from the proof. We are using the exact oracle here.}    
% % (1) For the LL problem in \cref{alg:inexact-gradient-oracle}, we apply the primal-dual gradient descent result from ~\cite{du2019linear} to get a linear convergence of the dual solution, i.e., find a dual solution $\lambda$ with $\norm{\lambda - \lambda^*} \leq \alpha$ in $O(\log \frac{1}{\alpha}) < O(\alpha^{-1})$ iterations. 
%     % (2) 
%     For the penalty minimization, the objective $\mathcal{L}$ is strongly convex but with a  condition number $\kappa_\mathcal{L} = O(\alpha^{-2})$ due to strong convexity $O(\alpha_1 \mu_g) = O( {\alpha^{-2} \mu_g})$ and smoothness $O(\alpha_2 C_h) = O(\alpha^{-4})$. This leads to $O(\sqrt{\kappa_\mathcal{L}} \log \| \alpha^{-1} \|) = \widetilde{O}({\alpha^{-1}})$ iterations to converge to $\alpha$ accuracy using standard accelerated methods.
%     Using these error bounds, we can bound the error propagation of inexact solution $y^*_{\lambda,\alpha}$ and inexact gradient oracle using \cref{thm:diff_in_hypergrad_and_gradLagr} by total error $O(\alpha)$.
%     Therefore, putting all together, we  need only  $O(\alpha^{-1})$ oracle calls and can maintain $O(\alpha)$ inexactness.
% \end{proof}

==> backup_src/intro.tex <==
\section{Introduction}\label{sec:introduction}
Bilevel optimization~\cite{bracken1973mathematical, colson2007overview,bard2013practical,sinha2017review}, an important problem in optimization, is defined as follows:
\begin{align*}\numberthis\label[prob]{prob:general-constraints}
     \mbox{minimize}_{x\in \mathcal{X}} ~ F(x) \coloneqq f(x, \ystar(x)) \text{ subject to } ~\ystar(x)\in \arg\min\nolimits_{y\in S(x)} g(x, y).
\end{align*}
Here, the value of the upper-level problem at any point $x$ depends on the solution of the lower-level problem. This framework has recently found numerous applications in meta-learning~\cite{ snell2017prototypical, bertinetto2018meta, rajeswaran2019meta, ji2020convergence}, hyperparameter optimization~\cite{franceschi2018bilevel, shaban2019truncated, feurer2019hyperparameter}, and 
reinforcement learning~\cite{konda1999actor, sutton2018reinforcement, hong2020two,zhang2020bi}.
Its growing importance has spurred increasing efforts towards designing computationally efficient algorithms for it. 

As demonstrated by \cite{ghadimi2018approximation}, a key computational step in algorithms for bilevel optimization is estimating ${dy^*(x)}/{dx}$, the gradient of the lower-level solution. This gradient estimation problem has been extensively studied in differentiable optimization~\cite{amos2017optnet,agrawal2019differentiable} by applying the implicit function theorem to the KKT system of the given problem~\cite{donti2017task,wilder2019melding,kotary2021end,lee2019meta,tang2022pyepo,bai2019deep}.
However, this technique typically entails computing (or estimating) second-order derivatives, which can be prohibitive in high dimensions~\cite{mehra2021penalty, ji2021bilevel,wang2021learning}.

Recently, \cite{liu2022bome} made a big leap forward towards addressing this computational bottleneck.  
Restricting themselves to the class of unconstrained bilevel optimization, they proposed a fully first-order method with finite-time stationarity guarantees. While a remarkable breakthrough,  \cite{liu2022bome} does not directly extend to the important setting of \textit{constrained} bilevel optimization. This motivates the question: 
\begin{quote}
\centering
    \emph{Can we develop a  first-order algorithm for constrained bilevel optimization?}
\end{quote}
Besides being natural from the viewpoint of complexity theory, this question is well-grounded
in applications such as 
% Stackelberg models~\cite{simaan1973stackelberg,paruchuri2008playing,chu2014integrated}, 
mechanism design~\cite{wang2022coordinating,dutting2021optimal},  
% urban planning~\cite{miao2010modeling,kang2010bilevel},
resource allocation~\cite{xu2013bilevel,gutjahr2016bi,zhang2010bilevel,fathollahi2022bi}, and decision-making under uncertainty~\cite{elmachtoub2022smart,munoz2022bilevel,wilder2019melding}. 
% In this paper, we  focus on bilevel programs with linear constraints in the lower-level problem; this problem class often arises  in adversarial training, decentralized meta learning, and sensor networks~(see \cite{khanduri2023linearly} and the discussion therein).
Our primary contribution is \textit{an affirmative answer to the highlighted question for bilevel programs with linear constraints}, an important problem class often arising in adversarial training, decentralized meta learning, and sensor networks~(see \cite{khanduri2023linearly}). 
While there have been some other recent works~\cite{khanduri2023linearly, yao2024constrained, lu2024firstorder} on this problem, our work is  first-order (as opposed to \cite{khanduri2023linearly}) and offers, in our view, a stronger guarantee on stationarity (compared to \cite{yao2024constrained, lu2024firstorder})--- cf. \cref{sec:related_work}. 
% We now summarize our contributions.

\subsection{Our contributions}\label{sec:introduction_main_results}
We provide first-order algorithms (with associated finite-time convergence guarantees) for linearly constrained bilevel programs (\cref{prob:general-constraints}). By ``first-order'', we mean that we use only zeroth and first-order oracle access to $f$ and $g$.  Our  assumptions for each of our contributions are  in \cref{{sec:differentiable-optimization}}. 
\begin{description}[style=unboxed,leftmargin=0cm, itemsep=.5em, parsep=.3em]

\item[{(1)}] \textbf{Linear equality constraints.} As our first contribution, we design first-order algorithms for solving \cref{prob:general-constraints} where the lower-level constraint set $S(x):=\left\{y:Ax-By-b=0\right\}$  comprises linear equality constraints,  and $\mathcal{X}$ a convex compact set. 
With appropriate regularity assumptions on $f$ and $g$, we show in this case smoothness in $x$ of the hyperobjective $F$. Inspired by ideas from \citet{kwon2023fully}, we use implicit differentiation of the KKT matrix of a slightly perturbed version of the lower-level problem to design a first-order approximation to $\nabla F$. Constructing our first-order approximation entails solving a strongly convex optimization problem on affine constraints, which can be done efficiently. With this inexact gradient oracle in hand,  we then run projected gradient descent, which converges in $\widetilde{O}(\epsilon^{-2})$ iterations for smooth functions. 

\begin{theorem}[Informal; cf. \cref{thm:lineq-cost}]
\label{thm:lineq-cost-inf}
    Given \cref{prob:general-constraints} with linear equality constraints $S(x)\coloneqq\left\{y:Ax-By-b=0\right\}$ and $\mathcal{X}$ a convex compact set, under regularity assumptions on $f$ and $g$ (\cref{assumption:linEq_smoothness,assumption:eq}), there exists an algorithm, which in $\widetilde{O}(\epsilon^{-2})$  oracle calls to $f$ and $g$, converges to an $\epsilon$-stationary point of $F$. 
\end{theorem}
For  linear equality constrained bilevel optimization, this is the first  first-order result attaining $\epsilon$-stationarity of $F$ with assumptions solely on the constituent functions $f$ and $g$ and none on $F$ --- cf. \cref{sec:related_work} for a discussion of the results of \citet{khanduri2023linearly} for this setting. 

\item [{(2)}] \textbf{Linear inequality constraints.} Next, we provide first-order algorithms for solving \cref{prob:general-constraints} where the lower-level constraint set $S(x):=\left\{y:Ax-By-b\leq0\right\}$  comprises linear inequality constraints, and the upper-level variable is unconstrained. 

Our measure of convergence of  algorithms in this case is that of $(\delta,\epsilon)$-stationarity~\cite{goldstein1977optimization}: for a Lipschitz function, we say that a point $x$ is $(\delta,\epsilon)$-stationary if within a $\delta$-ball around $x$ there exists a convex combination of subgradients of the function with norm at most $\epsilon$ (cf. \cref{def:GoldsteinDeltaEpsStationary}). 

\looseness=-1
To motivate this notion of convergence, we note that the hyperobjective $F$ (in \cref{prob:general-constraints}) as a function of $x$ could be nonsmooth and nonconvex (and Lipschitz, as  we later prove). Minimizing such a function in general is known to be intractable~\cite{nemirovskij1983problem}, necessitating local notions of stationarity. Indeed, not only is it impossible to attain $\epsilon$-stationarity in finite time~\cite{zhang2020complexity}, even getting \textit{near} an
approximate stationary point of an arbitrary Lipschitz function is impossible unless
the number of queries is exponential in the dimension~\cite{kornowski2022oracle}. Consequently, for this function class, $(\delta, \epsilon)$-stationarity has recently emerged~\cite{zhang2020complexity} to be a natural and algorithmically tractable notion of stationarity. We give the following guarantee under  regularity assumptions on $f$ and $g$. 


\begin{theorem}[Informal; \cref{{{thm:izo_complete_guarantees}}}]\label{thm:informal_izo_full}
 Consider \cref{prob:general-constraints} with linear inequality constraints $S(x)\coloneqq\left\{y:Ax-By-b\leq 0\right\}$. Under mild  assumptions on $f$ and $g$ (\cref{assumption:linEq_smoothness}) and the lower-level primal solution $y^*$ (\cref{assumption:ineq_mild}), there exists an algorithm, which converges to a $(\delta, \epsilon)$-stationary point of $F$ in $\widetilde{O}(d\delta^{-1}\epsilon^{-3})$  oracle calls to $f$ and $g$, where $d$ is the upper-level variable dimension.  
\end{theorem}

To the best of our knowledge, this is the first result to offer a  first-order finite-time stationarity guarantee on the hyperobjective for 
linear inequality constrained bilevel optimization (cf. \cref{sec:related_work} for a discussion of related work~\cite{khanduri2023linearly, yao2024constrained, lu2024firstorder}).
We obtain our guarantee in \cref{thm:informal_izo_full} by first invoking a result by \citet{zhang2022solving} to obtain inexact hyperobjective values of $F$ using only $\widetilde{O}(1)$ oracle calls to $f$ and $g$. We also show (\cref{{lem:LipscConstrBilevel}}) that this hyperobjective $F$ is Lipschitz. We then employ our inexact zeroth-order oracle for  $F$ in \cref{alg: IZO} designed to minimize Lipschitz nonsmooth nonconvex functions (in particular, $F$), with the following convergence guarantee. 

\begin{theorem}[see \cref{{thm: Lipschitz-min-with-inexact-zero-oracle}}]\looseness=-1
Given $L$-Lipschitz $F:\reals^d\to\reals$ 
and  $|\widetilde{F}(\cdot)-F(\cdot)|\leq\epsilon$,  there exists an algorithm, which, 
 in 
$\widetilde{O}(d\delta^{-1}\epsilon^{-3})$
calls to $\tF(\cdot)$, outputs 
 $x^{\out}$ with $\E[\mathrm{dist}(0,{\partial}_\delta F(x^{\out}))]\leq2\epsilon$.  

\end{theorem}

While such algorithms using  \emph{exact} zeroth-order access already exist~\cite{kornowski2024algorithm}, extending them to the inexact gradient  setting is non-trivial; we leverage recent ideas connecting online learning to nonsmooth nonconvex optimization by \citet{cutkosky2023optimal} (cf. \cref{{sec:nonsmooth}}).


\item[{(3)}] \textbf{Linear inequality under assumptions on dual variable access.}
 For the {inequality} setting (i.e., \cref{prob:general-constraints} with the lower-level constraint set $S(x):=\left\{y:Ax-By-b\leq0\right\}$), we obtain dimension-free rates under an additional assumption  (\cref{item:assumption_safe_constraints}) on oracle access to the optimal dual variable $\lambda^*$ of the lower-level problem. We are not aware of a method to obtain this dual variable in a first-order fashion (though in practice, highly accurate approximations to $\lambda^*$ are readily available), hence the need for imposing this assumption. We believe that removing this assumption and obtaining dimension-free first-order rates in this setting would be an important direction for future work. Our guarantee for this setting is summarized below. 

 
\begin{theorem}[Informal; \cref{thm:Lipschitz-min-with-inexact-grad-oracle} combined with \cref{thm:cost_of_computing_ystar_gammastar_inequality}]\label{thm:linIneqInformal}
    Consider \cref{prob:general-constraints} with linear inequality constraints $S(x)\coloneqq\left\{y:Ax-By-b\leq0\right\}$ and unconstrained upper-level variable. Under mild regularity assumptions on $f$ and $g$ (\cref{assumption:linEq_smoothness}), on $y^*$ (\cref{assumption:ineq_mild}), and assuming oracle access to the optimal dual variable $\lambda^*$ (\cref{item:assumption_safe_constraints}), there exists an algorithm, which in $\widetilde{O}(\delta^{-1}\epsilon^{-4})$ oracle calls to $f$ and $g$ converges to a $(\delta, \epsilon)$-stationary point for $F$. 
\end{theorem} 

We obtain this result  by first reformulating  \cref{{prob:ineq}} via the penalty method and constructing an
inexact gradient oracle for the hyperobjective $F$ (cf. \cref{sec:inequality-bilevel}). We then employ this inexact gradient oracle within {an algorithm (\cref{{alg: OIGRM}}) designed to minimize Lipschitz nonsmooth nonconvex functions}
(in particular, $F$), with the following convergence guarantee.
\begin{theorem}[Informal; \cref{{thm:Lipschitz-min-with-inexact-grad-oracle}}]\label{thm:informal_FO_inexact_ncns}
    Given Lipschitz $F:\reals^d\to\reals$ 
and $\|\widetilde{\nabla} F(\cdot)-\nabla F(\cdot)\|\leq\epsilon$,
 there exists an algorithm that, in 
$T=O(\delta^{-1}\epsilon^{-3})$
calls to $\widetilde{\nabla}F$,
outputs a $(\delta,2\epsilon)$-stationary point of $F$.
\end{theorem} 

Our  \cref{alg: OIGRM} is essentially a ``first-order'' version of  \cref{alg: IZO}. Similar to \cref{alg: IZO}, despite the existence of algorithms with these guarantees with access to exact gradients~\cite{davis2022gradient}, their extensions to the \emph{inexact} gradient setting are not trivial and also make use of the new framework of \citet{cutkosky2023optimal}.  We believe our analysis for this general task can be of independent interest to the broader optimization community.  
Lastly, we also use a more implementation-friendly variant of \cref{alg: OIGRM} (with slightly worse theoretical guarantees)  in numerical experiments. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{description}

==> backup_src/linearEquality.tex <==
\section{Lower-level problem with linear equality constraint}\label{sec:equality-bilevel}
\looseness=-1We first obtain improved results for the  setting of bilevel programs with linear \textit{equality} constraints in the lower-level problem. Our formal problem statement is:   
\begin{align*}\numberthis\label[prob]{prob:lin-eq}
     & \mbox{minimize}_{x\in \mathcal{X}} ~ F(x) \coloneqq f(x, \ystar(x))~\text{ subject to } ~\ystar(x)\in \arg\min\nolimits_{y: h(x, y) = 0} g(x, y), 
\end{align*}
where $f$, $g$, $h(x,y)\coloneqq Ax-By-b$, and $\mathcal{X}$ satisfy 
\cref{assumption:linEq_smoothness,assumption:eq}.
\looseness=-1The previous best result on \cref{{prob:lin-eq}}  providing finite-time $\epsilon$-stationarity guarantees, by ~\citet{khanduri2023linearly}, required certain regularity assumptions on $F$ as well as Hessian computations. In contrast, our finite-time guarantees \emph{require assumptions only on $f$ and $g$, not on $F$};
indeed, in our work, these desirable properties of $F$ are naturally implied by our analysis. 
Specifically, our key insight is that the hypergradient $\grad F(x):=\grad_{x}f(x,y^{*})+\left(\tfrac{d y^*(x)}{dx}\right)^\top\grad_{y}f(x,y^{*})$ for  \cref{{prob:lin-eq}} is Lipschitz-continuous and  admits an easily computable --- yet highly accurate --- finite-difference approximation. Therefore, $O(\epsilon^{-2})$ iterations of gradient descent  on $F$ with this finite-difference gradient proxy  yield an $\epsilon$-stationary point. 

Specifically, for any fixed $x\in \mathcal{X}$, our proposed finite-difference gradient proxy approximating the non-trivial-to-compute component $\left(\tfrac{d y^*(x)}{dx}\right)^\top\grad_{y}f(x,y^{*})$ of the hypergradient is given
by 
 \[ v_x := {\frac{\nabla_{x}[g(x,\ystardel)+\langle\lamdeltar, h(x,\ystar)\rangle]-\nabla_{x}[g(x,y^{*})+\langle\lamstar, h(x,y^{*})\rangle]}{\delta}
 \numberthis\label{eq:part-hypergrad-approx-lin-eq},}\]
where $(\ydelstar,\lamdeltar)$ are the primal and dual solutions to the
 perturbed lower-level problem:
\begin{align}\label{eq:lower_perturb}
    & \ydelstar \coloneqq \arg\min\nolimits_{y: h(x,y) = 0} ~g(x,y)+\delta f(x,y).
\end{align} We show in \cref{{lem:lineq-finitediff-equals-gradf}} that $v$ in \cref{eq:part-hypergrad-approx-lin-eq} approximates $\left(\tfrac{d y^*(x)}{dx}\right)^\top\grad_{y}f(x,y^{*})$ up to an $O(\delta)$-additive error, implying the gradient oracle construction outlined in the pseudocode presented in 
\cref{alg:LE-inexact-gradient-oracle}. Our full implementable algorithm for solving \cref{prob:lin-eq} is displayed in \cref{{alg:LE-full-alg}}.

\begin{algorithm}[h]\caption{Inexact Gradient Oracle for Bilevel Program with Linear Equality Constraint}\label{alg:LE-inexact-gradient-oracle}
\begin{algorithmic}[1]
\State \textbf{Input:}
Current $x$, accuracy $\epsilon$, perturbation $\delta = \epsilon^2$.
\State Compute $y^*$ (as in \cref{prob:lin-eq}) and corresponding optimal dual $\lamstar$ (as in \cref{eqs:kkt-lin-eq})\label{line:LEQ-first}
\State Compute $\ystardel$ (as in \cref{eq:lower_perturb}) and and corresponding optimal dual $\lamdeltar$ (as in \cref{eqs:lineq-kkt-perturbed}) \label{line:LEQ-second} 
\State Compute $v_x$ as in \cref{eq:part-hypergrad-approx-lin-eq} \Comment{Approximates $\left({d y^{*}(x)}/{d x}\right)^\top\nabla_{y}f(x,y^{*})$}
\State \textbf{Output:} $\widetilde{\nabla} F = v_x + \nabla_x f(x, y^*)$
\end{algorithmic}
\end{algorithm}

Notice that the finite-difference term in \cref{{eq:part-hypergrad-approx-lin-eq}} avoids differentiating through the implicit function $y^*$. Instead, all we need to evaluate it are the values of $(y^*,\lambda^*,\ydelstar,\lamdeltar)$ (and gradients of $g$ and $h$). Since $(y^*,\lambda^*)$ are solutions to a smooth strongly convex linearly constrained  problem, they can be approximated
at a linear rate. Similarly, since the approximation error in \cref{eq:part-hypergrad-approx-lin-eq}  is proportional to $\delta$ (cf. \cref{{lem:lineq-finitediff-equals-gradf}}), a  small enough $\delta$ in the perturbed objective $ g+\delta f$ in \cref{eq:lower_perturb} ensures that it is dominated by the strongly convex and smooth $g$, whereby accurate approximates to $(y_\delta^*,\lambda_\delta^*)$ can also be readily obtained. Putting it all together, the proposed finite-difference hypergradient proxy in \cref{eq:part-hypergrad-approx-lin-eq} is  efficiently computable, yielding the following guarantee. 
\begin{restatable}{theorem}{linEqFullCost}\label{thm:lineq-cost}
    Consider  \cref{prob:lin-eq} under \cref{assumption:linEq_smoothness}, and let $\kappa=C_g/\mu_g$ be the condition number of $g$. Then \cref{alg:LE-full-alg}  finds an $\epsilon$-stationary point (in terms of gradient mapping, see \cref{eq:gradient-mapping}) after $T=\widetilde{O}(C_F (F(x_0)-\inf F)\sqrt{\kappa}\epsilon^{-2})$  oracle calls to $f$ and $g$, where $C_F:= 2(L_f +C_f+C_g)C_H^3 S_g (L_g +\|A\|)^2$ is the smoothness constant of the hyperobjective $F$.
\end{restatable}  
We now sketch the proof of \cref{thm:lineq-cost}. The complete proofs may be found in \cref{{sec:appendix_linear_equality}}.   

\subsection{Main technical ideas}\label{sec:warmup-lin-eq} 
We briefly outline the two key technical building blocks alluded to above, that together give us  \cref{{thm:lineq-cost}}: the approximation guarantee of our finite-difference gradient proxy (\cref{{eq:part-hypergrad-approx-lin-eq}}) and the smoothness of hyperobjective $F$ (for \cref{{prob:lin-eq}}). The starting point for both these results is the following simple observation obtained by implicitly differentiating, with respect to $x$, the KKT system associated with $y^*=\arg\min_{h(x,y)=0} g(x,y)$ and optimal dual variable $\lamstar$: 
 \[ \begin{bmatrix}\frac{d\ystar(x)}{dx}\\
\frac{d\lamstar(x)}{dx}
\end{bmatrix}= {\begin{bmatrix}\grad^2_{yy}g(x,\ystar) & \nabla_y h(x,y^{*})^{\top}\\
\nabla_y h(x,y^{*}) & 0
\end{bmatrix}^{-1}} \begin{bmatrix}-\nabla^2_{yx}g(x,y^{*})\\
-\nabla_x h(x,\ystar)\end{bmatrix} \numberthis\label{eq:def_matrix_H}\]
The invertibility of the matrix in the preceding equation is proved in  \cref{{cor:nonsingularH}}:
essentially, this invertibility is implied by strong convexity of $g$ and $\grad_y h(x,y^*)=B$ having full row rank. This in conjunction with the compactness of $\mathcal{X}$ implies that the inverse of the matrix is bounded by some constant $C_H$ (cf. \cref{cor:nonsingularH} for details). Our hypergradient approximation guarantee follows: 

\begin{restatable}{lemma}{lemLineqFiniteDiffEqualsGradF}\label{lem:lineq-finitediff-equals-gradf} 
For  \cref{prob:lin-eq}
under \cref{assumption:linEq_smoothness}, with $v_x$ as in \cref{eq:part-hypergrad-approx-lin-eq}, 
the
following holds:
\[
\textstyle{\left\|v_x-\left(\frac{d y^{*}(x)}{d x}\right)^\top\nabla_{y}f(x,y^{*})\right\|\leq O(C_F \delta).}
\]
\end{restatable}
\begin{proof}[Proof sketch; see \cref{{sec:appendix_linear_equality}}]
    The main idea is that the two terms being compared are essentially the same by the implicit function theorem. First, we  use the expression for $\tfrac{dy^*(x)}{dx}$ from \cref{eq:def_matrix_H}:
\begin{align*}
\left(\frac{d y^{*}(x)}{d x}\right)^\top\nabla_{y}f(x,y^{*})
&=\begin{bmatrix}-\nabla^2_{yx} g(x,y^{*})\\
-\nabla_x h(x,\ystar)
\end{bmatrix}^\top\begin{bmatrix}\nabla^2_{yy} g(x,y^{*}) & \nabla_y h(x,y^{*})^{\top}\\
\nabla_y h(x,y^{*}) & 0
\end{bmatrix}^{-1}\begin{bmatrix}\nabla_{y}f(x,y^{*}) \\ 0\end{bmatrix}.
\end{align*} We now examine $v_x$. For simplicity of exposition, we instead consider $\lim_{\delta\rightarrow0}\frac{\nabla_{x}[g(x,\ystardel)+\langle\lamdeltar, h(x,y^*)\rangle]-\nabla_{x}[g(x,y^{*})+\langle\lamstar, h(x,y^{*})\rangle]}{\delta},$ which, by the fundamental theorem of calculus and \cref{assumption:eq}
, equals $v_x$ up to an $O(\delta)$-additive error. Note that this expression  is: \[\nabla^2_{xy} g(x,y^*) \frac{d\ydelstar}{d\delta} + \nabla_x h(x,y^*)^\top \frac{d\lamdeltar}{d\delta}.\numberthis\label{eq:LINEQ-lim-findiff}\] Since  $y^*_{\delta}$ is minimizes a strongly convex function over a linear equality constraint \cref{{eq:lower_perturb}}, the reasoning that yields \cref{eq:def_matrix_H} also gives the following, which, when combined with \cref{eq:LINEQ-lim-findiff}, finishes the proof:   
\[
\begin{bmatrix}\frac{d\ydelstar(x)}{d\delta}\\
\frac{d\lamdeltar(x)}{d\delta}
\end{bmatrix}\Bigg|_{\delta=0}=\begin{bmatrix}\nabla^2_{yy} g(x,\ystar) & \nabla_y h(x,\ystar)^{\top}\\
\nabla_y h(x,\ystar) & 0
\end{bmatrix}^{-1}\begin{bmatrix}-\nabla_y f(x,\ystar)\\
0
\end{bmatrix}. \numberthis\label{eq:LINEQ-dystardelta}
\] 
\end{proof}

Having shown the construction of the hypergradient approximation, we now state smoothness of the hyperobjective $F$ (proof in \cref{{sec:appendix_linear_equality}}), crucial to getting our claimed rate. 

\begin{restatable}{lemma}{lemYdelstarLamdelstarSmooth}\label{lem:smoothness_of_ydelstar_lamdelstar}
The solution $y^*$ (as defined in \cref{{prob:lin-eq}}) is $O(C_H \cdot (\gssmooth + \|A\|))$-Lipschitz continuous and $O(C_H^3\cdot\gtsmooth\cdot(\gssmooth+\|A\|)^2)$-smooth as a function
of $x$. Thus the hyper-objective $F$ is gradient-Lipschitz  with a  smoothness constant of $C_F:=O\{ (L_f +C_f+C_g)C_H^3 S_g (L_g +\|A\|)^2\}.$ 
\end{restatable}
% \begin{proof}[Proof sketch; see \cref{{sec:appendix_linear_equality}}]
%  The Lipschitz bound follows by combining \cref{{eq:def_matrix_H}} with the smoothness of $g$ and bound $C_H$ on the matrix inverse therein. Differentiating \cref{{eq:def_matrix_H}} by $x$ yields a linear system with the same matrix;  we repeat this approach to get the  smoothness bound. 
% \end{proof}


==> backup_src/problem-statement.tex <==
\section{Preliminaries}\label{sec:preliminaries}
We follow standard notation (see \Cref{sec:appendix_notation}), with only the following crucial definition stated here.
% since we use it crucially.

\begin{definition}\label{def:GoldsteinDeltaEpsStationary}
 Consider a locally Lipschitz function $f:\reals^d\to\reals$, a point $x\in\reals^d$, and a parameter $\delta>0$. The {Goldstein subdifferential}~\cite{goldstein1977optimization} of $f$ at $x$ is the set
 $\partial_{\delta} f(x):=\mathrm{conv} (\cup_{y\in \mathbb{B}_{\delta}(x)}\partial f(y)),$ where  $\partial f(x)=\mathrm{conv}\left\{\lim_{n\to \infty} \nabla f(x_n): x_n\to x, ~x_n\in \mathrm{dom}(\nabla f)\right\}$ is the Clarke subdifferential~\cite{clarke1981generalized} of $f$ and $\mathbb B_\delta(x)$ denotes the Euclidean ball of radius $\delta$ around $x$.
 A point $x$ is called $(\delta, \epsilon)$-stationary if $\mathrm{dist}(0,\partial_{\delta}f(x))\leq \epsilon$, where $\mathrm{dist}(x,S):=\inf_{y\in S}\|x-y\|$.
\end{definition}



\subsection{Assumptions}\label{sec:differentiable-optimization}
We consider \cref{{prob:general-constraints}} with linear equality constraints (\cref{sec:equality-bilevel}) under \cref{assumption:linEq_smoothness,assumption:eq} and  linear inequality constraints (\cref{sec:inequality-bilevel,sec:nonsmooth}) under \cref{assumption:linEq_smoothness,assumption:ineq_mild,item:assumption_safe_constraints}. 
We assume the upper-level (UL) variable $x\in \reals^{d_x}$,  lower-level (LL) variable $y\in \reals^{d_y}$, and $A\in \reals^{d_h \times d_x}$. 


\begin{assumption}\label{assumption:linEq_smoothness} 
For \cref{prob:general-constraints}, we assume the following for both settings we study: 
\begin{assumpenum}
\compresslist{
\item\label[assum]{item:assumption_upper_level} Upper-level: The objective $f$ is $C_f$-smooth and $L_f$-Lipschitz continuous in $(x,y)$. 
\item \label[assum]{item:assumption_lower_level}Lower-level: The objective $g$ is $C_g$-smooth. Fixing any $x\in\mathcal{X}$, $g(x,\cdot)$ is $\mu_g$-strongly convex.
\item \label[assum]{item:assumption_tangen_space}  We assume that the linear independence constraint qualification (LICQ) condition holds for the LL problem at every $x$ and $y$, i.e., the constraint $h(x,y)\coloneqq Ax-By-b$ has a full row rank $B$.
}
\end{assumpenum}
\end{assumption}

\begin{assumption}\label{assumption:eq}For \cref{prob:lin-eq} (with linear equality constraints), we additionally assume that the set $\mathcal{X}$ is convex and compact, and that the objective $g$ is $S_g$-Hessian smooth, that is, $\norm{\grad^2 g(x,y) -\grad^2 g(\bar x,\bar y)}\leq S_g \norm{(x,y) - (\bar x, \bar y)} \forall x,\bar x \in \mathcal{X}, \text{ and } y, \bar y \in \R^{d_y}.$ 
\end{assumption}

\begin{assumption}\label{assumption:ineq_mild}For \cref{prob:ineq} (with linear inequality constraints), we additionally assume  that $y^*$ is $L_y$-Lipschitz in $x$, where $y^*$ is the LL primal solution $y^*(x), \lambda^*(x) = \arg\max\nolimits_y \min\nolimits_{\beta \geq 0} g(x,y) + \beta^\top h(x,y)$, where $h(x,y)\coloneqq Ax-By-b$. 
\end{assumption}

\begin{assumption}\label{item:assumption_safe_constraints} 
We provide additional results for \cref{prob:ineq}  under additional stronger assumptions stated here: Denote the LL primal and dual solution $y^*(x), \lambda^*(x) = \arg\max\nolimits_y \min\nolimits_{\beta \geq 0} g(x,y) + \beta^\top h(x,y)$, where $h(x,y)\coloneqq Ax-By-b$; then, we  assume exact access to $\lambda^*$ and that $\norm{\lambda^*(x)} \leq R$. 
\end{assumption}

\cref{item:assumption_upper_level,item:assumption_lower_level} are standard in bilevel optimization. 
\cref{{item:assumption_tangen_space}} is the same as the complete recourse assumption in stochastic programming \cite{shapiro2021lectures}, that is, the LL problem is feasible $y$ for every $x\in\R^{d_x}$. \cref{assumption:eq} is used only in the equality case and guarantees smoothness of $F$. \cref{assumption:ineq_mild} is used in the inequality case and implies Lipschitzness of  $F$. We need the stronger assumption in  
\cref{item:assumption_safe_constraints}  for our dimension-free result for the linear inequality case. 

==> neurips2024/checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide algorithms and corresponding theoretical guarantees for all our claims in the abstract. We provide experiments (and relevant code) as claimed.  % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is discussed in \cref{sec:limitation}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The assumptions, theorem statements, and proof sketches are included in the main paper. The full proofs are included in the appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide our full code in the supplemental material, and it can be used to reproduce the experimental results.% \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code is included in the supplemental material and can be used to reproduce the experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide this information in \cref{{appendix:experiment-setup}}.%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}% \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide this in \cref{sec:exp} %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}% \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide this information in \cref{{appendix:experiment-setup}}. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}% \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the research conducted in the paper conforms, in every respect, with the NeurIPS Code of Ethics. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}% \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is no societal impact of this work.% \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}% \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks.% \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{}% \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not use existing assets.% \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release new assets.% \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}% \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No crowdsourcing or research with human subjects is involved. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.% \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> neurips2024/packages.tex <==
% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2024


% ready for submission
% \usepackage[nonatbib]{neurips_2024}

% to compile a preprint version, e.g., for submission to arXiv, add add the
% [preprint] option:
\usepackage[final,nonatbib]{neurips_2024}


% to compile a camera-ready version, add the [final] option, e.g.:
%     \usepackage[final]{neurips_2024}


% to avoid loading the natbib package, add option nonatbib:
%    \usepackage[nonatbib]{neurips_2024}


\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amssymb, amsthm, amsfonts, amsmath, mathtools, thm-restate}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % colors
\usepackage{bbm, bm}
\usepackage{subcaption}

\usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage[noend]{algpseudocode}
\usepackage{varwidth}
\usepackage{tabularx}
\usepackage{makecell}
\usepackage{nicematrix}
\usepackage{pifont}
\usepackage{thm-restate}
\usepackage{enumitem}
\newcommand{\xmark}{\ding{55}}
\usepackage[font=small,labelfont=bf]{caption}
\usepackage{xfrac} %for sfrac

\usepackage[
backref=true,
natbib=true,
% style=trad-alpha,
style=numeric-comp,
% style=authoryear,
giveninits=false, 
maxbibnames = 99, 
maxalphanames=8,
sorting=none
]{biblatex}
\addbibresource{src/reference.bib}

%colours for links 
\usepackage{xcolor}
% \usepackage{url}            % simple URL typesetting

\definecolor{otherlightblue}{RGB}{0, 100, 200}
\definecolor{otherblue}{RGB}{0, 50, 100}
\definecolor{othergreen}{RGB}{60, 120, 0}

\hypersetup{
	colorlinks=true,
	pdfpagemode=UseNone,
	citecolor=othergreen,
	linkcolor=otherlightblue,
	urlcolor=magenta
}




%cleveref loads at the end 
\usepackage[capitalize, nameinlink]{cleveref}
\crefformat{equation}{(#2#1#3)}
% \crefname{equation}{Equation}{Equations}
\crefname{eq}{Equation}{Equations}
\crefname{fact}{Fact}{Facts}
\crefname{lemmma}{Lemma}{Lemmas}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{figure}{Figure}{Figures}
\crefname{defn}{Definition}{Definitions}
\crefname{ineq}{Inequality}{Inequalities}
\crefname{prob}{Problem}{Problems}
\crefname{corollary}{Corollary}{Corollaries}
\creflabelformat{ineq}{#2{\upshape(#1)}#3} 
\crefalias{thm}{theorem}
\Crefname{listfact}{Fact}{Facts}
\newlist{assumpenum}{enumerate}{1} % also creates a counter called 'propenumi'
\setlist[assumpenum]{label=(\roman*), ref=\theproposition(\roman*), leftmargin = 2em, topsep=0em}
\crefalias{assumpenumi}{assumption} 
% \crefformat{prop}{Proposition~#2#1#3}
\crefname{assum}{Assumption}{Assumptions} 
\crefname{assumption}{Assumption}{Assumptions}
\crefname{section}{Section}{Sections}
%%%% nothing below this, cleveref loads at the end!

==> neurips2024/symbols.tex <==
%generic stuff 
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}} % lets us add numbers within \[ \] env. 
\numberwithin{equation}{section}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\innerprod}[2]{\langle#1,#2\rangle}%
\global\long\def\grad{\nabla}%
\global\long\def\del{\delta}%
\global\long\def\half{\frac{1}{2}}%
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\reals}{\mathbb{R}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\tbg}{\widetilde{{g}}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\S}{\mathbb{S}}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{thm}{Theorem}[section]
\newtheorem{claim}[theorem]{Claim}
\newtheorem{defn}[theorem]{Definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{assumption}[theorem]{Assumption}

\providecommand{\definitionname}{Definition}
\providecommand{\theoremname}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}

%paper specific stuff 
\global\long\def\grad{\nabla}%
\newcommand{\ystar}{y^*} 
\global\long\def\ydelstar{y_{\delta}^{*}}%
\global\long\def\ystardel{y_{\delta}^{*}}%
\global\long\def\ysl{y_{\lambda}^{\star}}%
\global\long\def\lamdeltar{\lam_{\delta}^{*}}%
\global\long\def\lam{\lambda}%
\global\long\def\lamstar{\lam^{*}}%
\newcommand{\Leqc}{\mathcal{L}_{\mathrm{eq}}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bw}{\mathbf{w}}

\newcommand{\lamstarsmoothlineq}{C_{\ell}}
\newcommand{\ystarsmoothlineq}{C_y}
\newcommand{\ystarliplineq}{M_y}
\newcommand{\gtsmooth}{S_g} %third order smoothness 
\newcommand{\gssmooth}{C_g}
\newcommand{\fobj}{f_{\mathrm{obj}}}
\newcommand{\fcon}{f_{\mathrm{con}}}

\global\long\def\xk{x_{k}}%
\global\long\def\xkp{x_{k+1}}%
\global\long\def\pq{\textrm{proj}_{\mathcal{X}}}%

\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\out}{\mathrm{out}}
\newcommand{\tf}{\widetilde{f}}
\newcommand{\tF}{\widetilde{F}}
\newcommand{\tvphi}{\widetilde{\varphi}}
% \newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\inner}[1]{\left\langle#1\right\rangle}

% Comments
\newcommand{\Comments}{1} % Change to 0 to hide comments
\newcommand{\mynote}[2]{\ifnum\Comments=1\textcolor{#1}{#2}\fi}
\newcommand{\kai}[1]{\mynote{red}{[Kai: {#1}]}}
\newcommand{\pswt}[1]{\mynote{blue}{[SP: {#1}]}}
\newcommand{\gk}[1]{\mynote{orange}{[Guy: {#1}]}}
\newcommand{\jz}[1]{\mynote{cyan}{[Jimmy: {#1}]}}
%display-specifics
\newcommand{\weakconvexity}{\checkmark\hspace{-0.5ex}\textsubscript{w}}
\newcommand{\strongconvexity}{\checkmark\hspace{-0.5ex}\textsubscript{s}}

\newcommand{\compresslist}{ % Define a command to reduce spacing within itemize/enumerate environments, this is used right after \begin{itemize} or \begin{enumerate}
\setlength{\itemsep}{1pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
}

==> neurips_poster/defs.tex <==
% basic packages
%%%%%%%%%%%%%%%%%
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{palatino} %for the beautiful font 
\usepackage{fullpage} %without this package, the lowermost boxes expand too much, and it looks bad. 
\usepackage{amssymb,amsmath,amsthm,amsfonts,mathtools, thmtools}
\usepackage{xifthen} %so that in defining macros I can have optional arguments. 
\numberwithin{equation}{section}
%%%%%%%%%%%%%%%%%%

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{corollary}{Corollary}

%%%%%%%%%%%%%%%%%%%
\newcommand{\R}{\mathbb{R}}

==> src/abstract.tex <==
% In this paper, we consider constrained bilevel optimization problems, where the lower level constrains are characterized by a convex function of the lower and upper variables.

% V1:
% Solving bilevel optimization is known to be challenging and often requires computing expensive Hessian due to the bilevel structure.
% Recently, a fully first-order gradient method was proposed to solve bilevel problems with stationarity guarantee, yet its result is limited to unconstrained bilevel problems only. % Background
% In this paper, we consider constrained bilevel optimization and present Fully First-order Constrained Approximation methods (F\textsuperscript{2}CA) with hyperobjective stationarity guarantee. % contribution intro
% For linear equality constraints, our algorithm can converge to an $\epsilon$-stationary solution within $O(1/\epsilon^2)$ gradient oracles, which matches to the best-known rate of the unconstrained case. % Equality summary
% For general convex inequality constraints, our algorithm constructs an inexact gradient oracle, and uses it to reach
% % an
% $(\delta,\epsilon)$-Goldstein stationarity within $\tilde{O}(\frac{1}{\delta \epsilon^4})$ first-order oracles, or $\tilde{O}(\frac{d}{\delta \epsilon^3})$ zero-order estimates where $d$ is the dimensionality of variable $x$.  % First-order and zero-order constrained
% Our experiment suggests that F\textsuperscript{2}CA demonstrates a significantly cheaper computation with a similar convergence performance compared to the Hessian-based method using differentiable optimization (\textit{cvxpylayer}).


% Our result is the first fully first-order algorithm with hyperobjective stationarity guarantees for constrained bilevel optimization problems.  % Conclusion


% Bilevel optimization is a popular yet difficult problem to solve due to the bilevel structure. Traditional methods use 

% V2:
% Solving bilevel optimization problems is known to be challenging, as most existing methods require Hessian computations which are prohibitive in modern large-scale applications.
% Recently, a fully first-order method was proposed to solve bilevel problems with finite-time stationarity guarantees, yet this result is limited only to unconstrained bilevel problems. % Background
% In this paper, we consider constrained bilevel optimization and present Fully First-order Constrained Approximation methods (F\textsuperscript{2}CA) with finite-time hyperobjective stationarity guarantees. % contribution intro
% For linear equality constraints, our algorithm converges to an $\epsilon$-stationary point within $O(1/\epsilon^2)$ iterations, matching the best-known rate in the unconstrained case. % Equality summary
% For general convex inequality constraints, our algorithm constructs an inexact hypergradient oracle, and uses it to reach
% % % an
% $(\delta,\epsilon)$-Goldstein stationarity within either $\tilde{O}(\frac{1}{\delta \epsilon^4})$ or $\tilde{O}(\frac{d}{\delta \epsilon^3})$ iterations, where $d$ is the upper-level dimension. Along the way we develop nonsmooth nonconvex optimization methods with inexact oracles, which may be of independent interest.
% We support our theoretical findings with a numerical experiment, suggesting that F\textsuperscript{2}CA demonstrates 
% similar convergence rate compared to Hessian-based methods using differentiable optimization (\textit{cvxpylayer}), while achieving significantly cheaper computation time.

Algorithms for bilevel optimization often encounter Hessian computations, which are prohibitive in high dimensions. While recent works offer first-order methods for {unconstrained} bilevel problems, \textit{constrained} bilevel optimization remains relatively underexplored. We present {the first} fully first-order constrained optimization methods with finite-time hypergradient stationarity guarantees. For linear equality constraints, our algorithm converges to an $\epsilon$-stationary point in $\widetilde{O}(\epsilon^{-2})$ gradient oracle calls, which is nearly-optimal. For general convex inequality constraints, we attain $(\delta,\epsilon)$-Goldstein stationarity in either $\widetilde{O}({\delta^{-1} \epsilon^{-4}})$ or $\widetilde{O}(d{\delta^{-1} \epsilon^{-3}})$ gradient oracle calls, where $d$ is the upper-level dimension. Along the way, we develop novel nonsmooth nonconvex optimization methods with inexact oracles. Our preliminary numerical experiments verify these theoretical convergence guarantees.

==> src/applications.tex <==
\subsection{Applications}

==> src/background.tex <==
% \subsection{Differentiable optimization and non-fully first-order baseline}
% More precisely, ~\cite{amos2017optnet} propose treating KKT conditions of the constrained optimization problem as a fixed point equation of the optimal primal $y^*$ and dual $\gamma$ solution, and applying implicit function theorem to compute the derivative $\frac{\partial y^*}{\partial x}$ and $\frac{\partial \gamma}{\partial x}$. However, differentiating through the KKT conditions involves second-order derivatives. 

% \pswt{do we use this stuff below? it does not seem like it's used later, so we can perhaps remove it.} \kai{I think we should keep all the KKT conditions related derivation here. Later we just refer back to Section 2 for that. Some of these can be simplified to save space though.}
% \begin{align}
%     & \nabla_y g(x,y^*) + \gamma^\top \nabla_y h(x,y^*) = 0 \label{eqn:first-order-gradient} & \text{and} \quad \gamma h(x,y^*) = 0 
% \end{align}
% By computing the derivative of Equation~\ref{eqn:first-order-gradient} and applying implicit function theorem, we get a linear system of $\frac{d y^*}{d x}$ and $\frac{d \gamma}{d x}$ that can be written in a matrix form:
% \begin{align}\label{eqn:kkt-system}
% \underbrace{
% \begin{bmatrix}
% \nabla^2_{yy} g + \gamma^\top \nabla_{yy}^2 h & \nabla_y h_S^\top \\
% \text{diag}(\gamma) \nabla_y h_S & 0
% \end{bmatrix}}_{H_{\text{ineq}}}
% \begin{bmatrix}
%     \frac{\partial y^*}{\partial x} \\
%     \frac{\partial \gamma_S}{\partial x}
% \end{bmatrix}
% = 
% -
% \begin{bmatrix}
%     \nabla^2_{xy} g + \gamma \nabla_{xy}^2 h \\
%     \text{diag}(\gamma_S) \nabla_x h_S
% \end{bmatrix}
% \end{align}
% where $S$ denotes the set of active constraints $S = \{ i: h_i(x,y^*) = 0 \}$. We notice that the inactive constraints ($i \in \bar{S} = \{ h_i(x,y^*) < 0 \}$) must have zero dual solution $\gamma_i$ and zero dual derivative $\frac{d \gamma_i}{d x}$ (see Appendix~\ref{sec:inactive-constraints-in-differentiable-optimization} for more details), which can be removed in the matrix form.

% For equality constraints, we get a similar expression where all the constraints are active:
% \begin{align}\label{eqn:linear-kkt-system}
% \underbrace{
% \begin{bmatrix}
% \nabla^2_{yy} g + \gamma^\top \nabla_{yy}^2 h & \nabla_y h^\top \\
% \nabla_y h & 0
% \end{bmatrix}}_{H_{\text{eq}}}
% \begin{bmatrix}
%     \frac{\partial y^*}{\partial x} \\
%     \frac{\partial \gamma}{\partial x}
% \end{bmatrix}
% = 
% -
% \begin{bmatrix}
%     \nabla^2_{xy} g + \gamma \nabla_{xy}^2 h \\
%     \nabla_x h
% \end{bmatrix}
% \end{align}

% \cref{eqn:kkt-system} and \cref{eqn:linear-kkt-system} give a valid expression to compute subgradient $\frac{\partial y^*}{\partial x}$ under different constraints, which can be used in \cref{eqn:inequality_reformulation}.


==> src/bilevel_using_ncns_blackbox.tex <==
%%% SUBSUMED BY OTHER SECTIONS %%%

\section{An Attempt via Nonconvex Nonsmooth Optimization}\label{sec:ncns_blackbox}
The objective $F$ in the lower-level constrained bilevel problem, \cref{prob:orig_bilevel},
is nonsmooth and nonconvex in $x$. In this section, we, therefore, propose solving \cref{prob:orig_bilevel} using recent developments in nonsmooth nonconvex optimization. A crucial requirement to be able to use these developments is that $F$ be Lipschitz. \pswt{note: the algorithm of DDLPY requires only Lipschitzness of the objective in question; is it possible that we can therefore get a result for the following setting: Lipschitz upper-level objective, ??? lower-level problem. Note that here we require no convexity or smoothness assumptions on the upper-level objective, something we've not seen thus far. Of course, the guarantee will also be only for Goldstein stationarity.}
\begin{lemma}\label{lem:LipscConstrBilevel}
$F$ is Lipschitz
\end{lemma}
\begin{proof}[Lipschitzness of Bilevel \pswt{check!}]
    By Lemma $2.1b$ of \cite{ghadimi2018approximation}, the hypergradient of $F$ computed with respect to the variable $x$ may be expressed as $\nabla_x F(x) = \nabla_x f(x, y^\ast(x)) + \nabla_x y^\ast(x) \cdot \nabla_y f(x, y^\ast(x))$. If we impose Lipschitzness assumptions on $f$, with respect to each of the coordinates, and additionally, if we can show $\|\nabla_x y^\ast(x)\|\leq L_{yx}$ for some constant, then it concludes the proof of Lipschitzness of $F$ with a Lipschitz constant $L_F \leq L_{fx} + L_{fy}\cdot L_{yx}$. Note that a bound on $\|\nabla_x y^\ast(x)\|$ was obtained by \cite{ghadimi2018approximation} in terms of second-order properties of $g$ and one in terms of constants from weaker assumptions in \cite{kwon2023fully} --- however, the latter also involves the Lagrange multiplier used therein. \pswt{How can we get for $y^\ast(x)$ a Lipschitz constant that is independent of any Lagrange multipliers? I think this is perhaps a self-contained question: what is the Lipschitz constant of the minimizer of a (strongly) convex function over the $0$-level set of a (strongly) convex function? Note: Jimmy has a solution for this.} 
\end{proof}

==> src/conclusion.tex <==
\section{Limitations and future directions}
Our computational complexity for solving bilevel programs with general convex inequalities is $O(\delta^{-1} \epsilon^{-4})$ oracle calls for reaching $(\delta,\epsilon)$-Goldstein stationarity, where we lose an $O(\epsilon^{-1})$ factor constructing the inexact gradient oracle. We believe this rate is not inherent to the problem and that a better approach could potentially improve it to the best known rate $O(\delta^{-1} \epsilon^{-3})$ for nonsmooth nonconvex optimization. Furthermore, removing the Lipschitzness assumption on $y^*(x)$ for this setting is an important direction for future research.
% \jz{maybe say something weaker: We believe this gap is not inherent to the problem. A better approach could potentially close the gap.}

==> src/condensed-relatedwork.tex <==
\subsection{Related work}\label{sec:related_work} 
% \pswt{the full related work section is in ``related-work.tex''; we can use it for reference if needed}
% The space of algorithms for bilevel programming is vast. 
The vast body of work on asymptotic results for bilevel programming, starting with classical works such as \cite{anandalingam1990solution, ishizuka1992double, white1993penalty, vicente1994descent, ye1995optimality, ye1997exact}, typically fall into two categories: those based on approximate implicit differentiation ~\cite{domke2012generic, pedregosa2016hyperparameter, gould2016differentiating, amos2017optnet, liao2018reviving, agrawal2019differentiable, grazzi2020iteration, lorraine2020optimizing} and those via iterative differentiation~\cite{domke2012generic, maclaurin2015gradient, franceschi2017forward,   franceschi2018bilevel,  shaban2019truncated, grazzi2020iteration}. Another recent line of work  in this category includes \cite{liu2021value, ye2023difference, khanduri2023linearly, gao2024moreau}, which use various smoothing techniques. 
% smoothing on the problem via some combination of barrier function and Moreau envelope. 
% Other uses of smoothing were seen in \cite{ye2023difference} and \cite{gao2024moreau}, which used tools from the literature on difference of convex programs. These results are mostly asymptotic.  

The first non-asymptotic result for bilevel programming was provided by \cite{ghadimi2018approximation}, which was followed by a flurry of work: for example, algorithms that are single-loop stochastic~\cite{chen2021closing, chen2022single, hong2023two}, projection-free~\cite{akhtar2022projection, jiang2023conditional, abolfazli2023inexact, cao2024projection}, use variance-reduction and momentum~\cite{khanduri2021near, guo2021randomized, yang2021provably, dagreou2022framework}, those for single-variable bilevel programs~\cite{sabach2017first, amini2019iterative, amini2019iterativereg, jiang2023conditional, merchav2023convex}, and  for bilevel programs with special  constraints~\cite{tsaknakis2022implicit, khanduri2023linearly, xu2023efficient, abolfazli2023inexact}. 
 
% There have also been some recent works on constrained bilevel programming, mostly focusing on specific types of constraints. Examples of these works include those by \cite{tsaknakis2022implicit} and \cite{khanduri2023linearly} for linear inequality constraints and \cite{xu2023efficient}, which provides asymptotic guarantees for attaining Clarke stationarity with more general constraints. 

The most direct predecessors of our work are \cite{liu2021value, kwon2023fully} and \cite{yao2024constrained, lu2024firstorder}. As alluded to earlier, until recently, there did not exist any fully first-order algorithms with finite-time stationary guarantees for bilevel programming. The work of \cite{liu2022bome} made a significant contribution to this end by providing a method to approximate the hypergradient of the unconstrained bilevel problem  in a fully-first order fashion. This was extended to the stochastic setting by \cite{kwon2023fully} (which we also build upon), which was simplified and improved by \cite{chen2023near}, and  recently extended to the constrained setting by \cite{yao2024constrained, lu2024firstorder}.

While \cite{yao2024constrained, lu2024firstorder} also study the constrained setting, a key difference of our work lies in the stationarity criteria. \cite{yao2024constrained, lu2024firstorder} use KKT stationarity over both upper and lower-level variables as a proxy to the hypergradient stationarity, whereas we directly work with $(\delta, \epsilon)$-stationarity over the upper-level objective.
Moreover, \cite{yao2024constrained} assumes joint convexity of the lower-level constraints in upper and lower variables to allow for efficient projections, 
while we require convexity only in the lower-level variable. 
% \pswt{can we perhaps explain why our notion of stationarity might be \emph{better}?}
% \pswt{add zhaosong-sanyou paper}
% \pswt{is this true when their upper level is also unconstrained?}

% \pswt{explain why ours is more meaningful}. Secondly, \pswt{nonconvex projection} 

==> src/error-propagation.tex <==

% Error in the inner optimization solution $y^*$ and $\lambda^*$ can lead to incorrect construction of the penalty function, which later causes error in the gradient approximation. Now we bound the error propagation here.

% Let us denote the approximate solution to the inner optimization problem by $y'$ and $\lambda^*'$, which are $\alpha^2$ close to the optimal solution $y^*$ and $\lambda^*$, i.e., $\norm{y' - y^*} \leq \alpha^2$ and $\norm{\lambda^*' - \lambda^*} \leq \alpha^2$.
% Using the approximate solution $y'$ and $\lambda^*'$ to construct the penalty function:
% \begin{align}
%     \mathcal{L}_{\lambda^*',\alpha}(x,y) = f(x,y) + \alpha_1 (g(x,y) + (\lambda^*')^\top h(x,y) - g(x,y')) + \frac{\alpha_2}{2} \norm{h_{\mathcal{I}(x,y)}}^2
% \end{align}
% which can also be used to find the optimal solution to the peanlty function defined on $y'$ and $\lambda^*'$:
% \begin{align}
%     y'_{\lambda^*,\alpha} \coloneqq \arg\min_y \mathcal{L}_{\lambda^*',\alpha}(x,y)
% \end{align}
% By the same argument in \cref{thm:solution-bound}, we also get:
% \begin{align}
%     & \norm{y'_{\lambda^*,\alpha} - y'} \leq O(\alpha_1^{-1}) = O(\alpha^{-2}), & \norm{h_\mathcal{I}(x,y'_{\lambda^*,\alpha})} \leq O(\frac{1}{\sqrt{\alpha_1 \alpha_2}}) = O(\alpha^{-3/2})
% \end{align}

% Combining this with our bound $\norm{y^*_{\lambda^*,\alpha} - y^*} \leq O(\alpha^{-2})$ and the accuracy of the primal solution $\norm{y' - y^*} \leq \alpha^2$, we get:
% \begin{align}
%     \norm{y'_{\lambda^*,\alpha} - y^*} \leq O(\alpha^{-2})
% \end{align}

% We can write the inexact gradient using the inexact inner problem solutions by:
% \begin{align}
%     & \nabla_x \mathcal{L}_{\lambda^*',\alpha}(x,y'_{\lambda^*',\alpha}) = \nabla_x f(x,y'_{\lambda^*',\alpha}) + \alpha_1 (\nabla_x g(x,y'_{\lambda^*',\alpha}) + (\lambda^*')^\top \nabla_x h(x,y'_{\lambda^*',\alpha}) - \nabla_x g(x,y') - (\lambda^*')^\top \nabla_x h(x,y')) \nonumber \\
%     & \quad \quad \quad + {\alpha_2} \nabla_x h_{\mathcal{I}}(x,y'_{\lambda^*',\alpha})^\top h_{\mathcal{I}}(x,y'_{\lambda^*',\alpha})
% \end{align}

% We are now ready to bound the difference between the inexact gradient estimated from the inexact solutions, and the inexact gradient estimated from the exact solutions:
% \begin{align}
%     & \nabla_x \mathcal{L}_{\lambda^*',\alpha}(x,y^*_{\lambda^*,\alpha}) - \nabla_x \mathcal{L}_{\lambda^*,\alpha}(x,y'_{\lambda^*,\alpha}) \nonumber \\
%     = & \nabla_x f(x,y^*_{\lambda^*,\alpha}) - \nabla_x f(x,y'_{\lambda^*,\alpha}) \\
%     & \quad + {\alpha_1} \biggl(\nabla_x g(x,y^*_{\lambda^*,\alpha}) + (\lambda^*)^\top \nabla_x h(x,y^*_{\lambda^*,\alpha}) - \nabla_x g(x,y'_{\lambda^*,\alpha}) - (\lambda^*')^\top \nabla_x h(x,y'_{\lambda^*,\alpha})  \biggl)\\
%     & \quad \quad + {\alpha_2} \biggl(\nabla_x h_{\mathcal{I}}(x,y^*_{\lambda^*,\alpha})^\top h_{\mathcal{I}}(x,y^*_{\lambda^*,\alpha}) - \nabla_x h_{\mathcal{I}}(x,y'_{\lambda^*',\alpha})^\top h_{\mathcal{I}}(x,y'_{\lambda^*',\alpha}) \biggl)
% \end{align}

==> src/experiment.tex <==
\section{Experiments}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{src/figures/ydim200_loss.pdf}
        \caption{Convergence comparison and gradient error plot.}
        \label{fig:convergence-comparison}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{src/figures/ydim200_gradient_error.pdf}
        \caption{Convergence analysis with varying gradient inexactness $\alpha$.}
        \label{fig:convergence-comparison-2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{src/figures/time_results.pdf}
        \caption{Computation cost per gradient step of varying problem size $d_y$.}
        \label{fig:computation-comparison}
    \end{subfigure}
    \caption{We run \cref{alg: PIGD} using \cref{alg:inexact-gradient-oracle} on the bilevel optimization in the toy example in \cref{eqn:experiment-bilevel-optimization} with $d_x = 100$, $d_y = 200$, $n_{\text{const}} = d_y / 5$, and accuracy $\alpha = 1$. \cref{fig:convergence-comparison}, \cref{fig:convergence-comparison-2}, \cref{fig:computation-comparison} vary \# of iterations, gradient exactness $\alpha$, and $d_y$, respectively, to compare the performance under different settings.}
    % Figure~\ref{fig:convergence-comparison} shows that \cref{alg: PIGD} converges in the same rate as CvxpyLayer, while the gradient errors at each iteration are plotted in the colorful bars and are mostly below $\alpha = 0.1$ as guaranteed. Figure~\ref{fig:convergence-comparison-2} shows the convergence under different gradient inexactness $\alpha$. Figure~\ref{fig:computation-comparison} shows the computation cost of both methods under different lower level problem size $d_y$.}
    \label{fig:three graphs}
\end{figure}

We randomly generate the following constrained bilevel optimization problems. 
\begin{align*}\numberthis\label[prob]{eqn:experiment-bilevel-optimization}
     & \mbox{minimize}_{x} ~  c^\top y^* + 0.01 \norm{x}^2 + 0.01 \norm{y^*}^2 ~\text{ subject to } ~ y^* = \argmin_{y: h(x,y) \leq 0} \frac{1}{2} y^\top Q y + x^\top P y, 
\end{align*}
% \begin{align}\label{}
%     \min\nolimits_{x} \quad & \\
%     \text{s.t.} \quad & \nonumber
% \end{align}
where $h_i(x,y) = x^\top A_i y - x^\top b_i ~\forall i \in [K]$ are $K$ bilinear constraints. The PSD matrix $Q \in \reals^{d_y \times d_y}$, $c \in \reals^{d_y}$, $P \in \reals^{d_x \times d_y}$, and constraints $A_i \in \reals^{d_x \times d_y}$, $b_i \in \reals^{d_x}$ are randomly generated from normal distributions (cf. \cref{appendix:experiment-setup}).
We compare our \cref{alg: PIGD} with a non-fully first-order method implemented using \texttt{cvxpyLayer}~\cite{agrawal2019differentiable}. Both algorithms use Adam~\cite{kingma2014adam} to control the learning rate in gradient descent. All the experiments are averaged over ten random seeds.

% \paragraph{Convergence and computation comparisons:} 
\looseness=-1\cref{fig:convergence-comparison} shows that  
% compares the convergence of both methods. We can see that 
both the algorithms converge to the same optimal solution, while the fully first-order method is slightly more stable. Simultaneously, the colorful bars represent the gradient difference between two methods, showing the inexactness of gradient.
\cref{fig:convergence-comparison-2} additionally varies the inexactness to demonstrate its impact to convergence. One can find that too accurate gradient may also harm the convergence due to instability from poor condition numbers.
\cref{fig:computation-comparison} compares the computation cost of different lower level problem size $d_y$. Our fully first-order method significantly outperforms the differentiable optimization method in computation cost.

==> src/inequalitySetting-gradient-approximation.tex <==
\section{Inequality constraints: constructing the inexact gradient oracle}\label{sec:inequality-bilevel}

We first consider constrained bilevel optimization in which the lower-level constraints are defined by general convex inequality constraints, i.e., 
% defined by 
$S(x) \coloneqq \{ y: h(x,y) \leq 0 \}$:
\begin{align}\label[prob]{prob:ineq}
     \mathop{\text{minimize}}\nolimits_{x} ~ F(x) \coloneqq f(x, \ystar(x)) \quad \text{ subject to} ~\ystar(x)\in \argmin\nolimits_{y: h(x, y) \leq 0} g(x, y).
\end{align}
Computing a stationary point of $F$ via any first-order method would require the gradient,  given by: %
%\jz{why run gradient descent? this line needs to be properly motivated}
% \pswt{Kai: we wanted some notation other than $\partial F$ and $\frac{\partial y^*}{\partial x}$, right?}
\begin{align}\label{eqn:second-order-method}
    \nabla_x F(x) = \nabla_x f(x,y^*) + \left(\frac{ dy^*(x)}{d x}\right)^\top \nabla_y f(x,y^*),
\end{align}
for which the key challenge lies in computing  $\frac{d y^*(x)}{d x}$. This requires differentiating through an argmin operator, 
% (recall $y^*(x) = \arg\min\nolimits_{y: h(x,y) \leq 0} g(x,y)$) 
% using differentiable optimization~\cite{amos2017optnet,agrawal2019differentiable}, 
which typically requires second-order derivatives.  
% \jz{Why do we have to call up differentiable optimization to motivate this part?  }
% As mentioned in \cref{sec:differentiable-optimization}, in order to compute the derivative of $F(x)$, we need to compute $\frac{dy^*}{dx}$ 
% \pswt{$\frac{dy^*}{dx}$? forgot what notatoin we settled on}. 
Instead, here we 
% here we follow the technique of differentiable optimization~\cite{amos2017optnet,agrawal2019differentiable} \pswt{In the introduction, we say that diff opt requires second-order derivatives, but we are saying in the next sentence that that is what we use; a bit confusing?} to 
differentiate (using the implicit function theorem) through the KKT conditions describing $y^*(x)$
% using implicit function theorem
and get: % \pswt{Some terms below are restricted to $\mathcal{I}$, while others aren't; can you define $h_{\mathcal{I}}$ and $\lambda_{\mathcal{I}}$ with dimensions?} \kai{TODO}
% \pswt{Kai: I'm slightly confused again with the dimensions; in $H$ below, would it need to be $\nabla^2_{yy} h \lambda$ instead of $\lambda^\top \nabla_{yy}^2 h$? Same comment for the RHS with $\nabla^2_{xy} h$. Notation of $\partial$? } \kai{Either $(\nabla_{yy}^2)^\top \lambda$ or $\lambda^\top (\nabla_{yy}^2)$ works. $\lambda \in \reals^{d_h}$ is a column vector and $\nabla_{yy}^2 h \in \reals^{d_h \times d_y \times d_y}$. In Section 5, I think the corresponding $\alpha^*$ (or $\lambda^*$) should be a column vector as well and thus the matrix multiplication there might be wrong (or just use dot product instead).}
\begin{align}\label{eqn:kkt-system}
\begin{bmatrix}
\nabla^2_{yy} g + \lambda^\top \nabla_{yy}^2 h & \nabla_y h_\mathcal{I}^\top \\
\text{diag}(\lambda_\mathcal{I}) \nabla_y h_\mathcal{I} & 0
\end{bmatrix}
\begin{bmatrix}
    \frac{d y^*(x)}{d x} \\
    \frac{d \lambda_\mathcal{I}(x)}{d x}
\end{bmatrix}
= 
-
\begin{bmatrix}
    \nabla^2_{yx} g + \lambda^\top \nabla_{yx}^2 h \\
    \text{diag}(\lambda_\mathcal{I}) \nabla_x h_\mathcal{I}
\end{bmatrix}
\end{align}
where given $x$, we define $y^*(x)$ and $\lambda(x)$ to be the primal and dual solutions to the LL problem in \cref{prob:ineq}. We denote $\mathcal{I} \coloneqq \{i \in [d_h]: h_i(x,y) = 0, \lambda_i > 0 \}$ to be the set of active constraints with non-zero dual solution, and
$h_\mathcal{I} \coloneqq [h_i]_{i \in \mathcal{I}}$ and $\lambda_{\mathcal{I}} \coloneqq [\lambda_i]_{i \in \mathcal{I}}$ are the constraints and dual variables corresponding to the set $\mathcal{I}$. 
The KKT system  involves only the constraints in $\mathcal{I}$ because other constraints are degenerate \pswt{phrasing unclear to me}; see \cref{sec:inactive-constraints-in-differentiable-optimization} for more details. 


% since the inactive constraints and zero dual solution lead to degeneracy in the KKT conditions;  % \jz{how do we identify the active constraint if we are doing only finite precision calculation?} \kai{Will discuss this later.}

Observe that as is, Equation \cref{eqn:kkt-system} leads to a second-order computation of $\frac{dy^*(x)}{dx}$.
% \pswt{check notation} 
In the rest of the section, we provide a fully first-order \emph{approximate} gradient oracle by constructing an equivalent reformulation of \cref{prob:ineq} using a penalty function (with two different penalties).
% to provide a fully first-order inexact gradient oracle.
% In this section, we provide a fully first-order inexact gradient oracle to compute $\frac{\partial y}{\partial x}$ with $\epsilon$ error.
% Compared to Section~\ref{sec:equality-bilevel}, the major technical challenge in the inequality case is the non-smoothness of the optimal solution $y^*(x)$ due to potentially a different set of constraints being satisfied. Although we can still ensure the continuity and Lipschitzness of $y^*(x)$, its smoothness is no longer guaranteed.



% \jz{do we still need the constraint $h(x,y)\leq 0$ in the reformulated problem? I think we would not need it for Theorem 3.1 to be valid, by Sion's minimax theorem. But I guess you need it for other reasons.} \kai{Yes, the inequality case still needs the constraint. I don't have a good intuition why it differs for ineq and eq cases.}

% \noindent\textbf{Intuition:} the idea is to assume an oracle access to the dual solution $\lambda$ and construct Lagrangian based on the dual solution. Realistically, the dual solution $\lambda(x)$ is also a function of $x$, and thus the derivative should be $\frac{d}{dx} g^*_\lambda(x) = \nabla_x g(x,y^*) + \lambda^\top \nabla_x h(x,y^*) + (\nabla_x \lambda(x))^\top h(x,y^*)$. But when some nice properties hold, the zero entries of $\nabla_x \lambda(x)$ matches to the non-zero entries of $h(x,y^*)$ (complementary slackness). Therefore, we can just use the remaining terms to compute gradient.






% They show that \cref{eqn:moreau-reformulation} is equivalent to the bilevel optimization problem, where:
% \begin{align}\label{eqn:moreau-function-definition}
%     v_{a,b}(x,y,z) = \min_{\theta} \max_{\beta} g(x,\theta) + \beta h(x,\theta)_+ + \frac{1}{2 a} \norm{\theta - y}^2 - \frac{1}{2 b} \norm{\beta - z}^2
% \end{align}


% \begin{align}
%     & v_{a,b}(x,y,z) = g(x,\theta^*) + \beta^* h (x,\theta^*)_+ + \frac{1}{2 a} \norm{\theta^* - y}^2 - \frac{1}{2 b} \norm{\beta^* - z}^2 \\
%     & \frac{d}{dx} v_{a,b}(x,y,z) = \frac{\partial}{\partial x} v_{a,b}(x,y,z) + \frac{\partial}{\partial \theta} v_{a,b}(x,y,z) \frac{d \theta^*}{dx} + \frac{\partial}{\partial \beta} v_{a,b}(x,y,z) \frac{d \beta^*}{dx} \\
%     & = \frac{\partial}{\partial x} v_{a,b}(x,y,z)
% \end{align}

% According to their result, we know that the gradient of the Moreau envelop is:
% \begin{align}\label{eqn:moreau-function-derivative}
%     \nabla v_{a,b}(x,y,z) = (\nabla_x g(x, \theta^*) + \beta^* \nabla_x h(x, \theta^*)_+, \frac{y - \theta^*}{a}, \frac{\beta^* - z}{b})
% \end{align}

% \subsection{Why the previous algorithm is not good enough?}
% If we just look at the reformulation in \cref{eqn:moreau-reformulation}, it asks us to solve a constrained optimization again:
% \begin{align}
%     \min_{x,y: h(x,y) \leq 0 ; z \geq 0} \quad & f(x,y) \\
%     \text{s.t.} \quad & g(x,y) \leq v_{a,b}(x,y,z)
% \end{align}
% which ~\cite{yao2024constrained} uses a Lagrangian-style algorithm to jointly do projected gradient descent on $x,y,z$, which yields a first-order algorithm with some convergence guarantees.
% However, their algorithm requires projecting back to the feasible region $\{ (x,y): g(x,y) \leq 0 \} $ jointly for $x$ and $y$. We know that the function $g(x,y)$ is convex in $y$ but not jointly convex for $x$ and $y$. This causes the feasible region not necessary a convex set jointly for $x$ and $y$, which makes projection a potentially non-trivial operation.
% Therefore, the goal here is to see if we can do gradient descent on $x$ and $y$ separately, which given $x$, we can project $y$ to its convex feasible region $\{y: g(x,y) \leq 0 \}$ with no additional computation challenge.

\subsection{Reformulation via the penalty method}
We begin by reformulating \cref{prob:ineq} into a single level constrained optimization problem:
\begin{align}\label{eqn:inequality_reformulation}
    \text{minimize}_{x,y} ~ f(x,y)  \text{ subject to}
    ~\begin{cases}
        g(x,y) + \lambda(x)^\top h(x,y) \leq g^*(x) \\ 
        h(x,y) \leq 0
    \end{cases},
\end{align}
where $g^*(x)  \coloneqq \min_{y: h(x,y) \leq 0} g(x,y) = g(x,y^*(x))$ and $\lambda(x)$ is the optimal dual solution. The equivalence of this reformulation to  \cref{prob:ineq} is spelled out in \cref{appendix:reformulation-equivalence}. 
% For a given $x$, evaluating \cref{eqn:inequality_reformulation} requires computing the primal solution $y^*(x)$ and the corresponding dual solution $\lambda(x)$ to the lower level problem.\pswt{commenting out because the sentence was not implying anything that was being used later}
% Given the reformulated problem in \cref{eqn:inequality_reformulation}, 
We therefore define the following penalty function, which is crucial to our analysis:
\begin{align}
    \mathcal{L}_{\lambda, \boldsymbol{\alpha}}(x,y) = f(x,y) + \alpha_1 \left( g(x,y) + \lambda^\top h(x,y) - g^*(x)  \right) + \frac{\alpha_2}{2} \norm{h_\mathcal{I}(x,y)}^2, \numberthis\label{eqn:penalty-lagrangian}
\end{align}
where $\boldsymbol{\alpha} = [\alpha_1, \alpha_2] \geq 0$ are the penalty parameters.
Notably, given the aforementioned penalty function, we can compute its derivative with respect to $x$ as
\begin{align*}
    \nabla_x \mathcal{L}_{\lambda, \boldsymbol{\alpha}}(x, y) = \nabla_x f(x,y) \! + \! \alpha_1 (\nabla_x g(x,y) \! + \! \lambda^\top \nabla_x h(x,y) \! - \! \nabla_x g^*(x) ) \! + \! \alpha_2 \nabla_x h_\mathcal{I}(x,y)^\top h_\mathcal{I}(x,y).
    % \label{eqn:lagrangian-derivative}
\end{align*}

We further define the optimal solutions to the penalty function optimization by:
\begin{align*}
    y_{\lambda, \boldsymbol{\alpha}}^*(x) := \arg\min\nolimits_{y} \mathcal{L}_{\lambda, \boldsymbol{\alpha}}(x,y).\numberthis\label{eq:def_y_lambda_star} 
\end{align*}
% where $S$ is the set of active constraints in the lower level optimization problem. This additional constraint ensures that inactive constraints in the lower level problem stay satisfied, while only the active constraints can be violated. This design choice plays an important role in the later analysis.



% , and $S$ is the set of active constraints with non-zero dual solution in the lower-level problem. \pswt{already defined in the previous paragraph; removed y* and lambda because they are also already defined}
% , and the penalty function $p(x,y) = h(x,y) - h(x,y^*) - \nabla_y h(x,y^*)^\top (y - y^*) \geq 0 ~\forall y$.

 To give some intuition for our choice of two different penalties in \cref{{eqn:penalty-lagrangian}}, we note that the the two constraints in \cref{eqn:inequality_reformulation} behave quite differently.
The first constraint $g(x,y) + \lambda(x)^\top h(x, y) \leq g^*(x)$ is one-sided, i.e., can only be violated or met, which just needs a penalty parameter $\alpha_1$ to weight the ``violation''.
As to the second constraint $h(x,y) \leq 0$, it can be arbitrary. To allow such a ``two-sided'' constraint, we penalize only the active constraints $\mathcal{I}$, i.e., we use $\norm{h_{\mathcal{I}}(x,y)}^2$ to penalize deviation.

Given this penalty function, we now show that the optimal solution to the penalty minimization is close to the optimal solution to the LL problem with a small constraint violation.

% We will gradually increase $\alpha_1$ and $\alpha_2$ to increase the penalty on constraint violations.

% This one is smooth but I am not sure if $\alpha \rightarrow \infty$ will lead to the same solution as the original bilevel optimization.


% \begin{assumption}\label{assumption:smoothness} 
%  \pswt{We seem to also use a bound on $\nabla^2_{xy}f$ in the proof of \cref{thm:diff_in_hypergrad_and_gradLagr}; is the constant for that included in the current assumption?} 
%     \begin{itemize}
%         \item $f(x,y), g(x,y), h(x,y)$ are smooth in $x$ and $y$ with smoothness $C_f$, $C_g$ and $C_h$, respectively.
%         \item $f(x,y)$ is $L_f$ Lipschitz in $y$.
%         \item $g(x,y)$ is $\mu_g$-strongly convex in $y$.
%         \item $h(x,y)$ is convex in $y$.
%     \end{itemize}
% \end{assumption}


% \begin{theorem}
%     $g(x,y) - v_{a,b}(x,y,z,s) + \frac{b}{2} \norm{h(x,y)}^2$ is convex in $y$.
% \end{theorem}
% \begin{proof}
%     Define $\phi_b(x,\theta,z) = \max_\alpha g(x,\theta) + \alpha h(x,\theta) - \frac{1}{2b} \norm{\alpha - z}^2$. We know that $v_{a,b}(x,y,z) = \min_{\theta} \phi_b(x,\theta,z) + \frac{1}{2a} \norm{\theta - y}^2$ by definition.

%     Now we can compute:
%     \begin{align}
%         g(x,y) - v_{a,b}(x,y,z) & = g(x,y) - \min_\theta \left( \phi_b(x,\theta,z) + \frac{1}{2a} \norm{\theta - y}^2 \right) \\
%         & \geq g(x,y) - \left( \phi_b(x,y,z) + \frac{1}{2a} \norm{y - y}^2 \right) \\
%         & = g(x,y) - \phi_b(x,y,z) \\
%         & = g(x,y) - \max_\alpha \left( g(x,y) + \alpha h(x,y) - \frac{1}{2b} \norm{\alpha - z}^2 \right) \\
%         & = - \max_\alpha \left( \alpha h(x,y) - \frac{1}{2b} \norm{\alpha - z}^2 \right) \\
%         & = - \frac{b}{2} \alpha \norm{h(x,y)}^2
%     \end{align}
% \end{proof}

% \begin{theorem}
%     {\color{red} $\max_{z \geq 0} v_{a,b}(x,y,z)$} is $\frac{\mu_g}{a \mu_g - 1}$-smooth in $y$.
% \end{theorem}
% \begin{proof}
%     Define $\phi_b(x,\theta,z) = \max_\beta g(x,\theta) + \beta^\top h(x,\theta) - \frac{1}{2b} \norm{z - \beta}^2$, which is a maximization over strongly convex function $g(x,\theta) + \beta h(x, \theta)$. Thus $\phi_b(x,\theta,z)$ is still $\mu_g$ strongly convex in $\theta$.

%     Given $\theta^*(x,y,z) = \arg\min_\theta \phi_b(x,\theta,z) + \frac{1}{2a} \norm{\theta - y}^2$, we know that:
%     \begin{align}
%         \frac{y - \theta^*}{a} = \nabla_y \phi(x,\theta^*,z)
%     \end{align}
%     For two different pairs $(x,y_1,z)$ and $(x,y_2,z)$, we can compute the difference in the gradient:
%     \begin{align}
%         \norm{\frac{y_1 - \theta^*_1}{a} - \frac{y_2 - \theta^*_2}{a}} & = \norm{\nabla_y \phi(x,\theta_1^*, z) - \nabla_y \phi(x, \theta^*_2, z)} \geq \mu_g \norm{\theta^*_1 - \theta^*_2} 
%     \end{align}
%     where the last inequality we use the $\mu_g$ strong convexity of the function $\phi$.
    
%     We can re-arrange the inequality to get:
%     \begin{align}
%         \mu_g \norm{\theta^*_1 - \theta^*_2} \leq \norm{\frac{y_1 - \theta^*_1}{a} - \frac{y_2 - \theta^*_2}{a}} \leq \frac{1}{a} \norm{y_1 - y_2} + \frac{1}{a} \norm{\theta_1 - \theta_2}
%     \end{align}
%     Therefore, we can bound
%     \begin{align}
%         (a \mu_g - 1) \norm{\theta^*_1 - \theta^*_2} \leq \norm{y_1 - y_2} 
%     \end{align}

%     Now come back to the difference of the gradients in the Moreau envelop function $v_{a,b}$. We can show that:
%     \begin{align}
%         \norm{\nabla_{y} v_{a,b}(x,y_1,z) - \nabla_{y} v_{a,b}(x,y_2,z)} = & \norm{\frac{y_1 - \theta^*_1}{a} - \frac{y_2 - \theta^*_2}{a}} \leq \frac{1}{a} \norm{y_1 - y_2} + \frac{1}{a} \norm{\theta_1 - \theta_2} \\
%         \leq & \frac{1}{a} \norm{y_1 - y_2} + \frac{1}{a} \frac{1}{a \mu_g - 1} \norm{y_1 - y_2} = \frac{\mu_g}{a \mu_g - 1} \norm{y_1 - y_2}
%     \end{align}
%     Therefore, the Moreau envelop function $v_{a,b}(x,y,z)$ is $\frac{\mu_g}{a \mu_g - 1}$-smooth in $y$, which concludes the proof.
% \end{proof}

% {\color{red}
% \begin{theorem}
%     $v_{a,b}(x,y,z)$ is $\frac{1}{b}$ strongly concave in $z$.
% \end{theorem}
% \begin{proof}
% % Fix $a,b>0$.
% % Let $\psi_{x,y}^{\beta,\theta}(z):=g(x,\theta)+\beta h(x,\theta)+\frac{1}{2a}\norm{\theta-y}^2-\frac{1}{2b}\norm{z-\beta}^2$, and note that $\psi_{x,y}^{\beta,\theta}(\cdot)$ is $\frac{1}{b}$-strongly concave for any $x,y,\theta,\beta$. Hence, 
% % $\Psi_{x,y}^{\beta}(z):=\min_{\theta}\psi_{x,y}^{\beta,\theta}(z)$ is $\frac{1}{b}$-strongly concave for any $x,y,\theta$ by preservation of strong concavity under the min operation. Therefore $-\Psi_{x,y}^{\beta}(\cdot)$ is $\frac{1}{b}$ strongly convex, hence $\max_{\beta}[-\Psi_{x,y}^{\beta}(z)]$ is $\frac{1}{b}$ strongly convex, or equivalently $-\max_{\beta}[-\Psi_{x,y}^{\beta}(z)]=-\min_{\beta}$
% % is $\frac{1}{b}$ strongly concave,


%     Define $\psi(x,y,\beta) = \min_\theta g(x,\theta) + \beta^\top h(x,\theta) + \frac{1}{2a} \norm{\theta - y}^2$
%     \begin{align}
%         \nabla_z v_{a,b}(x,y,z_1) - \nabla_z v_{a,b}(x,y,z_2) = \frac{\beta^*_1 - z_1}{b} - \frac{\beta^*_2 - z_2}{b}
%     \end{align}
    
%      Kai: Somehow I feel that $v_{a,b}$ is only concave in $z$. I couldn't prove its strong concavity...
% \end{proof}
% }


\begin{restatable}[]{lemma}{solutionApproximation}\label{thm:solution-bound}
Given any $x$, the corresponding dual solution $\lambda(x)$,  primal solution $y^*(x)$ of the lower optimization problem in \cref{prob:ineq}, and $y_{\lambda, \boldsymbol{\alpha}}^*(x)$ as in \cref{{eq:def_y_lambda_star}}, satisfy:
\begin{align}\label{eqn:solution-bound}
    \norm{y_{\lambda, \boldsymbol{\alpha}}^*(x) - y^*(x)} \leq O(\alpha_1^{-1}) \text{~~and~~} \norm{h_\mathcal{I}(x,y_{\lambda, \boldsymbol{\alpha}}^*(x))} \leq O(\alpha_1^{-1/2} \alpha_2^{-1/2}).
\end{align}
\end{restatable}
The proof of \cref{thm:solution-bound} is based on the strong convexity of $g$ for sufficiently large $\alpha_1$, and the Lipschitzness of $f$. Compared to \cite{kwon2023fully}, due to the inequality constraints, we get an additional bound on the constraint violation $h_\mathcal{I}(x,y)$. This constraint violation bound is later used in \cref{thm:diff_in_hypergrad_and_gradLagr} to bound the inexactness of our proposed gradient oracle that involves constraint violation. 

% \pswt{It might be more helpful to first state why are stating this bound (so that the reader knows why they are reading \cref{thm:solution-bound}), then state the bound itself, and then provide intuition on how it's proved}\jz{I think the reader would like to see some distilled insights before going into all the algebra. Like what's challenging about the inequality setting: the KKT matrix is not invertible. Then how were you able to overcome that fundemental challengee.} \kai{Added a sentence to explain. Depending on if we have space, I can add more intuitions if needed.}


\subsection{Main result: approximating the hypergradient}
Based on the penalty function $\mathcal{L}_{\lambda,\alpha}(x,y)$ and its solution bounds on $y^*_{\lambda,\alpha}$ in \cref{thm:solution-bound}, the main export of this section is the following bound on the approximation of  the hypergradient. 
\begin{restatable}[]{lemma}{gradientApproximation}\label{thm:diff_in_hypergrad_and_gradLagr}
Consider $F$ as in \cref{{prob:ineq}},   $\mathcal{L}$ as in  \cref{{eqn:penalty-lagrangian}},  a fixed $x$, and $y_{\lambda, \boldsymbol{\alpha}}^*$ as in \cref{{eq:def_y_lambda_star}}. Then under \cref{assumption:linEq_smoothness,item:assumption_safe_constraints}, we have: 
\begin{align*}%\label{eqn:gradient-approximation}
   & \norm{\nabla_x F(x) - \nabla_x \mathcal{L}_{\lambda, \boldsymbol{\alpha}}(x, y_{\lambda, \boldsymbol{\alpha}}^*)} \leq O({\alpha_1^{-1}}) + O({\alpha_1^{-1/2}\alpha_2^{-1/2}}) + O({\alpha_1^{1/2}}{\alpha_2^{-1/2}}) + O({\alpha_1^{-3/2}}{\alpha_2^{1/2}}).
\end{align*}
\end{restatable}
The proof can be found in \cref{appendix:proof-of-inexact-gradient}. % , which is based on bounding the gradient differences by function smoothness, primal solution and LL solution gap, and the penalty violation given by ~\cref{thm:solution-bound}.
% Given Theorem~\ref{thm:diff_in_hypergrad_and_gradLagr}, we notice that $O(\frac{1}{\alpha_1^{1/2}\alpha_2^{1/2}})$, $O(\frac{\alpha_1^{1/2}}{\alpha_2^{1/2}})$, and $O(\frac{\alpha_2^{1/2}}{\alpha_1^{3/2}})$ are the dominating terms in the upper bound. Therefore, by setting $\alpha_1 = \alpha$ and $\alpha_2 = \alpha^2$, we can minimize their dependency on $\alpha$ and get the following theorem:
% \begin{corollary}\label{thm:hypergradient-approximation}
% With \cref{thm:diff_in_hypergrad_and_gradLagr} in hand, we can choose $\alpha_1 = \alpha^2$ and $\alpha_2 = \alpha^4$ to get:
% \begin{align*}
%     \norm{\nabla_x F(x) - \nabla_x \mathcal{L}_{\lambda, \boldsymbol{\alpha}}(x, y_{\lambda, \boldsymbol{\alpha}}^*)} \leq O({\alpha^{-1}}).
% \end{align*} \pswt{commenting out since this is now part of the next proof}
% \end{corollary} 
With this hypergradient approximation guarantee, we design \cref{alg:inexact-gradient-oracle} to compute an inexact gradient oracle for the hyperobjective $F$.
\begin{algorithm}[h]\caption{Inexact Gradient Oracle for General Inequality Constraints}\label{alg:inexact-gradient-oracle}
\begin{algorithmic}[1]
\State \textbf{Input:}
Upper level variable $x$, accuracy $\alpha$, penalty parameters $\alpha_1 = {\alpha^{-2}}, \alpha_2 = {\alpha^{-4}}$.
\State Compute $y^*$, $\lambda$, and active constraints $\mathcal{I}$ of the constrained LL problem $\min_{y: h(x,y) \leq 0} g(x,y)$. \label{line:inner-optimization-problem} % $\min\limits_{y: h(x,y) \leq 0} g(x,y)$ to obtain a primal solution $y^*$ and a dual solution $\lambda$.
\State Define penalty function $\mathcal{L}_{\lambda, \boldsymbol{\alpha}}(x,y)$ by ~\cref{eqn:penalty-lagrangian}
\State Compute the minimizer $y^*_{\lambda, \boldsymbol{\alpha}} = \arg\min\nolimits_{y} \mathcal{L}_{\lambda, \boldsymbol{\alpha}}(x,y)$ (as in ~\cref{eq:def_y_lambda_star}).\label{line:lagrangian-optimization}
\State \textbf{Output:} $\widetilde{\nabla}_x F \coloneqq \nabla_x \mathcal{L}_{\lambda, \boldsymbol{\alpha}}(x,y^*_{\lambda, \boldsymbol{\alpha}})$. % \pswt{It would be good to cref an equation where this gradient is explicitly stated in terms of gradients of $f$,$g$, $h$, thus showing that this is truly first-order.}
\end{algorithmic}
\end{algorithm}

==> src/inequalitySetting-inexact-grad-oracle-cost.tex <==
% \subsection{Algorithm of Smooth Inexact Gradient Oracle}
% Given $x$, based on Theorem~\ref{thm:hypergradient-approximation}, we can design the following algorithm to compute an inexact gradient oracle to compute an approximate gradient to the gradient of the hyperobjective $F(x)$.

\begin{restatable}[]{theorem}{computationCostInequality}\label{thm:cost_of_computing_ystar_gammastar_inequality}
    Given any accuracy parameter $\alpha > 0$, \cref{alg:inexact-gradient-oracle} outputs $\widetilde{\nabla}_x F(x)$ such that $\|\widetilde{\nabla}_x F(x) - \nabla_x F(x)\| \leq \alpha$ within $\widetilde{O}({\alpha^{-1}})$ gradient oracle evaluations. 
    % \pswt{perhaps change $\alpha$ to something else since we now use $\alpha$ as the penalty parameter multiplier}
\end{restatable}
\begin{proof}[Proof sketch (full proof in \cref{appendix:cost_of_computing_ystar_gammastar_inequality})]
    By choosing 
    % \pswt{change $\lambda$ to $\alpha$ and $\alpha$ to something else} \kai{Fixed it. My plan is to keep $\alpha$ as both penalty parameter and accuracy.} 
    the penalty parameters $\alpha_1 = \alpha^{-2}$ and $\alpha_2 = \alpha^{-4}$, ~\cref{thm:diff_in_hypergrad_and_gradLagr} guarantees the inexactness of the gradient oracle is upper bounded by $O(\alpha)$.
    For the LL problem in \cref{alg:inexact-gradient-oracle}, we use prox-method~\cite{nemirovski2004prox,golowich2020last} to find a dual solution $\lambda$ that is $\alpha$ close to the optimal dual solution using $O(1/\alpha)$ oracles.
    For the penalty minimization, the objective $\mathcal{L}$ is strongly convex but with a poor condition number $\kappa_\mathcal{L} = O(1 / \alpha^2)$ due to strong convexity $O(\alpha_1 \mu_g) = O( {\alpha^{-2} \mu_g})$ and smoothness $O(\alpha_2 C_h) = O(\alpha^{-4})$. This leads to $O(\sqrt{\kappa_\mathcal{L}} \log \| \alpha^{-1} \|) = \widetilde{O}({\alpha^{-1}})$ iterations to converge to $\alpha$ accuracy using standard accelerated methods.
    
    Using these error bounds, we can bound the error propagation of the inexact dual solution $\lambda$, inexact primal solution $y^*_{\lambda,\alpha}$, and inexact gradient oracle using \cref{thm:diff_in_hypergrad_and_gradLagr} by total error $O(\alpha)$.
    Therefore, putting all together, we only need $O(1/\alpha)$ oracle calls and can maintain $O(\alpha)$ inexactness.
\end{proof}

% \subsection{Convergence rate analysis}
% \begin{theorem}
%     Given \cref{thm:cost_of_computing_ystar_gammastar_inequality}, \cref{thm:cost_of_y_lambda_star_inequality}, and \cref{thm:Lipschitz-min-with-inexact-grad-oracle}, we can show that the algorithm converges...
% \end{theorem}

==> src/inexact_gradient_oracle_algorithm.tex <==
\section{Nonsmooth nonconvex optimization with inexact  oracle}\label{sec:nonsmooth}
We now shift gears from the case of linear \emph{equality} constraints to that of linear \emph{inequality} constraints. Specifically, defining $h(x,y)=Ax-By-b$,  the problem we now consider is 
\begin{align}\label[prob]{prob:ineq}
     \mathop{\text{minimize}}\nolimits_{x} ~ F(x) \coloneqq f(x, \ystar(x)) \quad \text{ subject to} ~\ystar(x)\in \argmin\nolimits_{y: h(x, y) \leq 0} g(x, y). 
\end{align}
As noted earlier, for this larger problem class, the hyperobjective $F$ can be nonsmooth nonconvex, necessitating  our measure of convergence to be the now popular notion of Goldstein stationarity~\cite{zhang2020complexity}. 

Our first algorithm for solving \cref{prob:ineq}  is  presented in \cref{alg: IZO}, with its convergence guarantee in \cref{thm:izo_complete_guarantees}.
At a high level, this algorithm first obtains access to an inexact zeroth-order oracle to $F$ (we shortly explain how this is done) and uses this oracle to construct a (biased) gradient estimate of $F$. It then uses this gradient estimate to update the iterates with a rule motivated by  recent works reducing nonconvex optimization to online optimization~\cite{cutkosky2023optimal}. We explain this in \cref{sec:ncns_inexact_ZO}. 


\begin{algorithm}[h]
\begin{algorithmic}[1]\caption{Nonsmooth Nonconvex Algorithm with Inexact Zero-Order oracle}\label{alg: IZO}
\State \textbf{Input:}
Initialization $x_0\in\reals^d$, clipping parameter $D>0$,
step size $\eta>0$, smoothing parameter $\rho>0$, accuracy parameter $\nu>0$,
iteration budget $T\in\NN$, inexact zero-order oracle $\tF:\reals^d\to\reals$.
\State \textbf{Initialize:} ${\Delta}_1=\mathbf{0}$
\For{$t=1,\dots,T$}
\State Sample $s_t\sim\Unif[0,1]$,~~$w_t\sim\Unif(\S^{d-1})$
\State $x_t=x_{t-1}+{\Delta}_t$, ~~$z_t=x_{t-1}+s_t{\Delta}_t$
\State $\tbg_t=\tfrac{d}{2\rho}(\tF(z_t+\rho w_t)-\tF( z_t-\rho w_t))w_t$
\State ${\Delta}_{t+1}
=\mathrm{clip}_{D}\left({\Delta}_t-\eta\tbg_t\right) 
$
\Comment{$\mathrm{clip}_D(z):=\min\{1,\tfrac{D}{\norm{z}}\}\cdot z$}
\EndFor
\State $M=\lfloor\frac{\nu}{D}\rfloor,~K=\lfloor\frac{T}{M}\rfloor$
\For{$k=1,\dots,K$}
\State $\overline{x}_{k}=\frac{1}{M}\sum_{m=1}^{M} z_{(k-1)M+m}$
\EndFor
\State Sample $ x^{\out}\sim\Unif\{\overline{ x}_1,\dots,\overline{ x}_{K}\}$
\State \textbf{Output:} $ x^{\out}$. 
\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{thm:izo_complete_guarantees}
    Consider \cref{{prob:ineq}} under \cref{assumption:linEq_smoothness,assumption:ineq_mild}.  Let $\kappa=C_g/\mu_g$ be the condition number of $g$. Then combining  the procedure for \cref{{lem:ZeroOrderApprox}}
with \cref{alg: IZO} run with 
$\rho=\min\left\{\tfrac{\delta}{2},\tfrac{F(x_0)-\inf F}{L_fL_y}\right\},\nu=\delta-\rho,~D=\Theta\left(\frac{\nu\epsilon^2\rho^2}{d_x\rho^2 L_f^2L_y^2+\alpha^2 d_x^2}\right)$, and $\eta=\Theta\left(\frac{\nu\epsilon^3\rho^4}{(d_x\rho^2L_f^2L_y^2+\alpha^2d_x^2)^2}\right)$ 
outputs $x^{\out}$ such that $\E[\mathrm{dist}(0,{\partial}_\delta F(x^{\out}))]\leq\epsilon+\alpha$ with $T$ { oracle calls to } $f$ { and } $g$, where:
\[T=
O\left(\frac{\sqrt{\kappa}d_x(F(x_0)-\inf F)}{\delta\epsilon^3}\cdot \left(L_f^2L_y^2+\alpha^2 \left(\frac{d_x}{\delta^{2}}+\frac{d_x L_f^2L_y^2}{(F(x_0)-\inf F)^2}\right)\right)\cdot\log(L_f/\alpha)\right).
\]  
\end{theorem}
\Cref{alg: IZO} is a variant of gradient descent with momentum and clipping, with $\widetilde{g}_t$ the inexact gradient, $\Delta_t$ a clipped accumulated gradient (hence accounts for past gradients, which serve as a momentum), and  the clipping ensuring that consecutive iterates of the algorithm reside within a $\delta$-ball of each other. While similar algorithms have appeared in prior work on nonsmooth nonconvex optimization (e.g.~\cite{cutkosky2023optimal}), none of them account for inexactness in the gradient, crucial in our setting.

\subsection{Nonsmooth nonconvex optimization with inexact zeroth-order oracle}\label{sec:ncns_inexact_ZO}
We can obtain inexact zeroth-order oracle access to $F$  because (as formalized in \cref{lem:ZeroOrderApprox}) despite potential nonsmoothness and nonconvexity of  $F$ in \cref{prob:ineq},  estimating its \emph{value} $F(x)$  at any point $x$ amounts to solving a single smooth and strongly convex optimization problem, which can be done can be done in $\widetilde{O}(1)$ oracle calls to $f$ and $g$ by appealing to a result by \citet{zhang2022solving}.

\begin{restatable}[Proof in \Cref{{sec:zeroth-order-algs}}]{lemma}{lemZeroOrderApprox}\label{lem:ZeroOrderApprox}
    Given any $x$, we can return $\widetilde{F}(x)$ such that $|F(x)-\widetilde{F}(x)|\leq\alpha$ using $O(\sqrt{C_g/\mu_g}\log(L_f/\alpha))$ first-order oracle calls to $f$ and $g$.
\end{restatable}


Having computed an inexact value of the  hyperobjective $F$, we now show how to use it to develop an algorithm for solving  \cref{{prob:ineq}}. To this end, we first note that  $F$, despite being 
 possibly nonsmooth and nonconvex, is Lipschitz and hence amenable to the use of recent algorithmic developments  in nonsmooth nonconvex optimization pertaining to Goldstein stationarity. 
\begin{restatable}{lemma}{lemLipscConstrBilevel}\label{lem:LipscConstrBilevel}Under \cref{assumption:linEq_smoothness} and \ref{item:assumption_safe_constraints}, $F$ in  \cref{{prob:ineq}} is $O(L_fL_y)$-Lipschitz in $x$.
\end{restatable}

\looseness=-1With this guarantee on the Lipschitzness of $F$, we prove \cref{{thm: Lipschitz-min-with-inexact-zero-oracle}} for attaining Goldstein stationarity using the inexact zeroth-order oracle of a Lipschitz function. Our proof of \cref{{thm: Lipschitz-min-with-inexact-zero-oracle}} crucially uses the recent online-to-nonconvex framework of \citet{cutkosky2023optimal}. Combining \cref{lem:ZeroOrderApprox} and \cref{thm: Lipschitz-min-with-inexact-zero-oracle} then immediately implies \cref{thm:izo_complete_guarantees}. 

% \begin{theorem}\label{thm: Lipschitz-min-with-inexact-zero-oracle}
% Suppose $F:\reals^d\to\reals$ is $L$-Lipschitz, 
% and that $|\widetilde{F}(\cdot)-F(\cdot)|\leq\alpha$.
% Then running \cref{alg: IZO} with
% $\rho=\min\left\{\tfrac{\delta}{2},\tfrac{F(x_0)-\inf F}{L}\right\},\nu=\delta-\rho,~D=\Theta\left(\frac{\nu\epsilon^2\rho^2}{d\rho^2 L^2+\alpha^2 d^2}\right),\eta=\Theta\left(\frac{\nu\epsilon^3\rho^4}{(d\rho^2L^2+\alpha^2d^2)^2}\right)$,
% outputs a point $x^{\out}$ such that $\E[\mathrm{dist}(0,{\partial}_\delta F(x^{\out}))]\leq\epsilon+\alpha$ with
% \[T=
% O\left(\frac{d(F(x_0)-\inf F)}{\delta\epsilon^3}\cdot \left(L^2+\alpha^2 (\frac{d}{\delta^{2}}+\frac{dL^2}{(F(x_0)-\inf F)^2})\right)\right)
% \text{ calls to } \tF(\cdot).\] 
% \end{theorem}


\subsection{Nonsmooth nonconvex optimization with inexact \emph{gradient}  oracle}
In \cref{{sec:inequality-bilevel}}, we provide a way to generate approximate gradients of $F$. Here, we present an algorithm that attains Goldstein stationarity of \cref{prob:ineq} using this inexact gradient oracle.  While there has been a long line of recent work on algorithms for nonsmooth nonconvex optimization with convergence to Goldstein stationarity~\cite{zhang2020complexity, davis2022gradient, jordan2023deterministic, kong2023cost, grimmer2023goldstein}, these results necessarily require \textit{exact} gradients. 
This brittleness to any error in gradients renders them ineffective in our setting, where our computed (hyper)gradient necessarily suffers from an
additive error.
While inexact oracles are known to be effective for smooth or convex objectives \citep{devolder2014first}, utilizing inexact gradients in the nonsmooth nonconvex regime presents a nontrivial challenge.
Indeed, without any local bound on gradient variation due to smoothness, or convexity that ensures that gradients are everywhere correlated with the direction pointing at the minimum, it is not clear a priori how to control the accumulating price of inexactness throughout the run of an algorithm.
To derive such results, we  use the recently proposed connection between online learning and nonsmooth nonconvex optimization by \citet{cutkosky2023optimal}. By controlling the accumulated error suffered by online gradient descent for \emph{linear} losses (cf. \cref{lem: inexact OGD}), 
we derive guarantees for our setting of interest, providing Lipschitz optimization algorithms that converge to Goldstein stationary points even with inexact gradients.  


This algorithm matches the best known complexity in first-order nonsmooth nonconvex optimization \cite{zhang2020complexity,davis2022gradient,cutkosky2023optimal}, merely replacing the convergence to a $(\delta,\epsilon)$-stationary point by $(\delta,\epsilon+\alpha)$-stationarity, where $\alpha$ is the inexactness of the gradient oracle.

\begin{algorithm}[h]
\begin{algorithmic}[1]\caption{Nonsmooth Nonconvex Algorithm with Inexact Gradient Oracle}\label{alg: OIGRM}
\State \textbf{Input:}
Initialization $x_0\in\reals^d$, clipping parameter $D>0$,
step size $\eta>0$,
accuracy parameter $\delta>0$,
iteration budget $T\in\NN$, inexact gradient oracle $\widetilde{\nabla}F:\reals^d\to\reals^d$.
\State \textbf{Initialize:} ${\Delta}_1=\mathbf{0}$
\For{$t=1,\dots,T$}
\State Sample $s_t\sim\Unif[0,1]$ 
\State $x_t=x_{t-1}+{\Delta}_t$, ~~$z_t=x_{t-1}+s_t{\Delta}_t$
\State $\tbg_t=\widetilde{\nabla}F(z_t)$
\State ${\Delta}_{t+1}
=\mathrm{clip}_{D}\left({\Delta}_t-\eta\tbg_t\right) 
$
\Comment{$\mathrm{clip}_D(z):=\min\{1,\tfrac{D}{\norm{z}}\}\cdot z$}
\EndFor
\State $M=\lfloor\frac{\delta}{D}\rfloor,~K=\lfloor\frac{T}{M}\rfloor$
\For{$k=1,\dots,K$}
\State $\overline{x}_{k}=\frac{1}{M}\sum_{m=1}^{M} z_{(k-1)M+m}$
\EndFor
\State Sample $ x^{\out}\sim\Unif\{\overline{ x}_1,\dots,\overline{ x}_{K}\}$
\State \textbf{Output:} $ x^{\out}$. 
\end{algorithmic}
\end{algorithm}


\begin{restatable}{theorem}{thmLipscMinWithInexactGradOracle}\label{thm:Lipschitz-min-with-inexact-grad-oracle}
Suppose $F:\reals^d\to\reals$ is $L$-Lipschitz  
and that $\|\widetilde{\nabla} F(\cdot)-\nabla F(\cdot)\|\leq\alpha$. 
Then running \cref{alg: OIGRM} with
$D=\Theta(\frac{\delta\epsilon^2}{L^2}),\eta=\Theta(\frac{\delta\epsilon^3}{L^4})$,
outputs a point $x^{\out}$ such that $\E[\mathrm{dist}(0,{\partial}_\delta F(x^{\out}))]\leq\epsilon+\alpha$, with
$T=O\left(\frac{(F(x_0)-\inf F) L^2}{\delta\epsilon^3}\right)$
calls to $\widetilde{\nabla}F(\cdot)$.
\end{restatable}

We defer the proof of \cref{thm:Lipschitz-min-with-inexact-grad-oracle} to \cref{{sec:zeroth-order-algs}}.
Plugging the complexity of computing inexact gradients,
as given by \cref{thm:cost_of_computing_ystar_gammastar_inequality},
into the result above,
we immediately obtain convergence to a $(\delta,\epsilon)$-stationary point of \cref{prob:general-constraints} with $\widetilde{O}(\delta^{-1}\epsilon^{-4})$ gradient calls overall.



\paragraph{Implementation-friendly algorithm.}
While \cref{{alg: OIGRM}} matches the best-known results in nonsmooth nonconvex optimization, it could be  impractical  due to several hyperparameters which need tuning. 
Arguably, a more natural application of the hypergradient estimates would be simply plugging them into gradient descent, which requires tuning only the stepsize. Since  $F$ is neither smooth nor convex, perturbations are required to guarantee differentiability along the trajectory.
We therefore complement \cref{thm:Lipschitz-min-with-inexact-grad-oracle} by analyzing perturbed (inexact) gradient descent  in the nonsmooth nonconvex setting (\cref{{alg: PIGD}}) and state its theoretical guarantee in \Cref{thm:practical_Lipschitz-min-with-inexact-grad-oracle}. Despite its suboptimal worst-case theoretical guarantees, we find this algorithm  easier to implement in practice. 


==> src/intro.tex <==
\section{Introduction}\label{sec:introduction}
Bilevel optimization~\cite{bracken1973mathematical, colson2007overview,bard2013practical,sinha2017review}, an important problem in optimization, is defined as follows:
\begin{align*}\numberthis\label[prob]{prob:general-constraints}
     \mbox{minimize}_{x\in \mathcal{X}} ~ F(x) \coloneqq f(x, \ystar(x)) \text{ subject to } ~\ystar(x)\in \arg\min\nolimits_{y\in S(x)} g(x, y).
\end{align*}
Here, the value of the upper-level problem at any point $x$ depends on the solution of the lower-level problem. This framework has recently found numerous applications in meta-learning~\cite{ snell2017prototypical, bertinetto2018meta, rajeswaran2019meta, ji2020convergence}, hyperparameter optimization~\cite{franceschi2018bilevel, shaban2019truncated, feurer2019hyperparameter}, and 
% continual learning~\cite{borsos2020coresets, pham2020contextual}, 
reinforcement learning~\cite{konda1999actor, sutton2018reinforcement, hong2020two,zhang2020bi}.
% , and signal processing~\cite{, , }.  
Its growing importance has spurred increasing efforts towards designing computationally efficient algorithms for it. 

As demonstrated by \cite{ghadimi2018approximation}, a key computational step in algorithms for bilevel optimization is estimating ${dy^*(x)}/{dx}$, the gradient of the lower-level solution. This gradient estimation problem has been extensively studied in differentiable optimization~\cite{amos2017optnet,agrawal2019differentiable} by applying the implicit function theorem to the KKT system of the given problem% , a technique which has found many applications in end-to-end learning \pswt{commenting out to keep the focus on the difficulty of computing the gradient}
~\cite{donti2017task,wilder2019melding,kotary2021end,lee2019meta,tang2022pyepo,bai2019deep}.
However, this technique typically entails computing (or estimating) second-order derivatives, which can be prohibitive in high dimensions~\cite{mehra2021penalty, ji2021bilevel,wang2021learning}.

Recently, \cite{liu2022bome} made a big leap forward towards addressing this computational bottleneck.  %\jz{I would not say that.}
% and is therefore not fully first-order. The convergence of first-order method using differentiable optimization is also under-investigated.
Restricting themselves to the class of unconstrained bilevel optimization, they proposed a fully first-order method with finite-time stationarity guarantees. While a remarkable breakthrough,  \cite{liu2022bome} does not directly extend to the important setting of \textit{constrained} bilevel optimization. This motivates the question: 
\begin{quote}
\centering
    \emph{Can we develop a fully first-order algorithm for constrained bilevel optimization?}
\end{quote}
Besides being natural from the viewpoint of complexity theory, this question is well-grounded
in applications, including Stackelberg models~\cite{simaan1973stackelberg,paruchuri2008playing,chu2014integrated} and mechanism design~\cite{wang2022coordinating,dutting2021optimal},  urban planning~\cite{miao2010modeling,kang2010bilevel} and resource allocation~\cite{xu2013bilevel,gutjahr2016bi,zhang2010bilevel,fathollahi2022bi}, and decision-making under uncertainty~\cite{elmachtoub2022smart,munoz2022bilevel,wilder2019melding}.
% \pswt{State a few constrained blo applications.} 
Our primary contribution is an affirmative answer to the highlighted question. While there have been some other recent works~\cite{khanduri2023linearly, yao2024constrained, lu2024firstorder} on this problem, 
 we believe our notion of stationarity more directly addresses the problem at hand
 % , 
% \jz{rephrase}\pswt{done!}
(cf. \cref{sec:related_work}).  We now summarize our contributions.
% \pswt{filler text just to see how much more space we have filler text just to see how much more space we have filler text just to see how much more space we have filler text just to see how much more space we have filler text just to see how much }
% , we answer this question affirmatively. 
% \pswt{motivate constrained bilevel as well as first-order, pose the question we answer (efficient FO constrained BLO), and segue into the next subsection}
% $S$ is a constraint set for the LL variable $y$ 

\subsection{Our contributions}\label{sec:introduction_main_results}
% We provide the following algorithmic results for constrained bilevel programs.
% \, supplementing our theory with numerical experiments.
% Our contributions can be summarized as follows:
\begin{description}[style=unboxed,leftmargin=0cm, itemsep=.5em, parsep=.3em, topsep=.5em]
\item [{(1)}] \textbf{Convex inequality constraints.} As our first contribution, we design fully first-order algorithms for solving \cref{prob:general-constraints} where the lower-level constraint set $S(x):=\left\{y:h(x,y)\leq0\right\}$  is described by convex inequality constraints, and the upper-level variable is unconstrained. 
By ``fully first-order'', we mean that we use only zeroth and first order oracle access to $f$, $g$, and $h$. 


Our measure of convergence of these algorithms is that of $(\delta,\epsilon)$-stationarity~\cite{goldstein1977optimization}: for a Lipschitz function, we say that a point $x$ is $(\delta,\epsilon)$-stationary if within a $\delta$-ball around $x$ there exists a convex combination of subgradients of the function with norm at most $\epsilon$ (cf. \cref{def:GoldsteinDeltaEpsStationary}). 

\looseness=-1To motivate this notion of convergence, we note that the hyperobjective $F$ (in \cref{prob:general-constraints}) as a function of $x$ could be nonsmooth and nonconvex (and is Lipschitz, as  we later prove). Minimizing such a function in general is well-known to be intractable~\cite{nemirovskij1983problem}, necessitating local notions of stationarity. Indeed, not only is it impossible to attain $\epsilon$-stationarity in finite time~ \cite{zhang2020complexity}, even getting \textit{near} an
approximate stationary point of an arbitrary Lipschitz function is impossible unless
the number of queries has an exponential dependence on the dimension~\cite{kornowski2022oracle}. Consequently, for this function class, $(\delta, \epsilon)$-stationarity has recently emerged to be a natural and algorithmically tractable notion of stationarity~\cite{zhang2020complexity}. We give the following guarantee under  regularity assumptions on $f$, $g$, $h$, and $y^*$. 
% \pswt{is there a word to describe the assumption on $dy^*/dx$ without going into the math? like "constraint qualification" or something?}
% Our algorithm ensures that we converge to a point that satisfies $(\delta,\epsilon)$-stationarity for $F$ in $O(\delta^{-1}\epsilon^{-3})$ iterations, each iteration costing $O(\epsilon^{-1})$.  
\begin{theorem}[Informal; \cref{thm:Lipschitz-min-with-inexact-grad-oracle} combined with \cref{thm:cost_of_computing_ystar_gammastar_inequality}]
    Given \cref{prob:general-constraints} with convex inequality constraints $S(x)=\left\{y:h(x,y)\leq0\right\}$ and unconstrained upper-level variable, under  regularity assumptions on $f$, $g$, $h$, and $y^*$ (\cref{assumption:linEq_smoothness,item:assumption_safe_constraints}), there exists an algorithm, which in $\widetilde{O}(\delta^{-1}\epsilon^{-4})$ oracle calls to $f$, $g$, and $h$, converges to a $(\delta, \epsilon)$-stationary point for $F$. 
\end{theorem} To the best of our knowledge, this is the first result to achieve fully first-order finite-time $(\delta,\epsilon)$-stationarity of the hypergradient for constrained bilevel optimization (cf. \cref{sec:related_work} for a discussion of \cite{yao2024constrained}, which recently solved a related problem). 
To this end, we begin by carefully reformulating \cref{prob:general-constraints} via the penalty method and constructing a fully first-order inexact gradient oracle for the hyperobjective $F$ (cf. \cref{sec:inequality-bilevel}). We then employ this inexact gradient oracle within {an algorithm (\cref{{alg: OIGRM}}) designed to minimize Lipschitz nonsmooth nonconvex functions}
(in particular, $F$). Our proposed algorithm offers the following convergence guarantee.
\begin{theorem}[Informal; \cref{{thm:Lipschitz-min-with-inexact-grad-oracle}}]
    Given Lipschitz $F:\reals^d\to\reals$ 
    % be Lipschitz  
% $F(\bx_0)-\inf F\leq \Delta$
and $\|\widetilde{\nabla} F(\cdot)-\nabla F(\cdot)\|\leq\epsilon$,
% Under the same setting as \citep[Theorem 7.2]{chen2023bilevel},
% suppose that $\mathrm{SGM}$ (as in \citep[Theorem 7.1]{chen2023bilevel}) is set so that $|\tF(\cdot)-\varphi(\cdot)|\leq \zeta$ for $\zeta=\Theta(\delta\epsilon/d)$.
 there exists an algorithm that, in 
% $x^{\out}$ such that $\E[\mathrm{dist}(0,{\partial}_\delta F(x^{\out}))]\leq\epsilon+\alpha$, with
$T=O(\delta^{-1}\epsilon^{-3})$
calls to $\widetilde{\nabla}F$,
% Then running \cref{alg: OIGRM} with
% $D=\Theta\left(\frac{\delta\epsilon^2}{L^2}\right),\eta=\Theta\left(\frac{\delta\epsilon^3}{L^4}\right),\nu=\delta$,
outputs a $(\delta,2\epsilon)$-stationary point of $F$.
% \pswt{Make level of detail of runtime consistent across all inf. theorems}
\end{theorem} While such algorithms using  \emph{exact} gradients already exist~\cite{zhang2020complexity, davis2022gradient}, extending them to the inexact gradient  setting is non-trivial; we leverage recent ideas connecting online learning to nonsmooth nonconvex optimization~\cite{cutkosky2023optimal} (cf. \cref{{sec:nonsmooth}}). With the ubiquity of nonsmooth nonconvex  optimization problems associated with
training modern neural networks, we believe our analysis for this general task can be of independent interest to the broader optimization community.  


% \pswt{motivate this with experiments} 
We also design variants  of the aforementioned algorithm, one of which converges in $\widetilde{O}(d_x \delta^{-1}\epsilon^{-3})$ gradient calls, thus trading off an $\epsilon^{-1}$ factor for a linear dependence on the upper dimension $d_x$, while another is 
% trading off
% Finally, we present a 
more implementation-friendly
% version of this algorithm,
with slightly worse worst-case guarantee (cf. \cref{sec:nonsmooth}).
% for full details).
% \pswt{Guy: would you be able to say a bit more about these?} \gk{Added a brief, what do you think?} <sg!

\item[{(2)}] \textbf{Linear equality constraints.} Next, we study the special setting of \cref{prob:general-constraints} with $S(x):=\left\{y:Ax - By-b=0\right\}$ a linear equality constraint and $\mathcal{X}$ a convex compact set. With appropriate regularity assumptions on $f$ and $g$, the hyperobjective $F$ in this case is smooth as a function of $x$. Inspired by ideas from \cite{kwon2023fully}, we use implicit differentiation of the KKT matrix of a slightly perturbed version of the lower-level problem to design a fully-first order approximation to $\nabla F$. With this inexact gradient oracle in hand,  we then run projected gradient descent, which converges in $\widetilde{O}(\epsilon^{-2})$ iterations for smooth functions. Constructing our first-order approximation entails solving a strongly convex optimization problem on affine constraints, which can be done efficiently (cf. \cref{sec:equality-bilevel}). 
% at a linear rate; therefore,  our total cost for achieving $\epsilon$-stationarity of $F$ is nearly-optimal at $\widetilde{O}(\epsilon^{-2})$. 

\begin{theorem}[Informal; cf. \cref{thm:lineq-cost}]
\label{thm:lineq-cost-inf}
    Given \cref{prob:general-constraints} with linear equality constraints $S(x)=\left\{y:Ax-By-b=0\right\}$ and $\mathcal{X}$ a convex compact set, under regularity assumptions on $f$ and $g$ (\cref{assumption:linEq_smoothness,assumption:eq}), there exists an algorithm, which in $\widetilde{O}(\epsilon^{-2})$  oracle calls to $f$ and $g$, converges to an $\epsilon$-stationary point of $F$. 
\end{theorem}

The current result in literature for the linearly constrained setting is that of \cite{khanduri2023linearly}, which 
involves expensive Hessian computations and 
imposes on the hyperobjective $F$ some \textit{strong regularity assumptions} that are, in general, impossible to verify.
In contrast,  we impose \textit{assumptions solely on the constituent functions $f$ and $g$} (and none directly on $F$), which can be easily verified by the user of our algorithms.
Thus, \Cref{thm:lineq-cost-inf} makes substantial progress on these two fronts.
See \cref{sec:equality-bilevel} for details. 
% \pswt{Make this distinction clearer since it's quite big, imo filler text  filler text  filler text  filler text  filler text  filler text  filler text  filler text  filler text  filler text  filler text  filler text }


% \pswt{A line about the previous best result for lineq}
\end{description}

==> src/linearEquality.tex <==
\section{Lower-level problem with linear equality constraint}\label{sec:equality-bilevel}
\looseness=-1Shifting our focus from bilevel programs with general convex inequality constraints, we now turn to obtaining improved results for the specialized setting of bilevel programs with  \textit{linear equality }constraints in the lower-level problem, a problem often arising in adversarial training, decentralized meta learning, and sensor networks~(see \cite{khanduri2023linearly} and the discussion therein). Our formal problem statement is:   
\begin{align*}\numberthis\label[prob]{prob:lin-eq}
     & \mbox{minimize}_{x\in \mathcal{X}} ~ F(x) \coloneqq f(x, \ystar(x))~\text{ subject to } ~\ystar(x)\in \arg\min\nolimits_{y: h(x, y) = 0} g(x, y), 
\end{align*}
% \[
% \begin{array}{ll}
%      \mbox{minimize}_{x\in \mathcal{X}} & F(x):= f(x, \ystar(x))  \\
%      \mbox{subject to } & \ystar(x)\in \arg\min_{y: h(x, y) = 0} g(x, y), 
% \end{array} \numberthis\label[prob]{prob:lin-eq}
% \] 
where $f$, $g$, $h$, and $\mathcal{X}$ satisfy
% the 
% the properties in
satisfy 
\cref{assumption:linEq_smoothness,assumption:eq}.
% \pswt{and ...}. 

% \begin{assumption}\label{assumption:linEq_smoothness} 
% We study \cref{prob:lin-eq} under the following assumptions. 
% \begin{assumpenum}
% \compresslist{
% \item\label[assum]{item:assumption_lineq_first} Upper-level: The objective $f$  is $C_f$-smooth in $x,y$ jointly, i.e., $\norm{\nabla f(x_1,y_1) - \nabla f(x_2,y_2)} \! \leq C_f \norm{(x_1,y_1) - (x_2, y_2)}$ and $L_f$-Lipschitz in $y$. The constraint $\mathcal{X}$ is a convex compact set. 
%     \item Lower-level: The objective $g$ is second-order smooth with parameter $C_g$ and $\mu_g$-strongly convex in $y$. The constraint $h(x,y)=Ax-By-b$ has  $B$ being full row rank. \jz{Maybe we could justify the full rankness by complete recourse. That is, for any given $x$, there exists some $y$ to make the LL program feasible. I am wondering if we need that assumption for the inequality case? }
% }
% \end{assumpenum}
% \end{assumption}
\looseness=-1The previous best result on \cref{{prob:lin-eq}}~\cite{khanduri2023linearly} provided finite-time guarantees under regularity assumptions on $F$, while also requiring Hessian computations. In contrast, our finite-time guarantees \emph{require assumptions only on $f$ and $g$, not on $F$};
indeed, in our work, these desirable properties of $F$ are naturally implied by our analysis. 
Specifically, our key insight is that the hypergradient $\grad F(x):=\grad_{x}f(x,y^{*})+\left({d y^*(x)}/{dx}\right)^\top\grad_{y}f(x,y^{*})$ for  \cref{{prob:lin-eq}} is Lipschitz-continuous and  admits an easily computable --- yet highly accurate --- finite-difference approximation. Therefore, $O(\epsilon^{-2})$ iterations of gradient descent  on $F$ with this finite-difference gradient proxy  yield an $\epsilon$-stationary point. 


Specifically, for any fixed $x\in \mathcal{X}$, our proposed finite-difference gradient proxy approximating $\left({d y^*(x)}/{dx}\right)^\top\grad_{y}f(x,y^{*})$ is given
by
% by the 
% left-hand side of the 
% following equation:
% \kai{Change dual solution $\lambda^*$ to $\gamma$?}
% , approximating the implicit gradient term up to a $O(\delta)$-additive error:
 \[ v_x := {\frac{\nabla_{x}[g(x,\ystardel)+\langle\lamdeltar, h(x,\ystar)\rangle]-\nabla_{x}[g(x,y^{*})+\langle\lamstar, h(x,y^{*})\rangle]}{\delta}
 % = \frac{d y^*(x)}{dx}\grad_{y}f(x,y^{*}(x))+O(\delta) 
 \numberthis\label{eq:part-hypergrad-approx-lin-eq},}\]
where $(\ydelstar,\lamdeltar)$ are the primal and dual solutions to the
 perturbed lower-level problem:
 % for a given $x$
\begin{align}\label{eq:lower_perturb}
    & \ydelstar \coloneqq \arg\min\nolimits_{y: h(x,y) = 0} ~g(x,y)+\delta f(x,y).
\end{align} We show in \cref{{lem:lineq-finitediff-equals-gradf}} that $v$ in \cref{eq:part-hypergrad-approx-lin-eq} approximates $\left({d y^*(x)}/{dx}\right)^\top\grad_{y}f(x,y^{*})$ up to an $O(\delta)$-additive error, implying the gradient oracle construction outlined in 
% $v + \nabla_x f(x,y^*)$ is an $O(\delta)$-additive estimate of $\nabla_x F(x)$, as displayed in 
\cref{alg:LE-inexact-gradient-oracle}.

\begin{algorithm}[h]\caption{Inexact Gradient Oracle for Bilevel Program with Linear Equality Constraint}\label{alg:LE-inexact-gradient-oracle}
\begin{algorithmic}[1]
% \State \jz{state the accuracy we need to solve for the sub-problems}
\State \textbf{Input:}
Current $x$, accuracy $\epsilon$, perturbation $\delta = \epsilon^2$.
\State Compute $y^*$ (as in \cref{prob:lin-eq}) and corresponding optimal dual $\lamstar$ (as in \cref{eqs:kkt-lin-eq})\label{line:LEQ-first}
\State Compute $\ystardel$ (as in \cref{eq:lower_perturb}) and and corresponding optimal dual $\lamdeltar$ (as in \cref{eqs:lineq-kkt-perturbed}) \label{line:LEQ-second} 
% \kai{Same here about dual solution $\lambda^*$?}
\State Compute $v_x$ as in \cref{eq:part-hypergrad-approx-lin-eq} \Comment{Approximates $\left({d y^{*}(x)}/{d x}\right)^\top\nabla_{y}f(x,y^{*})$}
% \pswt{cref a standalone expression}
\State \textbf{Output:} $\widetilde{\nabla} F = v_x + \nabla_x f(x, y^*)$
\end{algorithmic}
\end{algorithm}

Our full implementable algorithm for solving \cref{prob:lin-eq} is displayed in \cref{{alg:LE-full-alg}}.
% \pswt{change to full alg}The method and accuracy requirements of \cref{line:LEQ-first} and \cref{line:LEQ-second} are detailed in \cref{sec:LEQ-cost-computing-ystar-lamstar}. 
Notice that the finite-difference term in \cref{{eq:part-hypergrad-approx-lin-eq}} avoids differentiating through the implicit function $y^*$. Instead, all we need to evaluate it are the values of $(y^*,\lambda^*,\ydelstar,\lamdeltar)$ (and gradients of $g$ and $h$). Since $(y^*,\lambda^*)$ are solutions to a smooth strongly convex linearly constrained  problem, they can be approximated
% may be  obtained
at a linear rate. Similarly, since the approximation error in \cref{eq:part-hypergrad-approx-lin-eq}  is proportional to $\delta$ (cf. \cref{{lem:lineq-finitediff-equals-gradf}}), a  small enough $\delta$ in the perturbed objective $ g+\delta f$ in \cref{eq:lower_perturb} ensures that it is dominated by the strongly convex and smooth $g$, whereby accurate approximates to $(y_\delta^*,\lambda_\delta^*)$ can also be readily obtained. Putting it all together, the proposed finite-difference hypergradient proxy in \cref{eq:part-hypergrad-approx-lin-eq} is  efficiently computable, yielding the following guarantee. 

% \jz{State the assumption on the smallest eigenvalue for the KKT matrix, and remark on why it holds automatically.}

% \jz{I feel it is better to list out all the constant dependences, at the major ones. Like the uniform upper bound on the KKT matrix, the Lipschitz smoothness and continuity constants.}
% \jz{we can only find points with a small gradient mapping, not a small gradient}
\begin{restatable}{theorem}{linEqFullCost}\label{thm:lineq-cost}
    Consider  \cref{prob:lin-eq} under \cref{assumption:linEq_smoothness}, and let $\kappa=C_g/\mu_g$ be the condition number of $g$. Then \cref{alg:LE-full-alg}  finds an $\epsilon$-stationary point (in terms of gradient mapping, see \cref{eq:gradient-mapping}) after $T=\widetilde{O}(C_F (F(x_0)-\inf F)\sqrt{\kappa}\epsilon^{-2})$  oracle calls to $f$ and $g$, where $C_F:= 2(L_f +C_f+C_g)C_H^3 S_g (L_g +\|A\|)^2$ is the smoothness constant of the hyperobjective $F$.
\end{restatable}  
We now sketch the proofs of the key components that together imply \cref{thm:lineq-cost} (cf. \cref{sec:LEQ-main-thm-full-proof}).  
% By an application of the implicit function theorem to the KKT system of \cref{eq:lower_perturb}, we show in \cref{{lem:lineq-finitediff-equals-gradf}} that the variable $\ystardel$  and its corresponding optimal dual variable $\lamdeltar$ can be used to construct an approximation to  $\frac{d}{dx}y^{*}(x)\grad_{y}f(x,y^{*}(x))$, as displayed in \cref{alg:LE-inexact-gradient-oracle}. 
% % The required regularity properties of $\ystardel$ and $\lamdeltar$ for this gradient approximation to hold are essentially satisfied when $f$, $g$, and $h$ satisfy \cref{assumption:linEq_smoothness}.  
% The regularity properties of $f$, $g$, and $h$  from \cref{assumption:linEq_smoothness} also imply smoothness of $F$, as we formally show in \cref{{{thm:lineq-cost}}}; 
% therefore, our inexact gradient oracle of $F$ (via \cref{alg:LE-inexact-gradient-oracle}) allows us to run  $O(\epsilon^{-2})$ iterations of projected gradient descent with an inexact gradient oracle to obtain an $\epsilon$-stationary point for \cref{prob:lin-eq}. 
% Since each iteration of \cref{alg:LE-inexact-gradient-oracle} solves a strongly convex optimization problem over a linear subspace, it costs $O(\sqrt{\kappa})$~\cite{salim2022optimal}, where $\kappa$ is the condition number of $f$, thus giving us a total cost of $O(\sqrt{\kappa}\epsilon^{-2})$ in attaining $\epsilon$-stationarity of \cref{prob:lin-eq}, as formalized in \cref{thm:lineq-cost}.
%%%%%%%%%%%%
\subsection{Main technical ideas}\label{sec:warmup-lin-eq}
% \jz{describe the smoothness result, the local version of which comes from the implicit function theorem.}
% \jz{sketch Lemma 3.3 in a high level, why does these two quantities match in the limit? just show the core of algebra, I don't think we need to spend too much effort in polishing the intuition. It is going to be out-dated pretty soon.ß }
We briefly outline the two key technical building blocks alluded to above, that together give us  \cref{{thm:lineq-cost}}: the approximation guarantee of our finite-difference gradient proxy (\cref{{eq:part-hypergrad-approx-lin-eq}}) and the smoothness of hyperobjective $F$ (for \cref{{prob:lin-eq}}). The starting point for both these results is the following simple observation obtained by implicitly differentiating, with respect to $x$, the KKT system associated with $y^*=\arg\min_{h(x,y)=0} g(x,y)$ and optimal dual variable $\lamstar$: 
% , define $\Leqc(x,y,\lam)=g(x,y)+\lam^\top h(x,y)$: 
 \[ \begin{bmatrix}\frac{d\ystar(x)}{dx}\\
\frac{d\lamstar(x)}{dx}
\end{bmatrix}= {\begin{bmatrix}\grad^2_{yy}g(x,\ystar) & \nabla_y h(x,y^{*})^{\top}\\
\nabla_y h(x,y^{*}) & 0
\end{bmatrix}^{-1}} \begin{bmatrix}-\nabla^2_{yx}g(x,y^{*})\\
-\nabla_x h(x,\ystar)\end{bmatrix} \numberthis\label{eq:def_matrix_H}\]
The invertibility of the matrix in the preceding equation is proved in  \cref{{cor:nonsingularH}}:
% we provide a condition
% for when the matrix $H$ from  \cref{eq:def_matrix_H} is invertible; 
essentially,  invertibility is ensured by strong convexity of $g$ and $\grad_y h(x,y^*)=B$ having full row rank. Further, together with the compactness of $\mathcal{X}$, we obtain that the inverse of the matrix is bounded by some constant $C_H$ (cf. \cref{cor:nonsingularH} for details). 
% , combined with continuity of the inverse function.  

\begin{restatable}{lemma}{lemLineqFiniteDiffEqualsGradF}\label{lem:lineq-finitediff-equals-gradf} 
For  \cref{prob:lin-eq}
under \cref{assumption:linEq_smoothness}, with $v_x$ as in \cref{eq:part-hypergrad-approx-lin-eq}, 
% Assume $h(x,y):=Ay-Bx-b$ with $A$ having full rank. <-included in \cref{prob:lin-eq} maybe put $A$ being full rank in an assumption env for clarity?
% it holds that
the
following holds:
% \pswt{also requires third order smoothness of $g$}
\[
\textstyle{\left\|v_x-\left(\frac{d y^{*}(x)}{d x}\right)^\top\nabla_{y}f(x,y^{*})\right\|\leq O(C_F \delta).}
\]
% \jz{super high accuracy requirement, direct extension to the stochastic setting would be a mess. To go there, we really need to make the algorithm single loop.}
\end{restatable}
\begin{proof}[Proof sketch; see \cref{{sec:appendix_linear_equality}} for the complete proof]
    The main idea for this proof is that the two terms being compared are essentially the same by an application of the implicit function theorem. First, we can use the expression for $\tfrac{dy^*(x)}{dx}$ from \cref{eq:def_matrix_H} as follows: 
\begin{align*}
\left(\frac{d y^{*}(x)}{d x}\right)^\top\nabla_{y}f(x,y^{*})
% &=
% \begin{bmatrix}\nabla_{y}f(x,y^{*}(x)) & 0\end{bmatrix}\begin{bmatrix}\frac{d\ystar}{dx}\\
% \frac{d\lamstar}{dx}
% \end{bmatrix}\\
&=\begin{bmatrix}-\nabla^2_{yx} g(x,y^{*})\\
-\nabla_x h(x,\ystar)
\end{bmatrix}^\top\begin{bmatrix}\nabla^2_{yy} g(x,y^{*}) & \nabla_y h(x,y^{*})^{\top}\\
\nabla_y h(x,y^{*}) & 0
\end{bmatrix}^{-1}\begin{bmatrix}\nabla_{y}f(x,y^{*}) \\ 0\end{bmatrix}.
% \numberthis\label{prop3eq:RHS-mainbody}
\end{align*} We now examine our finite-difference gradient proxy. For simplicity of exposition, we instead consider $\lim_{\delta\rightarrow0}\frac{\nabla_{x}[g(x,\ystardel)+\langle\lamdeltar, h(x,y^*)\rangle]-\nabla_{x}[g(x,y^{*})+\langle\lamstar, h(x,y^{*})\rangle]}{\delta},$ which, by an application of the fundamental theorem of calculus and \cref{assumption:eq}% \pswt{smoothness assumptions}
, equals our finite-difference gradient proxy up to an $O(\delta)$-additive error. Note that this expression  is exactly \[\nabla^2_{xy} g(x,y^*) \frac{d\ydelstar}{d\delta} + \nabla_x h(x,y^*)^\top \frac{d\lamdeltar}{d\delta}.\numberthis\label{eq:LINEQ-lim-findiff}\] Since  $y^*_{\delta}$ is also a minimizer of a strongly convex function over a linear equality constraint \cref{{eq:lower_perturb}}, the same reasoning that yields \cref{eq:def_matrix_H} can be also used to obtain 
\[
\begin{bmatrix}\frac{d\ydelstar(x)}{d\delta}\\
\frac{d\lamdeltar(x)}{d\delta}
\end{bmatrix}\Bigg|_{\delta=0}=\begin{bmatrix}\nabla^2_{yy} g(x,\ystar) & \nabla_y h(x,\ystar)^{\top}\\
\nabla_y h(x,\ystar) & 0
\end{bmatrix}^{-1}\begin{bmatrix}-\nabla_y f(x,\ystar)\\
0
\end{bmatrix}. \numberthis\label{eq:LINEQ-dystardelta}
\] Combining \cref{eq:LINEQ-lim-findiff} and \cref{eq:LINEQ-dystardelta}  immediately yields the claim. 
% So we can express the left-hand side of the expression in the lemma statement by 
% \begin{align*}
% &\lim_{\delta\rightarrow0}\frac{\nabla_{x}[g(x,\ystardel(x))+\lamdeltar h(x,y^*)]-\nabla_{x}[g(x,y^{*}(x))+\lamstar h(x,y^{*})]}{\delta}\\
% &= \nabla^2_{xy} g(x,y^*) \frac{d\ydelstar}{d\delta} + \nabla_x h(x,y^*) \frac{d\lamdeltar}{d\delta}\\ 
% &=\begin{bmatrix}\nabla^2_{xy} g(x,\ystar) & \nabla_x h(x,\ystar)\end{bmatrix}\begin{bmatrix}\nabla^2_{yy} g(x,\ystar) & \nabla_y h(x,\ystar)^{\top}\\
% \nabla_y h(x,\ystar) & 0
% \end{bmatrix}^{-1}\begin{bmatrix}-\nabla_y f(x,\ystar)\\
% 0
% \end{bmatrix},
% \end{align*}
\end{proof}

% The core technical difficulty encountered in the construction of the hypergradient  for \cref{prob:lin-eq} is due to the term in \cref{eqn:second-order-method} involving $\frac{dy^*}{dx}$. 

% As discussed in \cref{sec:differentiable-optimization}, we can differentiate through the KKT conditions and apply implicit function theorem to derive the following linear equation to solve $\frac{dy^*}{dx}$.
% Specifically, fix a point $x$. Given $y^*= \arg\min_{y: h(x,y)=0} g(x,y)$, and $\lamstar$ is the dual optimal variable, define $\Leqc(x,y,\lam)=g(x,y)+\lam^\top h(x,y)$. Then, we have 
% \[
% \underbrace{\begin{bmatrix}\grad^2_{yy}\Leqc(x,\ystar,\lamstar) & \nabla_y h(x,y^{*})^{\top}\\
% \nabla_y h(x,y^{*}) & 0
% \end{bmatrix}}_{H ~\text{for linear equality constraints}}\begin{bmatrix}\frac{d\ystar}{dx}\\
% \frac{d\lamstar}{dx}
% \end{bmatrix}=\begin{bmatrix}-\nabla^2_{yx}g(x,y^{*})-\langle\lamstar, \nabla^2_{yx}h(x,y^{*})\rangle\\
% -\nabla_x h(x,\ystar)\end{bmatrix}.\numberthis\label{eq:def_matrix_H}\]

% Hence, we first make the following technical observation. 
% \jz{put one of the matrix inequality here to show how finite difference match the desired thing.}
% \begin{restatable}{lemma}{lemDystarDxLineq}\label{lem:dystarDxLinEq}
%     Fix a point $x$. Given $y^*= \arg\min_{y: h(x,y)=0} g(x,y)$ where $g$ is strongly convex in $y$ and $\lamstar$ is the dual optimal variable, define $\Leqc(x,y,\lam)=g(x,y)+\lam^\top h(x,y)$. Then, we have 
% \[\underbrace{\begin{bmatrix}\grad^2_{yy}\Leqc(x,\ystar,\lamstar) & \nabla_y h(x,y^{*})^{\top}\\
% \nabla_y h(x,y^{*}) & 0
% \end{bmatrix}}_{H ~\text{for linear equality constraints}}\begin{bmatrix}\frac{d\ystar}{dx}\\
% \frac{d\lamstar}{dx}
% \end{bmatrix}=\begin{bmatrix}-\nabla^2_{yx}g(x,y^{*})-\langle\lamstar, \nabla^2_{yx}h(x,y^{*})\rangle\\
% -\nabla_x h(x,\ystar)\end{bmatrix}.\numberthis\label{eq:def_matrix_H}\]
% \end{restatable}


% before showing how to approximate the hypergradient, we first analyze $\frac{dy^*}{dx}$ in the simpler setting of $y^*$ being the solution of an equality
% constrained problem (i.e., focusing on only the lower level of \cref{prob:lin-eq}). Specifically, consider the following nonlinear
% optimization problem given by 
% \[
% y^{*} := \begin{array}{ll}
% \arg\min_{y} & g(x,y)\\
% \mbox{subject to} & h(x,y)=0,
% \end{array}\numberthis\label{eq:ystar_def_leqc}
% \] where $g$ is assumed strongly convex. 
% Define $\Leqc(x,y,\lam):=g(x,y)+\lam h(x,y).$ \pswt{dimensions of $\lam$ and $h$}  

% \begin{equation}
% \underbrace{\begin{bmatrix}\grad^2_{yy}\Leqc(x,\ystar,\lamstar) & h_{y}(x,y^{*})^{\top}\\
% h_{y}(x,y^{*}) & 0
% \end{bmatrix}}_{H}\begin{bmatrix}\frac{d\ystar}{dx}\\
% \frac{d\lamstar}{dx}
% \end{bmatrix}=\begin{bmatrix}-g_{yx}(x,y^{*})-\lamstar h_{yx}(x,y^{*})\\
% -h_{x}(x,\ystar)
% \end{bmatrix}.\label{eq:def_matrix_H}
% \end{equation}
% If the matrix $H$ as in \cref{eq:def_matrix_H} is invertible, we may express the above equation as \[
% \begin{bmatrix}\frac{d\ystar}{dx}\\
% \frac{d\lamstar}{dx}
% \end{bmatrix}=H^{-1}\begin{bmatrix}-g_{yx}(x,y^{*})-\lamstar h_{yx}(x,y^{*})\\
% -h_{x}(x,\ystar)
% \end{bmatrix}.
% \]
% When $H$ is invertible, it affords us a formulation of $\frac{dy^*}{dx}$ as th

\begin{restatable}{lemma}{lemYdelstarLamdelstarSmooth}\label{lem:smoothness_of_ydelstar_lamdelstar}
The solution $y^*$ (as defined in \cref{{prob:lin-eq}}) is $O(C_H \cdot (\gssmooth + \|A\|))$-Lipschitz continuous and $O(C_H^3\cdot\gtsmooth\cdot(\gssmooth+\|A\|)^2)$-smooth as a function
of $x$. Thus the hyper-objective $F$ is gradient-Lipschitz  with a  smoothness constant of $C_F:=O\{ (L_f +C_f+C_g)C_H^3 S_g (L_g +\|A\|)^2\}.$ %\pswt{propagate from appendix}
\end{restatable}
\begin{proof}[Proof sketch; see \cref{{sec:appendix_linear_equality}}]
 The Lipschitz bound follows by combining \cref{{eq:def_matrix_H}} with the smoothness of $g$ and bound $C_H$ on the matrix inverse therein. Differentiating \cref{{eq:def_matrix_H}} by $x$ yields a linear system with the same matrix;  we repeat this approach to get the  smoothness bound. 
\end{proof}



%


%%%%%%%%%%%%
% \subsection{Inexact gradient oracle}
% We approximate the component $\partial_{y}f(x,y^{*}(x))\frac{\partial y^{*}(x)}{\partial x}$ of the hypergradient by \[\frac{\partial_{x}[g(x,\ystardel(x))+\lamdeltar h(x,\ystar)]-\partial_{x}[g(x,y^{*}(x))+\lamstar h(x,y^{*})]}{\delta}, \numberthis\label{eq:part-hypergrad-approx-lin-eq}\] where $\ydelstar$ and $\lamdeltar$ are, respectively, the primal and dual optimal values of the perturbed lower-level problem described in \cref{eq:lower_perturb}. 
% The strong convexity of $g$ and a sufficiently small $\delta$  ensure closeness of $\ydelstar$ to $y^*$ (as shown in \cref{lem:y-delstar-Lip}), which in turn helps obtain the desired approximation to the hypergradient (\cref{{lem:lineq-in-limit-finitediff-equals-gradf}} and \cref{lem:lineq-finitediff-equals-gradf}). 




% \begin{lemma}
% The matrix $H$ defined in \ref{eq:def_matrix_H} is invertible if
% the Hessian $\grad_{yy}^{2}\L(x,\ystar,\lamstar):=g_{yy}+\lamstar h_{yy}$
% satisfies $\nabla_{yy}^{2}\mathcal{L}(x,\ystar,\lamstar)\succ0$ over
% the tangent plane $T:=\{y:h_{y}(x,y^{*})y=0\}$ and $h_{y}$has full
% rank, i.e., $\ystar$ is a non-degenerate local optimal solution.
% \label{lem:non-singular-req}
% \end{lemma}

% \begin{proof}
% Let $u=[y,\lam].$ We show $Hu=0\Rightarrow u=0$. If $h_{y}(x,\ystar)y\neq0,$we
% have $Hu\neq0$. Otherwise if $h_{y}(x,\ystar)y=0$and $y\neq0$,
% the quadratic form reduces to 

% \[
% u^{\top}Hu=y^{\top}\grad_{yy}\L(x,\ystar,\lamstar)y>0.
% \]
% If $y=0$, $h_{y}$having full rank implies $\lam=0$.
% \end{proof}


% To turn \cref{{lem:lineq-in-limit-finitediff-equals-gradf}} into the desired gradient approximation result (\cref{lem:lineq-finitediff-equals-gradf}), we need \cref{lem:smoothness_of_ydelstar_lamdelstar} bounding smoothness of $\ydelstar$ and $\lamdeltar$. 

% We are now ready to show our main gradient approximation result for this section. 







==> src/linearEqualityFD.tex <==
\section{Lower level problem with linear equality constraint}\label{sec:equality-bilevel}
We consider bilevel programming with a linear equality constraint in the lower-level problem: 
\begin{align*}\numberthis\label[prob]{prob:lin-eq}
     & \mbox{minimize}_{x\in \mathcal{X}} ~ F(x) \coloneqq f(x, \ystar(x)) \text{ subject to } ~\ystar(x)\in \arg\min\nolimits_{y: h(x, y) = 0} g(x, y), 
\end{align*}
% \[
% \begin{array}{ll}
%      \mbox{minimize}_{x\in \mathcal{X}} & F(x):= f(x, \ystar(x))  \\
%      \mbox{subject to } & \ystar(x)\in \arg\min_{y: h(x, y) = 0} g(x, y), 
% \end{array} \numberthis\label[prob]{prob:lin-eq}
% \] 
where $f$, $g$, and $h$ satisfy the 
the regularity properties as described in  \cref{assumption:linEq_smoothness}. 

% \begin{assumption}\label{assumption:linEq_smoothness} 
% We study \cref{prob:lin-eq} under the following assumptions. 
% \begin{assumpenum}
% \compresslist{
% \item\label[assum]{item:assumption_lineq_first} Upper-level: The objective $f$  is $C_f$-smooth in $x,y$ jointly, i.e., $\norm{\nabla f(x_1,y_1) - \nabla f(x_2,y_2)} \! \leq C_f \norm{(x_1,y_1) - (x_2, y_2)}$ and $L_f$-Lipschitz in $y$. The constraint $\mathcal{X}$ is a convex compact set. 
%     \item Lower-level: The objective $g$ is second-order smooth with parameter $C_g$ and $\mu_g$-strongly convex in $y$. The constraint $h(x,y)=Ax-By-b$ has  $B$ being full row rank. \jz{Maybe we could justify the full rankness by complete recourse. That is, for any given $x$, there exists some $y$ to make the LL program feasible. I am wondering if we need that assumption for the inequality case? }
% }
% \end{assumpenum}
% \end{assumption}

Our main insight is that the hyper-gradient  $\grad_{x}F(x):=\grad_{x}f(x,y^{*}(x))+\frac{d y^*(x)}{dx}\grad_{y}f(x,y^{*}(x))$ is Lipschitz-continuous and  admits an easily computable --- yet highly accurate --- finite-difference approximation. Running gradient descent  for smooth non-convex optimization with this finite difference gradient proxy would then lead us to an approximate-stationary point. 

\iffalse
Specifically, fixing an $x\in \mathcal{X}$, our proposed finite-difference gradient proxy is motivated by the chain rule from calculus
$$\lim_{\delta\rightarrow0} \frac{y^*[x+\delta \nabla_y f(x,y^*(x))]-y^*(x)}{\delta}=\frac{d y^*(x)}{dx}\nabla_{y}f(x,y^{*}(x)).$$

Our proposed finite-difference proxy to it is given by 
 \[\mathcal{G}_{y^*}(x;\delta):={\frac{y^*[x+\delta \nabla_y f(x,y^*(x))]-y^*(x)}{\delta} \numberthis\label{eq:part-hypergrad-approx-lin-eq}.}\]
We will show that $\mathcal{G}_{y^*}(x;\delta)$ approximates $\frac{d y^*(x)}{dx}\nabla_{y}f(x,y^{*}(x))$ up to an error of $O(\delta)$. Notice  \cref{{eq:part-hypergrad-approx-lin-eq}} avoids differentiating through the implicit function $y^*(x)$. Instead, all we need to evaluate it are the values of $(y^*(x),y^*(x+\delta \nabla_y f(x,y^*(x))))$. Since these are  solutions to a smooth strongly convex linearly constrained  problem, accurate approximates to them could be readily obtained. 
 % for a given $x$


\begin{algorithm}[h]
\begin{algorithmic}[1]\caption{Inexact Gradient Oracle for Linear Equality Constraint}\label{alg:LE-inexact-gradient-oracle}
\State \textbf{Input:} 
Current $x$, accuracy $\epsilon$, perturbation $\delta = \epsilon^2$.
\jz{maybe we should state the accuracy required for solving these subproblems. We can only get some $\hat{y}^*(x)$ to approximate $y^*(x)$, also $\nabla_y f(x,y^*(x))$  would be evaluated at such a  $\nabla_y f(x,\hat{y}^*(x))$}
\State Compute $y^*$ (as in \cref{prob:lin-eq}) and $\lamstar$ (as in \cref{eqs:kkt-lin-eq}) 
\State Compute $\ystardel$ (as in \cref{eq:lower_perturb}) and $\lamdeltar$ (as in \cref{eqs:lineq-kkt-perturbed}) 
\State Compute $v$ as in \cref{eq:part-hypergrad-approx-lin-eq} \Comment{Approximates $\partial_{y}f(x,y^{*}(x))\frac{\partial y^{*}(x)}{\partial x}$}
\State Compute $\hat{\mathcal{G}}_{y^*}(x;\delta):=\frac{\hat{y}^*[x+\delta \nabla_y f(x,\hat{y}^*(x))]-\hat{y}^*(x)}{\delta}$
% \pswt{cref a standalone expression}
\State \textbf{Output:} $\widetilde{\nabla} F = v + \partial_x f(x, y^*(x))$
\end{algorithmic}
\end{algorithm}


\fi 

Specifically, fixing an $x\in \mathcal{X}$, our proposed finite-difference gradient proxy is given by the left-hand side of the following equation, approximating the implicit gradient term up to a $O(\delta)$-additive error:
 \[{\frac{\nabla_{x}[g(x,\ystardel)+\lamdeltar h(x,\ystar)]-\nabla_{x}[g(x,y^{*}(x))+\lamstar h(x,y^{*})]}{\delta}= \frac{d y^*(x)}{dx}\grad_{y}f(x,y^{*}(x)+O(\delta) \numberthis\label{eq:part-hypergrad-approx-lin-eq},}\]
where, for a fixed $x$, $(\ydelstar,\lamdeltar)$ are the primal and dual solutions to the
 perturbed lower level problem
 % for a given $x$
\begin{align}\label{eq:lower_perturb}
    & \ydelstar \coloneqq \arg\min\nolimits_{y: h(x,y) = 0} ~g(x,y)+\delta f(x,y).
\end{align}

\begin{algorithm}[h]
\begin{algorithmic}[1]\caption{Inexact Gradient Oracle for Linear Equality Constraint}\label{alg:LE-inexact-gradient-oracle}
\State \textbf{Input:}
Current $x$, accuracy $\epsilon$, perturbation $\delta = \epsilon^2$.
\State Compute $y^*$ (as in \cref{prob:lin-eq}) and $\lamstar$ (as in \cref{eqs:kkt-lin-eq}) 
\State Compute $\ystardel$ (as in \cref{eq:lower_perturb}) and $\lamdeltar$ (as in \cref{eqs:lineq-kkt-perturbed}) 
\State Compute $v$ as in \cref{eq:part-hypergrad-approx-lin-eq} \Comment{Approximates $\partial_{y}f(x,y^{*}(x))\frac{\partial y^{*}(x)}{\partial x}$}
% \pswt{cref a standalone expression}
\State \textbf{Output:} $\widetilde{\nabla} F = v + \partial_x f(x, y^*(x))$
\end{algorithmic}
\end{algorithm}

Notice that the finite-difference term in \cref{{eq:part-hypergrad-approx-lin-eq}} avoids differentiating through the implicit function $y^*(x)$. Instead, all we need to evaluate it are the values of $(y^*,\lambda^*,\ydelstar,\lamdeltar)$ (followed by gradient queries to $g$ and $h$). Since these are  solutions to a smooth strongly convex linearly constrained  problem, accurate approximates to $(y^*,\lambda^*)$ could be readily obtained. Similarly, since the approximation error in \cref{eq:part-hypergrad-approx-lin-eq}  is proportion to $\delta$, we can choose a  small $\delta$  such that the perturbed objective $ g+\delta f$ in \cref{eq:lower_perturb} is dominated by the strongly convex and smooth $g$, whereby accurate approximates to $(y_\delta^*,\lambda_\delta^*)$ could also be readily obtained. Putting it all together, the proposed finite-difference hyper-gradient proxy in \cref{eq:part-hypergrad-approx-lin-eq}  can be  efficiently computed.

\begin{restatable}{theorem}{linEqFullCost}\label{thm:lineq-cost}
    Consider  \cref{prob:lin-eq} under \cref{assumption:linEq_smoothness}, and define $\kappa=C_g/\mu_g$ to be the condition number of $g$. Then there exists an algorithm so that after $T=O(\sqrt{\kappa}\epsilon^{-2})$ gradient oracle calls to $f$, $g$, and $h$, we have $\min_{i\in [T]} \|\nabla F(x_i)\|\leq \epsilon$. 
\end{restatable}


By an application of the implicit function theorem to the KKT system of \cref{eq:lower_perturb}, we show in \cref{{lem:lineq-finitediff-equals-gradf}} that the variable $\ystardel$  and its corresponding optimal dual variable $\lamdeltar$ can be used to construct an approximation to  $\frac{d}{dx}y^{*}(x)\grad_{y}f(x,y^{*}(x))$, as displayed in \cref{alg:LE-inexact-gradient-oracle}. 
% The required regularity properties of $\ystardel$ and $\lamdeltar$ for this gradient approximation to hold are essentially satisfied when $f$, $g$, and $h$ satisfy \cref{assumption:linEq_smoothness}.  
The regularity properties of $f$, $g$, and $h$  from \cref{assumption:linEq_smoothness} also imply smoothness of $F$, as we formally show in \cref{{{thm:lineq-cost}}}; therefore, our inexact gradient oracle of $F$ (via \cref{alg:LE-inexact-gradient-oracle}) allows us to run  $O(\epsilon^{-2})$ iterations of projected gradient descent with an inexact gradient oracle to obtain an $\epsilon$-stationary point for \cref{prob:lin-eq}. Since each iteration of \cref{alg:LE-inexact-gradient-oracle} solves a strongly convex optimization problem over a linear subspace, it costs $O(\sqrt{\kappa})$~\cite{salim2022optimal}, where $\kappa$ is the condition number of $f$, thus giving us a total cost of $O(\sqrt{\kappa}\epsilon^{-2})$ in attaining $\epsilon$-stationarity of \cref{prob:lin-eq}, as formalized in \cref{thm:lineq-cost}.


%%%%%%%%%%%%

\subsection{Main idea}\label{sec:warmup-lin-eq}

\jz{sketch Lemma 3.3 in a high level, why does these two quantities match in the limit? also explain the smoothness}
The core technical difficulty encountered in the construction of the hypergradient  for \cref{prob:lin-eq} is due to the term in \cref{eqn:second-order-method} involving $\frac{dy^*}{dx}$. 

As discussed in \cref{sec:differentiable-optimization}, we can differentiate through the KKT conditions and apply implicit function theorem to derive the following linear equation to solve $\frac{dy^*}{dx}$.
Specifically, fix a point $x$. Given $y^*= \arg\min_{y: h(x,y)=0} g(x,y)$, and $\lamstar$ is the dual optimal variable, define $\Leqc(x,y,\lam)=g(x,y)+\lam^\top h(x,y)$. Then, we have 
\[
\underbrace{\begin{bmatrix}\grad^2_{yy}\Leqc(x,\ystar,\lamstar) & \nabla_y h(x,y^{*})^{\top}\\
\nabla_y h(x,y^{*}) & 0
\end{bmatrix}}_{H ~\text{for linear equality constraints}}\begin{bmatrix}\frac{d\ystar}{dx}\\
\frac{d\lamstar}{dx}
\end{bmatrix}=\begin{bmatrix}-\nabla^2_{yx}g(x,y^{*})-\langle\lamstar, \nabla^2_{yx}h(x,y^{*})\rangle\\
-\nabla_x h(x,\ystar)\end{bmatrix}.\numberthis\label{eq:def_matrix_H}\]

% Hence, we first make the following technical observation. 
% \jz{put one of the matrix inequality here to show how finite difference match the desired thing.}
% \begin{restatable}{lemma}{lemDystarDxLineq}\label{lem:dystarDxLinEq}
%     Fix a point $x$. Given $y^*= \arg\min_{y: h(x,y)=0} g(x,y)$ where $g$ is strongly convex in $y$ and $\lamstar$ is the dual optimal variable, define $\Leqc(x,y,\lam)=g(x,y)+\lam^\top h(x,y)$. Then, we have 
% \[\underbrace{\begin{bmatrix}\grad^2_{yy}\Leqc(x,\ystar,\lamstar) & \nabla_y h(x,y^{*})^{\top}\\
% \nabla_y h(x,y^{*}) & 0
% \end{bmatrix}}_{H ~\text{for linear equality constraints}}\begin{bmatrix}\frac{d\ystar}{dx}\\
% \frac{d\lamstar}{dx}
% \end{bmatrix}=\begin{bmatrix}-\nabla^2_{yx}g(x,y^{*})-\langle\lamstar, \nabla^2_{yx}h(x,y^{*})\rangle\\
% -\nabla_x h(x,\ystar)\end{bmatrix}.\numberthis\label{eq:def_matrix_H}\]
% \end{restatable}


% before showing how to approximate the hypergradient, we first analyze $\frac{dy^*}{dx}$ in the simpler setting of $y^*$ being the solution of an equality
% constrained problem (i.e., focusing on only the lower level of \cref{prob:lin-eq}). Specifically, consider the following nonlinear
% optimization problem given by 
% \[
% y^{*} := \begin{array}{ll}
% \arg\min_{y} & g(x,y)\\
% \mbox{subject to} & h(x,y)=0,
% \end{array}\numberthis\label{eq:ystar_def_leqc}
% \] where $g$ is assumed strongly convex. 
% Define $\Leqc(x,y,\lam):=g(x,y)+\lam h(x,y).$ \pswt{dimensions of $\lam$ and $h$}  

% \begin{equation}
% \underbrace{\begin{bmatrix}\grad^2_{yy}\Leqc(x,\ystar,\lamstar) & h_{y}(x,y^{*})^{\top}\\
% h_{y}(x,y^{*}) & 0
% \end{bmatrix}}_{H}\begin{bmatrix}\frac{d\ystar}{dx}\\
% \frac{d\lamstar}{dx}
% \end{bmatrix}=\begin{bmatrix}-g_{yx}(x,y^{*})-\lamstar h_{yx}(x,y^{*})\\
% -h_{x}(x,\ystar)
% \end{bmatrix}.\label{eq:def_matrix_H}
% \end{equation}
% If the matrix $H$ as in \cref{eq:def_matrix_H} is invertible, we may express the above equation as \[
% \begin{bmatrix}\frac{d\ystar}{dx}\\
% \frac{d\lamstar}{dx}
% \end{bmatrix}=H^{-1}\begin{bmatrix}-g_{yx}(x,y^{*})-\lamstar h_{yx}(x,y^{*})\\
% -h_{x}(x,\ystar)
% \end{bmatrix}.
% \]
% When $H$ is invertible, it affords us a formulation of $\frac{dy^*}{dx}$ as th
In \cref{lem:non-singular-req}, we provide a condition
for when the matrix $H$ from  \cref{eq:def_matrix_H} is invertible; essentially, it says that
$H$ is invertible as long as $g$ is strongly convex. 
\begin{restatable}{lemma}{lemLineqHinvertibility}\label{lem:non-singular-req} 
Consider the setup in \cref{{lem:dystarDxLinEq}}. The matrix $H$ defined in \cref{eq:def_matrix_H}  is invertible if
the Hessian $\grad_{yy}^{2}\Leqc(x,\ystar,\lamstar):=\nabla^2_{yy} g(x, y^*) +\lamstar \nabla^2_{yy} h(x, y^*)$
satisfies $\nabla_{yy}^{2}\Leqc(x,\ystar,\lamstar)\succ0$ over
the tangent plane $T:=\{y:\nabla_y h(x,y^{*})y=0\}$ and $\nabla_y h$ has full
rank.
% , i.e., $\ystar$ is a non-degenerate local optimal solution. 
% As such, \pswt{move this}
% \label{lem:non-singular-req}
\end{restatable}

%
\begin{restatable}{corollary}{corNonSingularH}\label{cor:nonsingularH}
For \cref{prob:lin-eq} under \cref{assumption:linEq_smoothness}, 
 the matrix $H$  (as defined in \cref{eq:def_matrix_H}) is non-singular. Further, there exists a finite $C_H$ such that $\|H^{-1}\|\leq C_H$. 
% and $\|\frac{d\ystar}{dx}\|\leq C_H C_g$. 
\end{restatable}

%%%%%%%%%%%%
% \subsection{Inexact gradient oracle}
% We approximate the component $\partial_{y}f(x,y^{*}(x))\frac{\partial y^{*}(x)}{\partial x}$ of the hypergradient by \[\frac{\partial_{x}[g(x,\ystardel(x))+\lamdeltar h(x,\ystar)]-\partial_{x}[g(x,y^{*}(x))+\lamstar h(x,y^{*})]}{\delta}, \numberthis\label{eq:part-hypergrad-approx-lin-eq}\] where $\ydelstar$ and $\lamdeltar$ are, respectively, the primal and dual optimal values of the perturbed lower-level problem described in \cref{eq:lower_perturb}. 
% The strong convexity of $g$ and a sufficiently small $\delta$  ensure closeness of $\ydelstar$ to $y^*$ (as shown in \cref{lem:y-delstar-Lip}), which in turn helps obtain the desired approximation to the hypergradient (\cref{{lem:lineq-in-limit-finitediff-equals-gradf}} and \cref{lem:lineq-finitediff-equals-gradf}). 




% \begin{lemma}
% The matrix $H$ defined in \ref{eq:def_matrix_H} is invertible if
% the Hessian $\grad_{yy}^{2}\L(x,\ystar,\lamstar):=g_{yy}+\lamstar h_{yy}$
% satisfies $\nabla_{yy}^{2}\mathcal{L}(x,\ystar,\lamstar)\succ0$ over
% the tangent plane $T:=\{y:h_{y}(x,y^{*})y=0\}$ and $h_{y}$has full
% rank, i.e., $\ystar$ is a non-degenerate local optimal solution.
% \label{lem:non-singular-req}
% \end{lemma}

% \begin{proof}
% Let $u=[y,\lam].$ We show $Hu=0\Rightarrow u=0$. If $h_{y}(x,\ystar)y\neq0,$we
% have $Hu\neq0$. Otherwise if $h_{y}(x,\ystar)y=0$and $y\neq0$,
% the quadratic form reduces to 

% \[
% u^{\top}Hu=y^{\top}\grad_{yy}\L(x,\ystar,\lamstar)y>0.
% \]
% If $y=0$, $h_{y}$having full rank implies $\lam=0$.
% \end{proof}


% To turn \cref{{lem:lineq-in-limit-finitediff-equals-gradf}} into the desired gradient approximation result (\cref{lem:lineq-finitediff-equals-gradf}), we need \cref{lem:smoothness_of_ydelstar_lamdelstar} bounding smoothness of $\ydelstar$ and $\lamdeltar$. 

We are now ready to show our main gradient approximation result for this section. 
\begin{restatable}{lemma}{lemLineqFiniteDiffEqualsGradF}\label{lem:lineq-finitediff-equals-gradf} Consider  \cref{prob:lin-eq} under \cref{assumption:linEq_smoothness}. 
% Assume $h(x,y):=Ay-Bx-b$ with $A$ having full rank. <-included in \cref{prob:lin-eq} maybe put $A$ being full rank in an assumption env for clarity?
Then the
following relation is valid.
% \pswt{also requires third order smoothness of $g$}
\[
\left\|\frac{\nabla_{x}[g(x,\ystardel(x))+\lamdeltar h(x,\ystar)]-\nabla_{x}[g(x,y^{*}(x))+\lamstar h(x,y^{*})]}{\delta}-\nabla_{y}f(x,y^{*}(x))\frac{d y^{*}(x)}{d x}\right\|\leq O(\delta).
\]
\end{restatable}







==> src/old.tex <==
\section{Some old attempt}
\subsection{Removing dependency on the derivative of Lagrangian multiplier}
\cref{eqn:derivative-bound1} offers a way to estimate the difference in derivatives of the objectives $\phi_{\gamma(x)}(x) = \phi(x)$.
However, the challenge here is the dependency on $\gamma(x)$ and its derivative $\nabla_x \gamma(x)$. 
In order to compute the derivative to the dual solution $\gamma(x)$, it still requires to compute the second-order term, which still does not solve the issue.

To resolve this issue, we define another Lagrangian:
\begin{align}\label{eqn:constrained-lagrangian}
    \mathcal{L}_\lambda(x,y) = f(x,y) + \lambda (g(x,y) - g^*(x)) ~ \text{where}~g^*(x) = \min_{y: h(x,y) \leq 0} g(x,y)
\end{align}

We compute the derivative of $\mathcal{L}_\lambda(x,y)$ by:
\begin{align}
    \nabla_x \mathcal{L}_\lambda(x,y) = \nabla_x f(x,y) + \lambda \left(\nabla_x g(x,y) - \nabla_x g(x,y^*_{\gamma(x)}) - {\color{orange} \nabla_y g(x, y^*_{\gamma(x)}) \cdot \frac{d y^*_{\gamma(x)}}{d x}} \right)
\end{align}

\begin{align}
    \nabla_y g(x,y^*_{\gamma(x)}) + \gamma(x) \nabla_y h(x,y^*_{\gamma(x)}) = 0
\end{align}

\begin{align}
    \gradx \mathcal{L}_{\lambda,\gamma}(x,y) = \gradx f(x,y) + \lambda(\gradx g(x,y) + {\color{blue}\gamma\gradx h(x,y)} + {\color{red}h(x,y)\gradx\gamma}-\gradx g(x,\ysg) - {\color{blue}\gamma\gradx h(x,\ysg)} - {\color{red}h(x,\ysg)\gradx\gamma})
\end{align}

Comparing this term to the other derivative:
\begin{align}
    \nabla_x \mathcal{L}_{\lambda,\gamma}(x, \yslg) - \nabla_x \mathcal{L}_\lambda(x,\yslg)
\end{align}

\begin{theorem}
    \begin{align}
    \norm{\frac{d \phi_{\gamma(x)}(x)}{d x} - \nabla_x \mathcal{L}_{\lambda}(x, y^*_{\lambda}(x)) + M \cdot\grady\Llg(x,y)} = O(\frac{1}{\lambda}) + \left(\nabla_x h(x,y) - \nabla_x h(x,y^*_{\lambda})\right) \gamma(x)
    \end{align}
    where $y^*_{\lambda}(x) = \arg\min_y \mathcal{L}_{\lambda}(x, y)$.
\end{theorem}
\begin{proof}
    TODO
\end{proof}

Now the expression does not depend on the derivative of the dual solution $\gamma(x)$. It only depends on the value of the dual solution. Under the assumption that the dual solution is bounded, and the constraint function $h$ is smooth, we can bound:
\begin{theorem}
    \begin{align}
    \norm{\frac{d \phi(x)}{d x} - \nabla_x \mathcal{L}_{\lambda}(x, y^*_{\lambda}(x))} = O(\frac{1}{\lambda}) + \left(\nabla_x h(x,y) - \nabla_x h(x,y^*_{\lambda})\right) \gamma(x)
    \end{align}
    where $y^*_{\lambda}(x) = \arg\min_y \mathcal{L}_{\lambda}(x, y)$.
\end{theorem}
\begin{proof}
    TODO
\end{proof}
which is due to $\phi_{\gamma(x)}(x) = \phi(x)$ and $\norm{\nabla_x h(x,y) - \nabla_x h(x,y^*_{\lambda}} \leq c \norm{y - y^*_{\lambda}}$.

What this tells us is that we just need to compute the derivative of the Lagrangian in \cref{eqn:constrained-lagrangian} to get an approximate to the derivative of the constrained bilevel optimization problem in Equation~\ref{eqn:constrained-bilevel-optimization}.

% further analyze the derivative $\nabla_x \mathcal{L}_{\lambda, \gamma}(x, y^*_{\lambda,\gamma}(x))$:

% \begin{align}
%     \frac{d}{dx}\mathcal{L}_{\lambda, \gamma}(x, y^*_{\lambda,\gamma}(x)) = \nabla_x \mathcal{L}_{\lambda, \gamma}(x, y^*_{\lambda,\gamma}(x))
% \end{align}

\section{Feb 26th discussion}

\begin{align}
    g_{a,b}^*(x,y,z) = \min_{\theta} \max_{\gamma} g(x,\theta) + \gamma h(x,\theta) + \frac{1}{a} \norm{\theta - y}^2 - \frac{1}{b} \norm{\gamma - z}^2
\end{align}

\begin{align}
    \mathcal{L}_\lambda(x,y,z) = f(x,y) + \lambda (g(x,y) + z h(x,y) - g_{a,b}^*(x,y,z))
\end{align}

First, given $x_1$, $x_2$, $\lambda_1, \lambda_2$, we want to show $y^*_{\lambda_1}(x_1)$ and $y^*_{\lambda_2}(x_2)$, $\gamma_{\lambda_1}(x_1)$ and $\gamma_{\lambda_2}(x_2)$ are close?


\section{Old materials (to be organized)}


The main challenge in this formulation is the presence of constraints $h(x,y)$. If we do not have constrains in the lower optimization problem, the derivative $\frac{dy^*}{dx}$ can be simply written as $(\nabla^2_{yy} g)^{-1} \nabla^2_{xy} g$. There are also nice properties like $\norm{\nabla_x \phi(x) - \nabla_x \mathcal{L}_\lambda(x,\bar{y}^*(x))} = O(\frac{1}{\lambda})$~\cite{chen2023near,kwon2023fully} which we will talk about it later.


One potential solution to resolve the constraints in the inner optimization problem is to define a Lagrangian problem with a multiplier $\gamma \geq 0$ to convert constraints $h(x,y)$ to the objective in the lower optimization problem, which can be found below.
% \begin{align}\label{eqn:unconstrained-bilevel-optimization}
%     \min_{x} & \quad \bar{\phi}_\gamma(x) \coloneqq f(x, \bar{y}^*_\gamma(x)) \\
%     \text{where} & \quad \bar{y}^*_\gamma(x) = \arg\min_{y} g(x, y) + \gamma h(x,y) \nonumber
% \end{align}

The derivative of \cref{eqn:unconstrained-bilevel-optimization} can be easily computed by:
\begin{align}
    \frac{d \bar{\phi}_\gamma(x)}{d x} & = \frac{\partial f}{\partial x} + \frac{\partial f}{\partial y} \frac{d \bar{y}_\gamma}{d x} \nonumber \\
    & = \frac{\partial f}{\partial x} + \frac{\partial f}{\partial y} (\nabla^2_{yy} g + \gamma \nabla_{yy}^2 h)^{-1} (\nabla^2_{xy} g + \gamma \nabla_{xy}^2 h)
\end{align}

We can also define a similar reformulation as shown in~\cite{chen2023near,kwon2023fully}:
% \begin{align}
%     \min_{x \in \mathcal{X}} \bar{\phi}_\gamma(x) \coloneqq & \min_y \objective(x, y) \\
%     \text{s.t.} & \quad \bar{g}_\gamma(x,y) \leq \bar{g}^*_\gamma(x) % y = \arg\min_{y} \Bar{g}_\gamma(x,y)
% \end{align}

Since this is a unconstrained belevel optimization problem with strong convexity, we can use the result from~\cite{chen2023near,kwon2023fully} to show:
% \begin{theorem}[Known result]
% \begin{align}
%     \norm{\frac{d \bar{\phi}_\gamma(x)}{d x} - \nabla_x \mathcal{L}_{\lambda,\gamma}(x, \bar{y}^*_{\lambda,\gamma}(x))} = O(\frac{1}{\lambda})
% \end{align}
where $\bar{y}^*_{\lambda,\gamma}(x) \coloneqq \arg\min_{y} \mathcal{L}_{\lambda,\gamma}(x,y)$. \pswt{I think this is true only for the Lagrangian defined for $\bar{\phi}_\gamma$ since following \cite{kwon2023fully}'s proof requires us to use $\nabla_y \mathcal{L}_{\lambda, \gamma}(x,y) = \nabla_y f(x,y) + \lambda\cdot(\nabla_y g(x, y) + \gamma \nabla_y h(x,y))$} 

% \end{theorem}
Therefore, we just need to use the gradient computed from solving the Lagrangian problem without doing differentiable optimization.

Compared to \cref{eqn:constrained-bilevel-optimization}, \cref{eqn:unconstrained-bilevel-optimization} has no constraints in the inner optimization problem due to the use of Lagrangian. But it may also have a different solution $\bar{y}_\gamma$ that is different from the original one $y^*$.

\begin{theorem}[Our final goal]
    \begin{align}
    \norm{\frac{d \phi}{d x} - \nabla_x \mathcal{L}_{\lambda,\gamma}(x, \bar{y}^*_{\lambda,\gamma}(x))} = \text{poly}(\frac{1}{\lambda}, \frac{1}{\gamma})
\end{align}
\end{theorem}
If this is true, then we can select $\lambda$ and $\gamma$ to control the error or biasness of the gradient estimated from the Lagrangian. Computing the gradient from the Lagrangian also only involves first-order gradient computation:
\begin{align}
    \nabla_x \mathcal{L}_{\lambda,\gamma}(x, \bar{y}^*_{\lambda,\gamma}(x)) = \frac{\partial \mathcal{L}_{\lambda,\gamma}}{\partial x} + \frac{\partial \mathcal{L}_{\lambda,\gamma}}{\partial y} \frac{d \bar{y}^*_{\lambda,\gamma}(x)}{d x} = \frac{\partial \mathcal{L}_{\lambda,\gamma}}{\partial x}
\end{align}
where $\frac{\partial \mathcal{L}_{\lambda,\gamma}}{\partial y} = 0$ at the optimal solution $y = \bar{y}^*_{\lambda,\gamma}(x)$ since it is an unconstrained problem.



\begin{definition}[Some notations]
\begin{align}
    \Bar{g}_\gamma(x,y) = g(x,y) + \gamma h(x,y), \quad \mathcal{L}_{\lambda,\gamma}(x,y) = f(x,y) + \lambda \Bar{g}_\gamma(x,y)
\end{align}
\begin{align}
    g^*(x) = \min_{y: h(x,y) \leq 0} g(x,y), \quad \Bar{g}^*_\gamma(x) = \min_{y} \Bar{g}_\gamma(x,y), \quad \Bar{g}^*_{\lambda,\gamma}(x) = \min_{y} \mathcal{L}_{\lambda,\gamma}(x,y)
\end{align}
\begin{align}
    y^*(x) = \arg\min_{y: h(x,y) \leq 0} g(x,y), \quad \Bar{y}^*_\gamma(x) = \arg\min_{y} \Bar{g}_\gamma(x,y), \quad \Bar{y}^*_{\lambda,\gamma}(x) = \arg\min_{y} \mathcal{L}_{\lambda,\gamma}(x,y)
\end{align}
\end{definition}


{\color{red}
\begin{itemize}
    \item Can we bound the difference between $y^*(x)$, $\bar{y}^*_\gamma(x)$, and $\bar{y}^*_{\lambda,\gamma}(x)$?
    \item This seems to be an essential step if we want to follow the proof in~\cite{chen2023near,kwon2023fully}.
\end{itemize}
}


\subsection{Another reformulation}

{\color{red}
\begin{align} 
    \min_{x \in \mathcal{X}} \phi(x) \coloneqq & \min_y \objective(x, y) \\
    \text{s.t.} & \quad g(x,y) \leq g^*(x), \quad h(x,y) \leq 0 \label{eqn:two_constraints}
\end{align}
\begin{itemize}
    \item This is in fact (to be checked) equivalent to the Lagrangian $\mathcal{L}_{\lambda,\gamma}(x,y) = f(x,y) + \lambda \Bar{g}_\gamma(x,y)$.
    \item Can we show that the derivative derived from \cref{eqn:double-lagrangian-reformulation} is also close to the derivative in \cref{eqn:full-derivative} and \cref{eqn:schur-compliment}?
\end{itemize}
\begin{align}\label{eqn:double-lagrangian-reformulation}
    \min_{x,y} f(x,y) + \lambda (g(x,y) - g^*(x)) + \gamma h(x,y)
\end{align}
}

==> src/problem-formulation.tex <==
\section{Preliminaries}\label{sec:preliminaries}
% We set our notation and review some useful facts from convex analysis before providing formal details of our problem. 
Throughout, we use $\langle \cdot{}, {}\cdot\rangle$ to denote inner products and $\|{}\cdot{}\|$ to denote the Euclidean norm, and unless transposed, all vectors are column vectors. For $f:\reals^{d_2}\to\reals^{d_1}$ its Jacobian with respect to $x\in \reals^{d_2}$ is 
% \pswt{this is dimensionally fine, but notationally horrible}
$\nabla_x f\in \reals^{d_1 \times d_2}$.  For $f:\reals^d\to\reals$, we overload notation and term $\nabla_x f$ its gradient (the transposed Jacobian), a column vector. \pswt{notation for  partial derivatives, higher order derivatives, etc.}

A function $f:\reals^n\to\reals^m$ is $L$-Lipschitz if for any $x,y$, we have $\|f(x) - f(y)\|\leq L \|x-y\|$.
A differentiable function $f:\reals^n\to\reals$ is convex if for any $x, y\in \reals^n$ we have $f(y)\geq f(x) + \nabla f(x)^\top (y-x)$; 
% A differentiable function $f:\reals^n\mapsto\reals$
it is 
 $\mu$-strongly convex
 if $f - \tfrac{\mu}{2}\|{}\cdot{}\|^2$ is convex;
% w.r.t. the $\ell_2$-norm
% if for any $x, y \in \reals^n$, we  have  $f(y) \geq f(x) + \nabla f(x)^\top (y-x) + \tfrac{\mu}{2}\|y-x\|^2$; 
it is  $\beta$-smooth
% w.r.t. the $\ell_2$-norm
if
$\nabla f$ is $\beta$-Lipschitz.
% $0.5\beta\|{}\cdot{}\|^2- f$ is convex. 
% \jz{maybe we can say something like $\norm{\grad f(y)-\grad f(x)}\leq \beta \norm{y-x} \ \forall y,x$. The stated one is equivalent, but less frequently used in the literature.}
% for any $x, y \in \reals^n$, we  have  $f(y) \leq f(x) + \nabla f(x)^\top (y-x) + \tfrac{\beta}{2}\|y-x\|^2$. 


\begin{definition}\label{def:GoldsteinDeltaEpsStationary}
 Consider a locally Lipschitz function $f:\reals^d\to\reals$, a point $x\in\reals^d$, and a parameter $\delta>0$. The {Goldstein subdifferential}~\cite{goldstein1977optimization} of $f$ at $x$ is the set
 $\partial_{\delta} f(x):=\mathrm{conv} (\cup_{y\in \mathbb{B}_{\delta}(x)}\partial f(y)),$ where  $\partial f(x)=\mathrm{conv}\left\{\lim_{n\to \infty} \nabla f(x_n): x_n\to x, ~x_n\in \mathrm{dom}(\nabla f)\right\}$ is the Clarke subdifferential~\cite{clarke1981generalized} of $f$ and $\mathbb B_\delta(x)$ denotes the Euclidean ball of radius $\delta$ around $x$.
 A point $x$ is called $(\delta, \epsilon)$-stationary if $\mathrm{dist}(0,\partial_{\delta}f(x))\leq \epsilon$, where $\mathrm{dist}(x,S):=\inf_{y\in S}\|x-y\|$.
 % for $x\in \reals^d$ and $S \subseteq \reals^d$ is $\inf_{y\in S}\|x-y\|$.

\end{definition}
%
Thus, for a Lipschitz function $f$, a point $x$ is $(\delta, \epsilon)$-stationary if within a $\delta$-ball around $x$, there exists a convex combination of  subgradients of $f$ with norm at most $\epsilon$. 
% Thus, the Goldstein subdifferential of $f$ at $x$ is the convex hull of all Clarke subgradients at points in a  $\delta$-ball around $x$. 
For a differentiable function $f$, we say that $x$ is $\epsilon$-stationary if $\|\nabla f(x)\|\leq \epsilon$. 

\subsection{Assumptions}\label{sec:differentiable-optimization}
We consider \cref{{prob:general-constraints}} with convex inequality constraints (\cref{sec:inequality-bilevel} and \cref{sec:nonsmooth}) under \cref{assumption:linEq_smoothness,item:assumption_safe_constraints}, and with linear equality constraints (\cref{sec:equality-bilevel}) under \cref{assumption:linEq_smoothness,assumption:eq}. 
We have $x\in \reals^{d_x}$ for the upper-level (UL) variable and $y\in \reals^{d_y}$ for the lower-level (LL) variable. We assume that $h:\reals^{d_x} \times \reals^{d_y}\to \reals^{d_h}$ is an element-wise constraint function with $d_h$ constraints. % \pswt{add dims of $h$} \kai{added. To check consistency.}. 
% We have the upper-level (UL) objective function $f:\reals^{d_x}\times\reals^{d_y}\to\reals$ of the UL variable $x\in\reals^{d_x}$ and  $y^*(x)\in\reals^{d_y}$, the minima of a possibly constrained lower-level (LL) objective $g:\reals^{d_x}\times\reals^{d_y}\to\reals$.
% \gk{dimension as above?}. 

\iffalse 
following bilevel optimization problem with constrained lower level problem:
\begin{align}
    \min\nolimits_{x} \quad & F(x):= f(x, y^\ast(x))  &
     \text{s.t.} \quad & y^\ast(x) \in \arg\min\nolimits_{ x,y \text{ feasible}} g(x,y) \label{prob:orig_bilevel}
\end{align}
We consider the case where the lower objective is strongly convex and smooth, and the constraints to be equality constraints ($h(x,y) = 0$) in Section~\ref{sec:equality-bilevel}, and inequalty constrains ($h(x,y) \leq 0$) in Section~\ref{sec:inequality-bilevel} and Section~\ref{sec:nonsmooth}, where $h$ is a vector value function in both cases.

The upper objective just needs to be smooth and Lipschitz in $y$. 

Our assumptions on the objective functions are summarized in Assumption~\ref{assumption:linEq_smoothness} and Assumption~\ref{assumption:smoothness} (additionally for inequality constraints).
\fi 

\begin{assumption}\label{assumption:linEq_smoothness} 
For \cref{prob:general-constraints}, we assume the following for both settings we study: 
% \gk{Having swapped the order of results, should we swap the order of assumptions (for clarity)?}\pswt{(5/13)Yes, Jimmy and I discussed again, and it looks like having equality going \emph{after} inequality makes most sense; so yes, we can present the assumptions in whatever order makes most sense for this!} \kai{I think my plan was Assumption 2.2 is for both ineq and eq, while Assumption 2.3 is for ineq only. Swapping the assumption order may not work in this way?}
\begin{assumpenum}
\compresslist{
\item\label[assum]{item:assumption_upper_level} Upper-level: The objective $f$ is $C_f$-smooth and $L_f$-Lipschitz continuous in $(x,y)$. 
%\jz{Lipschitz on $(x,y)$ implies Lipschitz on $x$ while fixing $y$.}%in $x$, $y$, and $x,y$ jointly
% , i.e., $\norm{\nabla f(x_1,y_1) - \nabla f(x_2,y_2)} \! \leq C_f \norm{(x_1,y_1) - (x_2, y_2)}$ %\pswt{removing this since we already just defined smoothness}
%and $L_f$-Lipschitz in $x$ and $y$. % The constraint $\mathcal{X}$ is a convex compact set. 
    \item \label[assum]{item:assumption_lower_level}Lower-level: The objective $g$ is $C_g$-smooth and the constraint $h$ is $C_h$-smooth in $(x,y)$. Fixing any $x\in\mathcal{X}$, $g(x,\cdot)$ is $\mu_g$-strongly convex and the constraint $h(x,\cdot)$ is convex in $y$.

    \item \label[assum]{item:assumption_tangen_space} LICQ: We assume the LICQ condition holds for the LL problem for every $x$ and $y$, that is,
    the derivative $\nabla_y h(x,y)$ has full row rank on active constraints. In the linear equality case, this corresponds to the constraint $h(x,y)=Ax-By-b$ having a full row rank $B$.
    
    %\item \label[assum]{item:assumption_tangen_space} Tangent space: the derivative $\nabla_y h(x,y)$ has full row rank on active constraints, which in the linear case it corresponds to the constraint $h(x,y)=Ax-By-b$ has  $B$ being full row rank.
    %\jz{Maybe we could justify the full rankness by complete recourse. That is, for any given $x$, there exists some $y$ to make the LL program feasible. I am wondering if we need that assumption for the inequality case? }
}
\end{assumpenum}
\end{assumption}


\begin{assumption}\label{item:assumption_safe_constraints} 
% \pswt{We seem to also use a bound on $\nabla^2_{xy}f$ in the proof of \cref{thm:diff_in_hypergrad_and_gradLagr}; is the constant for that included in the current assumption?}
For \cref{prob:ineq} (with convex inequality constraints), we additionally assume $y^*(x)$ is $L_y$-Lipschitz in $x$ and $\gamma(x)$ is  bounded: $\norm{\gamma(x)} \leq R$, where for a given $x$, we denote the LL primal and dual solution $y^*(x), \gamma(x) = \arg\max\nolimits_\theta \min\nolimits_{\beta \geq 0} g(x,y) + \beta^\top h(x,y)$. % \gk{undefined at this point.} 
    % We assume  . 
    %\jz{maybe we should point out that this implies some full recourse assumption, that is, for every $x$ there exists some $y$ to make the LL problem feasible.} 
% \begin{assumpenum} 
% \compresslist{
%     % \item Upper-level: The objective $f$ is $L_f$-Lipschitz in $y$ and $C_f$-smooth in $x,y$ jointly, i.e., $\norm{\nabla f(x_1,y_1) - \nabla f(x_2,y_2)} \! \leq \! C_f \! \norm{(x_1,y_1) - (x_2, y_2)} $. 
%     % \item Lower-level: The objective $g$ is $C_g$-smooth and $\mu_g$-strongly convex in $y$. The constraint $h$ is convex in $y$ and $C_h$-smooth. 
%     \item\label[assum]{item:assumption_safe_constraints} Primal and dual optimizers: Given $x$, denote the LL primal and dual solution $y^*(x), \gamma(x) = \arg\max\nolimits_\theta \min\nolimits_{\beta \geq 0} g(x,y) + \beta h(x,y)$. % \gk{undefined at this point.} 
%     We assume  $y^*(x)$ is $L_y$-Lipschitz in $x$, and that the dual solution $\gamma(x)$ is  bounded: $\norm{\gamma(x)} \leq R$. 
%     \jz{maybe we should point out that this implies some full recourse assumption, that is, for every $x$ there exists some $y$ to make the LL problem feasible.}
% }   
% \end{assumpenum}
\end{assumption}

\begin{assumption}\label{assumption:eq}For \cref{prob:lin-eq} (with linear equality constraints), we additionally assume that the set $\mathcal{X}$ is convex and compact, and that the objective $g$ is $S_g$-Hessian smooth, that is, $\norm{\grad^2 g(x,y) -\grad^2 g(\bar x,\bar y)}\leq S_g \norm{(x,y) - (\bar x, \bar y)} \forall x,\bar x \in \mathcal{X}, \text{ and } y, \bar y \in \R^{d_y}.$
% \begin{assumpenum}
% \compresslist{
%     \item  
% }
% \end{assumpenum}
\end{assumption}

\looseness=-1\cref{item:assumption_upper_level,item:assumption_lower_level} correspond to standard regularity assumptions in bilevel optimization. 
\cref{{item:assumption_tangen_space}} that  $B$ has full rank is the same as the complete recourse assumption in stochastic programming \cite{shapiro2021lectures}, that is, the LL problem is feasible $y$ for every $x\in\R^{d_x}$.
\cref{item:assumption_safe_constraints} is  needed only for the convex inequality case 
and ensures Lipschitz-continuity of the hyperobjective $F$. 
% to bound the non-smooth change of the LL problem solutions and their impact to the Lipschitzness of hyperobjective objective, which is later used to bound the convergence of bilevel algorithms.
\cref{assumption:eq} is used only in the equality case and guarantees smoothness of $F$.

\iffalse
Specifically, we also assume that the optimal solution $y^*(x)$ to be Lipschitz in $x$, and the dual solution is upper bounded by a constant $R$. 
\begin{assumption}[Bilevel solution assumptions]\label{assumption:safe-constraints}
    Given $x$, the lower level problem primal solution $y^*$, and the dual solution $\gamma(x)$, we assume
    \begin{itemize}
        \item $y^*(x)$ is $L_y$-Lipschitz in $x$. 
        \item The dual solution $\gamma(x)$ is upper bounded: $\norm{\gamma(x)} \leq R$.
        % This implies $\norm{M^{-1} \begin{bmatrix}
        %     \nabla^2_{xy} g + \gamma^\top \nabla_{xy}^2 h \\
        % \text{diag}(\gamma) \nabla_x h
        % \end{bmatrix}} \leq C_M$ with a constant $C > 0$, where $M = \begin{bmatrix}
        % \nabla^2_{yy} g + \gamma \nabla_{yy}^2 h & \nabla_y h_S^\top \\
        % \text{diag}\gamma \nabla_y h_S & 0
        % \end{bmatrix}$ as defined in Section~\ref{sec:differentiable-optimization}.
    \end{itemize}
\end{assumption}
\fi 

==> src/random-idea.tex <==
\section{Random Ideas}
\subsection{Multi-objective Optimization Formulation}
The above bilevel optimization problem is equivalent to the following multi-objective optimization problem with an additional constraint.

\begin{align}
    \min_{\mechanism, \decision, \newdecision} & \quad \objective(\mechanism, \decision) ~ \text{and} ~ g(\mechanism, \newdecision) \\
    \text{s.t.} & \quad \decision = \newdecision \\ 
    & \quad \decision, \newdecision \in \Decision \\
    & \quad \mechanism \in \Mechanism
\end{align}


One of the most commonly used solutions to multi-objective optimization problem is to apply a weighted sum to multiple objectives to reduce to a single-objective optimization problem:

\begin{align}
    \min_{\mechanism, \decision, \newdecision} & \quad \objective(\mechanism, \decision) + w g(\mechanism, \newdecision) \\
    \text{s.t.} & \quad \decision = \newdecision \\
    & \quad \mechanism \in \Mechanism
\end{align}
where the weight $w$ is a hyper-parameter that can be tuned.
\textcolor{red}{Jimmy: I wonder if some strong regularity condition is required for existence of some $\omega$ to make it work. For the simple Bilevel optimization problem, a sufficiently large $\omega$ should be good.}


\subsection{Nonsmooth formulations}

Considering Eq.~\ref{eqn:two_constraints}, one can replace the two constraints $g(x,y)\leq g^*(x),~h(x,y)\leq0$ by the single constraint 
\[
c(x,y):=\max\{g(x,y)-g^*(x),h(x,y)\}\leq 0~.
\]
Note that whenever $g,h$ are $L$-Lipschitz and $\alpha$-strongly convex, then so is $c$, so good properties (other than smoothness) are preserved. This reduces the Lagrangian based analyses to a single multiplier, which seems good. Also note that we need to evaluate now the gradient of $c$, but this is possible whenever we have 0th+1st order access to $g,g^*,h$, since $\partial \max\{f_1,f_2\}=\mathrm{conv}\{\nabla f_i:f_i\mathrm{~attains~the~max}\}$.



Unrelated but also useful in this context, is that we can probably reduce the dimension dependence of \cite{chen2023bilevel} from $d^{3/2}$ to $d$. Their algorithm uses the gradient-free method of \cite{lin2022gradient} which suffers from a $d^{3/2}$ dependence, while they extend the analysis to hold for inexact zero-order oracles. Using instead the algorithm from \cite{kornowski2023algorithm} would reduce the dimension-dependence to $d$, if we show that this algorithm works with inexact oracles as well. The heart would be showing that \citep{cutkosky2023optimal} works under biased oracles. For a very concise analysis of that algorithm, I recommend the blog post: https://truenobility303.github.io/Optimal-NSNC/ (+ run through google translate if needed).

\subsection{Possibly using prior work via prox point method?}
The work of \cite{sabach2017first} provides an  algorithm for $\min_{x\in \arg\min f(x) + g(x)} \omega(x),$ where $f$ is smooth convex, $g$ is nonsmooth convex, and $\omega$ is smooth and convex. In particular, they prove convergence to an $\epsilon$-additive solution in both the outer and inner level problems at an iteration cost of $\epsilon^{-1}$, with a prox operation per iteration. Currently, it's not entirely clear to me if they allow any $g$ or only prox-friendly $g$. Can we use $g(x)= \delta_{h(x)\leq 0}$ (i.e., the indicator of the desired constraint set) and apply \cite{sabach2017first} directly? Their algorithm requires the use of the prox operator; specifically, to apply their algorithm as a blackbox, we need to understand to what accuracy they need to compute $\min_{x: h(x) \leq 0} \|u-x\|_2^2$ for some fixed $u$. Note that \cite{beck2014first} solves the constrained bilevel problem but seem to be limited to  the constraint set being ``prox-friendly''. Can we extend this to the general (strongly convex) $h$ case? Does \cite{sabach2017first} extend to $\omega$ not strongly convex; they seem to use properties of the resolvent of the gradient, which perhaps has extensions in the weakly convex settings. Also note that \cite{jiang2023conditional} improves upon \cite{sabach2017first}. 

==> src/related-work.tex <==
\subsection{Related Work}

%latex note: we are using the nicematrix package to be able to get alternately shaded rows when we have multiple rows per row: this feature seems difficult to get with merely tabular (booktabs) see https://stackoverflow.com/questions/69174994/how-to-create-a-latex-table-with-specific-multicolumns-and-multirows
\begin{table}[h]
  \centering
  \resizebox{\linewidth}{!}{%
  \begin{NiceTabular}{*{11}{c}}
  \CodeBefore
  \rowcolors{1}{}{gray!10}[respect-blocks]
  \Body
    \toprule
    \Block{2-1}{\textbf{Paper}} & \Block{1-2}{\textbf{Upper Objective}} & & \Block{1-2}{\textbf{Upper Constraint}} & & \Block{1-2}{\textbf{Lower Objective}} & & \Block{1-2}{\textbf{Lower Constraint}} & & \Block{1-2}{\textbf{Cost}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
    & $C(x,y)$ & Smoothness & $C(x,y)$ & Smoothness & $C(x,y)$ & Smoothness & $C(x,y)$ & Smoothness & Iters. & Per Iter.\\
    \midrule
    \cite{liu2021value} & Cell 1,2.1 & Cell 1,2.2 & Cell 1,2.3 & Cell 1,3 & Cell 1,4 & Cell 1,5 & None \\
    \cite{ji2021bilevel} & --- & \checkmark & --- & --- & (, \strongconvexity) & \checkmark & --- & --- & $\kappa^3 \varepsilon^{-1}$ & Hess$\times$vec \\  
    \cite{kwon2023fully} & --- & \checkmark & \checkmark (set) & --- & (, \strongconvexity) & \checkmark & --- & --- & $\varepsilon^{-3}$ & FO \\
    \cite{chen2023near} & --- & (\checkmark, \checkmark) & --- & --- & (, \strongconvexity) & \checkmark & --- & --- & $\kappa^4\varepsilon^{-2}$ & FO \\
       \Block{2-1}{\cite{abolfazli2023inexact}} & none & (\checkmark, \checkmark) & \checkmark (set) & --- & (, \strongconvexity) & \checkmark & --- & --- & $\varepsilon^{-2}$ & mv \\
    & (\checkmark, \checkmark) & & & & & & & & $\varepsilon^{-1}$ \\
    \cite{tsaknakis2022implicit} & & & & & & & \checkmark(linear) & &  asymptotic\\ 
    \Block{4-1}{\cite{khanduri2023linearly}} & --- & (\checkmark, \checkmark) & \checkmark (set) & --- & (, \strongconvexity) & \checkmark & \checkmark (linear) & \xmark & asymptotic & --- \\
      & weak ($F$) & (\checkmark, \checkmark) & \checkmark (set) & --- & (, \strongconvexity) & \checkmark & \checkmark (linear) & \xmark & $\varepsilon^{-2}$  & \Block{3-1}{Hess$\times$vec} \\ 
      & convex  ($F$) & (\checkmark, \checkmark) & \checkmark (set) & --- & (, \strongconvexity) & \checkmark & \checkmark (linear) & \xmark & $\varepsilon^{-2}$ & \\ 
      & strongly  ($F$)  & (\checkmark, \checkmark) & \checkmark (set) & --- & (, \strongconvexity) & \checkmark & \checkmark (linear) & \xmark & $\varepsilon^{-1}$ &  \\ 
    \cite{ye2023difference} & diff. of convex & \checkmark & \checkmark (set) & --- & (\checkmark, \checkmark) & --- & (\checkmark, \checkmark) & --- &  asymptotic & \\
    \cite{gao2024moreau} & diff. of weak & & \checkmark (set) & --- & (\checkmark\hspace{-0.5ex}\textsubscript{w}, \checkmark) & \checkmark & (\checkmark, \checkmark) & & asymptotic \\
    \cite{yao2024constrained} & & \checkmark & \checkmark & \checkmark & (, \checkmark) & \checkmark & ?? \\
    \cite{DMLCBO} & --- & \checkmark & \checkmark (set) & & (, \strongconvexity) & \checkmark & \checkmark (set) & --- & $d_2^2 \varepsilon^{-4}$ & {\thead{PO, \\ inv Hess}} \\ 
    \bottomrule
\end{NiceTabular}
  }
  \captionsetup{font=scriptsize}
  \caption{All known (to us) results for two-variable bilevel problems. We use $\strongconvexity$ and $\weakconvexity$ to denote strong and weak convexity, respectively. We use $C(x,y)$ to denote the convexity in the tuple $(x,y)$. In \cite{khanduri2023linearly}, there are only smoothness assumptions on the component functions and (weak/strong) convexity assumptions on the overall smoothed implicit function $F$ (\pswt{I think this is stronger than imposing assumptions on the individual component functions making up $F$}) for nonasymptotic rates. In \cite{DMLCBO}, the $d_2$ is the dimension of the variable $y$. \pswt{Note: this table is still work in progress, and some cells are simply copied from others (when copying the corresponding rows); feel free to correct any of the cells}}
  \label{tab:distinct-columns}
\end{table}


% \begin{table}[h]
%   \centering
%   \resizebox{\linewidth}{!}{%
%   \begin{tabular}{ccccccccccc}
%     \toprule
%     \multirow{2}{*}{\textbf{Paper}} & \multicolumn{2}{c}{\textbf{Upper Objective}} & \multicolumn{2}{c}{\textbf{Upper Constraint}} & \multicolumn{2}{c}{\textbf{Lower Objective}} & \multicolumn{2}{c}{\textbf{Lower Constraint}} & \multicolumn{2}{c}{\textbf{Cost}} \\
%         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
%     & $C(x,y)$ & Smoothness & $C(x,y)$ & Smoothness & $C(x,y)$ & Smoothness & $C(x,y)$ & Smoothness & Iters. & Per Iter.\\
%     \midrule
%     \makecell{\cite{liu2021value}} & \makecell{Cell 1,2.1} & \makecell{Cell 1,2.2} & \makecell{Cell 1,2.3} & \makecell{Cell 1,3} & \makecell{Cell 1,4} & \makecell{Cell 1,5} & \makecell{None} \\
%     \makecell{\cite{kwon2023fully}} & \makecell{Cell 2,2.1} & \makecell{Cell 2,2.2} & \makecell{Cell 2,2.3} & \makecell{Cell 2,3} & \makecell{Cell 2,4} & \makecell{Cell 2,5} & & & \makecell{$\varepsilon^{-3}$} \\
%     \makecell{\cite{chen2023near}} & \makecell{Cell 2,2.1} & \makecell{Cell 2,2.2} & \makecell{Cell 2,2.3} & \makecell{Cell 2,3} & \makecell{Cell 2,4} & \makecell{Cell 2,5} & & &  \makecell{$\varepsilon^{-2}$} \\
%       \multirow{4}{*}{\makecell{\cite{khanduri2023linearly}}} & \makecell{---} & \makecell{(\checkmark, \checkmark)} & \makecell{\checkmark (set)} & \makecell{---} & \makecell{(, strong)} & \makecell{\checkmark} & \makecell{\checkmark (linear)} & \makecell{\xmark} & \makecell{asymptotic} & \makecell{---} \\
%       & \makecell{weak ($F$)} & & & & & & & & \makecell{$\varepsilon^{-2}$} & \makecell{$\geq$Hessian} \\ 
%             & \makecell{convex  ($F$)}  & & & & & & & & \makecell{$\varepsilon^{-2}$} & \makecell{$\geq$Hessian}\\ 
%       & \makecell{strongly  ($F$)}  & & & & & & & & \makecell{$\varepsilon^{-1}$} & \makecell{$\geq$Hessian} \\ 
%   \multirow{2}{*}{\makecell{\cite{abolfazli2023inexact}}} & \makecell{none} & \makecell{(\checkmark, \checkmark)} & \makecell{\checkmark (set)} & \makecell{---} & \makecell{(, strong)} & \makecell{\checkmark} & \makecell{---} & \makecell{---} & \makecell{$\varepsilon^{-2}$} & \makecell{mv} \\
% & \makecell{(\checkmark, \checkmark)} & & & & & & & &  \makecell{$\varepsilon^{-1}$} \\
%     \makecell{\cite{ye2023difference}} & \makecell{} & \makecell{\checkmark} & \makecell{\checkmark} & \makecell{\checkmark, \xmark} & \makecell{\checkmark} & \makecell{\checkmark} & \makecell{None} \\
%     \makecell{\cite{gao2024moreau}} & \makecell{diff. of weak} & \makecell{} & \makecell{\checkmark (set)} & \makecell{---} & \makecell{(weak, \checkmark)} & \makecell{\checkmark} & \makecell{(\checkmark, \checkmark)} & & \makecell{asymptotic} \\
%     \makecell{\cite{yao2024constrained}} & \makecell{} & \makecell{\checkmark} & \makecell{\checkmark} & \makecell{\checkmark} & \makecell{(, \checkmark)} & \makecell{\checkmark} & \makecell{??}  \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{All Known (to us) Results for Two-Variable Bilevel Problems. We use $C(x,y)$ to denote the convexity in the tuple $(x,y)$. In \cite{khanduri2023linearly}, there are only smoothness assumptions on the component functions and (weak/strong) convexity assumptions on the overall smoothed implicit function $F$ for nonasymptotic rates. \pswt{Note: this is still work in progress, feel free to correct any of the cells}}
%   \label{tab:distinct-columns}
% \end{table}

\paragraph{Lagrangian Approximation of the Hyperobjective}
Interestingly, so far, this has been the only approach to achieving truly Hessian-free algorithms. \pswt{This (not-yet-fully verified) assertion is based on me currently not understanding how \cite{yao2024constrained} is claimed to be  "hessian-free".} This remarkable breakthrough was achieved by \cite{kwon2023fully} who reformulated the given problem into a Lagrangian form, and with some very simply --- but  clever --- observations, were able to perform hypergradient updates by using \emph{exclusively first-order components}! Their rate was $\varepsilon^{-3}$ iterations, each performing only gradient computations. \pswt{note: the true dependence on $\kappa$ and polylog factors isn't shown here; see \cite{chen2023near} for this.} In another remarkable paper, \cite{chen2023near} did a more careful analysis of the algorithm and technique in \cite{kwon2023fully} to get the optimal number of iterations $\varepsilon^{-2}$. At the heart of \cite{kwon2023fully}'s novelty is a first-order approximation of the hypergradient. \pswt{To extend this to our setting, can we get a similar first-order approximation of the \emph{projected} hypergradient?}

\cite{landry2019differentiable}: no complexity analysis. 

% \cite{kwon2023fully} ($\epsilon^{-3} \log {\frac{1}{\epsilon}}$) and \cite{chen2023near} ($\epsilon^{-2} \log {\frac{1}{\epsilon}}$)

\paragraph{Smoothing the Lower-Level Solution.}
The gradient of the solution $y^\ast(x)$ of the lower-level problem plays a central role in the hypergradient (i.e., gradient of the overall objective). However, one cannot in general assume $y^\ast(x)$ to be differentiable. Some papers impose assumptions on the lower-level objective (and constraint, if needed) so that they can obtain this differentiability for free; others (which we discuss in this subsection) achieve this property via some kind of smoothing. So far, we have observed two kinds of smoothing: one via inf-convolution (also called Moreau envelope) and the other via random perturbation (e.g., \cite{khanduri2023linearly} and \cite{DMLCBO}.). We discuss these approaches below. 

The work of \cite{liu2021value} studies $\min_{x\in \mathcal{X}, y^\ast(x)\in \arg\min f(x,y)\leq 0} F(x, y^\ast(x))$, assuming only continuous differentiability of $F$ and $f$. Conceptually, the paper performs a very simple algorithm: reformulate the problem as one requiring $y$ be in the set $f(x, y) - \min_y f(x, y)\leq 0$, then uses inf-convolution to smoothen $\min_y f(x, y)$. It then transforms the bilevel problem into a single-level one by incorporating the (smoothed) constraint into the objective via a \emph{barrier} function, as is done in interior-point methods. Finally, it uses inf-convolution again to smoothen the resulting objective function of $x$. The algorithm therefore iteratively performs the following sequence of steps: first, compute the minimizer of the smoothed lower-level constraint; second, find the minimizer (with respect to $y$) of the smoothed barrier objective; third, we take a gradient step (with respect to $x$) on the smooth barrier objective. This whole subroutine is then run in the IPM framework. The paper does not provide a non-asymptotic convergence guarantee, but their technique of smoothing via inf-convolution is used in many other papers, and in what follows, we describe some of the most relevant such works. 

First, we note the work of \cite{ye2023difference}, which performs a ``value function smoothing'' via inf-convolution, then notes that the resulting problem is a difference of convex functions. It then uses established techniques from the DC programming literature to solve this problem. The paper provides asymptotic convergence guarantees. 

The (very) recent work of \cite{gao2024moreau} extends the work of \cite{ye2023difference} by removing the convexity assumption on the second variable of the lower-level problem. To do so, the paper proves weak convexity of the Moreau envelope. \pswt{To check: \cite{davis2019stochastic} already proved that the Moreau envelope of any weakly convex function is smooth with Lipschitz continuous gradient; doesn't this already imply weak convexity of the Moreau envelope? Specifically, doesn't Lemma $2.2$ of \cite{davis2019stochastic} subsume Theorems $2$ and $3$ of \cite{gao2024moreau}?} The paper provides asymptotic guarantees (see Theorem $18$).

Another similarly relevant paper that also falls under the framework of ``value function smoothing'' is that of 
  \cite{yao2024constrained}, which studies \[\min_{x\in \mathcal{X}, y^\ast(x)\in \arg\min_{y\in \left\{\mathcal{Y}\cap g(x, y)\leq 0\right\}} f(x,y)} F(x, y^\ast(x)),\] which is essentially identical to our setup. The paper's first idea is to incorporate the lower-level constraint $g(x,y)\leq0$ into the lower-level objective via a Lagrange multipler they call $\lambda$ \pswt{(note that they seem to consider $\lambda$ to be a variable independent of $x$: is this valid?)} and then using the same inf-convolution as in \cite{liu2021value} to smoothen $\min_{y\in \mathcal{Y}} f(x,y) + \lambda g(x,y)$. One key innovation is to bound $\lambda$ in the optimization used in the smoothening process. \pswt{(Note: What is the justification for this bound? How can we ensure that we will not miss the correct $\lambda$ by imposing this bound?)} The algorithm then proceeds iteratively, performing the following sequence of steps: first, it computes the minimizer of these two inf-convolutions with the current $x$, $y$, and $z$; second, it updates $x$ and $y$; third it updates $z$. \pswt{The operation of updating $x$ and $y$ is performed via a projection onto the set $\left\{y\in \mathcal{Y}| g(x, y)\leq 0\right\}$. Would the final runtime not have to consider the cost of this operation? Can we ensure it is Hessian-free, as the title claims the paper to be?} Also, \pswt{This is the only paper that \emph{claims} what our goal is; so we would need to definitely write down their correct runtime in order for us to be able to compare with them}

  Another approach to smoothing is seen in the work of \cite{khanduri2023linearly}. The authors perform a slightly different kind of smoothing, by using random perturbation. Overall, their algorithm is as follows: randomly perturb the lower-level objective, then compute the $y^\ast(x)$ corresponding to this perturbed lower-level (linearly constrained) problem. The perturbation enables differentiability of $y^\ast(x)$ (note that the expression for $\nabla_x y^\ast(x)$ has the optimal lower-level Lagrangian in it; in this setting, because the lower-level constraint is linear, the authors are able to get a closed-form expression for it \pswt{Note: the authors seem to provide a very in-depth analysis of the conditions required for differentiability of $y^\ast(x)$; I wasn't able to see such in-depth proofs in other papers, all of which use the differentiability of $y^\ast(x)$}), which is then used in computing the hypergradient; the variable $x$ is then updated using this hypergradient. The authors provide nonasymptotic rates by imposing additional assumptions of weak convexity/convexity/strong convexity on the hyperobjective obtained by perturbed smoothing. The authors also show "closeness" of the perturbed smoothed hyperobjective from the true hyperobjective. \pswt{My main concern is that the authors do not seem to have proved \emph{under what conditions on the original problem} can one see this imposed assumption on the perturbed smoothed objective $F$. Without such a proof, wouldn't their theorem be essentially incomplete?} 

  In \cite{DMLCBO}, the authors consider bilevel optimization with both upper and lower level constraints, the constraints given as explicitly defined convex sets. The authors use a closed-form formula for the hypergradient citing a result from \cite{blondel2022efficient}. Note: \pswt{This expression requires the computation of the inverse of a product of a matrix with a Gaussian-smoothed projection operator}. Instead of using the true projection operator, they use a Gaussian-smoothed version of it, thus incurring an extra dimension factor in the smoothness constant. The convergence metric used is like a gradient mapping of the projection.\pswt{Is their proof of Lemma 6 correct?}    
 
\paragraph{Projection-Free Approaches}
There has been some attempt at developing projection-free algorithms for various versions of bilevel optimization. Below, describe as many approaches as possible. 

In \cite{abolfazli2023inexact}, the authors consider $\min_{x\in \mathcal{X}, y^\ast(x)\in \arg\min_y g(x,y).} f(x, y^\ast(x))$. Note that the constraint here is in the \emph{upper-level} problem, unlike what we are considering. They assume the lower-level objective to be strongly convex and smooth; they assume the upper-level objective to be smooth, providing results for both convex and nonconvex assumptions on $f$. 
% \pswt{Note I found their assumptions somewhat difficult to parse (I believe they are all fine, just a bit technically dense for me)}. 
Their algorithm is very natural: They compute the hypergradient, followed by updating $x_k$ via Frank-Wolfe (to ensure feasibility in $\mathcal{X}$), followed by updating $y_k$ (which approximates $y^\ast(x_k)$) via a gradient step on $g$. While the naive approach to the first step (taking a gradient step on the hyperobjective) would require an expensive matrix inversion, the authors come up with a simple new idea (presented in their equations $7a$ and $7b$) that essentially changes the order of operations in the naive approach; this circumvents the expensive operations from the naive approach. We note two important points here: First: \pswt{Their equations $7a$ and $7b$, which are two slightly new steps show up in Proposition $1$ of \cite{ji2021bilevel} as well.} Second: \pswt{Given the overall nonconvexity, wouldn't convergence heavily rely on very accurate initialization, and wouldn't the stationary guarantee be weak-ish? I'm also very confused about the fact that Lemma $2.1$'s ``Lipschitz/smoothness constants" look really bad (i.e., square of some condition number), but somehow those bad constants disappear in the final iteration cost (e.g., see the proof of Corollary $4.2$) and are omitted in the results table.} 

==> src/symbols.tex <==

\newcommand{\N}{\mathbb{N}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\Sbb}{\mathbb{S}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\tbg}{\tilde{\mathbf{g}}}

\newcommand{\bg}{\mathbf{g}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\out}{\mathrm{out}}
\newcommand{\tf}{\tilde{f}}
\newcommand{\tvphi}{\tilde{\varphi}}
\newcommand{\tF}{\tilde{F}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\inner}[1]{\left\langle#1\right\rangle}

%%% way too many specialized macros: 
\global\long\def\ys{y^{\star}}%
\global\long\def\ysl{y_{\lambda}^{\star}}%
\global\long\def\fxxys{\nabla_{x}f(x,\ys)}%
\global\long\def\fyxys{\nabla_{y}f(x,\ys)}%
\global\long\def\dysdx{\frac{d\ys}{dx}}%
\global\long\def\fxxysl{\nabla_{x}f(x,\ysl)}%
\global\long\def\fyxysl{\nabla_{y}f(x,\ysl)}%
\global\long\def\gxxysl{\text{\ensuremath{\nabla_{x}g(x,\ysl)}}}%
\global\long\def\gyxysl{\nabla_{y}g(x,\ysl)}%
\global\long\def\hxxysl{\nabla_{x}h(x,\ysl)}%
\global\long\def\hyxysl{\nabla_{y}h(x,\ysl)}%
\global\long\def\gxxys{\nabla_{x}g(x,\ys)}%
\global\long\def\hxxys{\nabla_{x}h(x,\ys)}%
\global\long\def\hyxys{\nabla_{y}h(x,\ys)}%
\global\long\def\gyxys{\nabla_{y}g(x,\ys)}%


